Demystifying Privacy Policy of Third-Party Libraries in Mobile Apps

The privacy of personal information has received significant attention in mobile software. Although previous researchers have designed some methods to identify the conflict between app behavior and privacy policies, little is known about investigating regulation requirements for third-party libraries (TPLs). The regulators enacted multiple regulations to regulate the usage of personal information for TPLs (e.g., the "California Consumer Privacy Act" requires businesses clearly notify consumers if they share consumers' data with third parties or not). However, it remains challenging to analyze the legality of TPLs due to three reasons: 1) TPLs are mainly published on public repositoriesinstead of app market (e.g., Google play). The public repositories do not perform privacy compliance analysis for each TPL. 2) TPLs only provide independent functions or function sequences. They cannot run independently, which limits the application of performing dynamic analysis. 3) Since not all the functions of TPLs are related to user privacy, we must locate the functions of TPLs that access/process personal information before performing privacy compliance analysis. To overcome the above challenges, in this paper, we propose an automated system named ATPChecker to analyze whether the Android TPLs meet privacy-related regulations or not. Our findings remind developers to be mindful of TPL usage when developing apps or writing privacy policies to avoid violating regulations.

==> CaseStudy.tex <==
\noindent\textbf{Case study}
For example, TPL: com.noqoush.adfalcon

PP: http://www.adfalcon.com/en/3p-tag-policy.html

data trace:

% 	$d3 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLongitude()>() --> if $b3 == 0 goto return r1
% 	$d3 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLongitude()>() --> $b3 = $d3 cmpl -1.0
% 	$z2 = virtualinvoke r3.<android.location.LocationManager: boolean isProviderEnabled(java.lang.String)>("network") --> if $z2 == 0 goto return
% 	$d5 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLongitude()>() --> $r16 = virtualinvoke $r15.<java.lang.StringBuilder: java.lang.StringBuilder append(double)>($d5)
% 	$d4 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLatitude()>() --> $r11 = virtualinvoke $r10.<java.lang.StringBuilder: java.lang.StringBuilder append(double)>($d4)
% 	$r4 = virtualinvoke r3.<android.location.LocationManager: java.util.List getAllProviders()>() --> $z1 = interfaceinvoke $r4.<java.util.List: boolean contains(java.lang.Object)>("network")
% 	$d2 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLatitude()>() --> if $b2 == 0 goto return r1
% 	$d2 = virtualinvoke r2.<com.noqoush.adfalcon.android.sdk.ADFTargetingParams: double getLocationLatitude()>() --> $b2 = $d2 cmpl -1.0
% 	$d1 = virtualinvoke r1.<android.location.Location: double getLongitude()>() --> virtualinvoke $r2.<com.noqoush.adfalcon.android.sdk.g: void b(double)>($d1)
% 	$d0 = virtualinvoke r1.<android.location.Location: double getLatitude()>() --> virtualinvoke $r0.<com.noqoush.adfalcon.android.sdk.g: void a(double)>($d0)

conflict : location

location:permission: "android.permission.ACCESS-\_COARSE\_-LOCATION" / "android.permission.ACCESS-\_FINE-\_LOCATION" 

==> figures/algorithm_data_flow.tex <==
\RestyleAlgo{ruled}


\begin{algorithm}[]
% \vspace{-2ex}
\caption{Data usage analysis}\label{alg:data_flow}
\label{alg:data_usage}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  
  \KwInput{method $m_t$, statement $s_t$, variable $v_t$}
  \KwOutput{data usage $FD$ of variable $v_t$}
  
 

% Set Function Names
    \SetKwFunction{FInterMVA}{InterMethodVarAnalysis}
    \SetKwFunction{FIntraMVA}{IntraMethodVarAnalysis}
    \SetKwFunction{FForwar}{ForwardAnalysis}
    \SetKwFunction{FBackwar}{BackwardAnalysis}
  
    % BackwardAnalysis($src_{var}$, $src_{stmt}$, $src_{m}$)\;
    BackwardAnalysis($m_t$, $s_t$, $v_t$)\;

    IntraMethodVarAnalysis($m_t$, $s_t$, $v_t$) \;
    % \vspace{-1.1ex}\;\vspace{-1.1ex}
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FIntraMVA{$m$, $stmt$, $var$}}{
        $uses$ = find statements that use $var$ in method $m$ \;
        \For{$u$ in $uses$}{
            store($var$, u) in $DF$ \;
            ForwardAnalysis($m$, $u$, $var$)
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    \SetKwProg{Fn}{Def}{:}{\KwRet}
    \Fn{\FBackwar{$m_t$, $s_t$, $v_t$}}{
        % InterProcedureVariableAnalysis($m$, $stmt$, $var$)  \;
        % $cfg$ = construct\_cfg($m$)\;
        $defs$ = getDefsOfAt($v_t$, $s_t$, $cfg$)  \;
        \For{$d$ in $defs$}{
            $src_{var}$ = get the signature of $v_t$ in $d$\;
            $caller_{list}$ = find methods that invoke $m_t$ \;
            \For{$m$ in $caller_{list}$}{
                $src_{stmt}$ = statements that invoke $m_t$ in $m$\;
                $src_{v}$ = variables in $src_{stmt}$ that correspond to $v_t$\;
                \If{$src_{v}$  is \textit{Variable}}{
                    BackwardAnalysis($src_{v}$, $src_{stmt}$, $src_{m}$)
                } \ElseIf{$src_{v}$ is \textit{Constant}}{
                    store ($v_t$, $src_{stmt}$) in $DF$
                }
            }
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FForwar{$m$, $stmt$, $var$}}{
        $tar_{stmt}$ = find all statements that contain $stmt$ \;
        \For{$s$ in $tar_{stmt}$}{
            store ($var$, $s$) in $DF$ \;
            \If{$s$ contain invoke statements}{
                $tar_{m}$ = method that invokes $stmt$ in $s$ \;
                $tar_{v}$ = variable in $tar_{m}$ that correspond to $var$\;
                ForwardAnalysis($tar_{method}$, $s$, $tar_{v}$)
            }
        }
    }

% \vspace{-1ex}
\end{algorithm}


==> table/PI_related_API_list.tex <==
\begin{table}[]
\centering
\smaller
\vspace{2ex}
\caption{Personal information and corresponding API}
\scalebox{0.95}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.14\textwidth}@{}}
\toprule
\textbf{PI}                    & \textbf{Class Name}                                      & \textbf{Method Name}                         \\ \midrule
Ad ID                          & AdvertisingIdClient                                      & AdvertisingIdClient                          \\
\rowcolor[HTML]{EFEFEF} 
Bluetooch address              & android.bluetooth.BluetoothAdapter                       & getAddress                                   \\
Camera                         & android.hardware.Camera                                  & setPreviewDisplay                            \\
\rowcolor[HTML]{EFEFEF} 
Cell   Loca-tion                & android.telephony.TelephonyManager                       & getCellLocation                              \\
Contact                        & android.provider.ContactsContract                        & PhoneLookup                                  \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude          \\
                               & android.location.Location                                & getLongitude                                 \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLastKnownLocation \\
                               & android.location.LocationManager                         & requestLocationUpdates                       \\
\multirow{-5}{*}{GPS Location} & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLongitude         \\
Sim Number                     & android.telephony.TElephonyManager                       & getSimSerialNumber                           \\
\rowcolor[HTML]{EFEFEF} 
IMEI                           & android.telephony.TElephonyManager                       & getDeviceId                                  \\
IMSE                           & android.telephony.TElephonyManager                       & getSubscriberId                              \\
\rowcolor[HTML]{EFEFEF} 
Location                       & java.util.Calendar                                       & getTimeZone                                  \\
MAC address                    & android.net.wifi.WifiInfo                                & getMacAddress                                \\
\rowcolor[HTML]{EFEFEF} 
Password                       & android.accounts.AccountManager                          & getPassword                                  \\
Phone   Number                 & android.telephony.TelephonyManager                       & getLine1Number                               \\
\rowcolor[HTML]{EFEFEF} 
SMS                            & android.telephony.SmsManager                             & sendTextMessage                              \\
SSID                           & android.net.wifi.WifiInfo                                & getSSID                                      \\
\rowcolor[HTML]{EFEFEF} 
User Credential                & android.accounts.AccountManager                          & getAccounts                                  \\
UserName                       & android.os.UserManager                                   & getUserName                                  \\ \bottomrule
\end{tabular}
}
\label{tab:pi_api}
\end{table}



\begin{comment}
\begin{table}[]
\centering
\smaller
\caption{Personal information and corresponding API}
\scalebox{0.98}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.15\textwidth}@{}}
\toprule
\textbf{PI}                   & \textbf{System Class}              & \textbf{Method}        \\ \midrule
Ad ID                         & AdvertisingIdClient                & AdvertisingIdClient    \\
Bluetooch address             & android.bluetooth.BluetoothAdapter & getAddress             \\
Camera                        & android.hardware.Camera            & setPreviewDisplay      \\
Cell   Location               & android.telephony.TelephonyManager & getCellLocation        \\
Contact                       & android.provider.ContactsContract  & PhoneLookup            \\
\multirow{5}{*}{GPS Location} & android.location.Location          & getLatitude            \\
                              & android.location.Location          & getLongitude           \\
                              & android.location.LocationManager   & getLastKnownLocation   \\
                              & android.location.LocationManager   & requestLocationUpdates \\
                              & android.location.LocationManager   & getLongitude           \\
Sim Number                    & android.telephony.TElephonyManager & getSimSerialNumber     \\
IMEI                          & android.telephony.TElephonyManager & getDeviceId            \\
IMSE                          & android.telephony.TElephonyManager & getSubscriberId        \\
Location                      & java.util.Calendar                 & getTimeZone            \\
MAC address                   & android.net.wifi.WifiInfo          & getMacAddress          \\
Password                      & android.accounts.AccountManager    & getPassword            \\
Phone   Number                & android.telephony.TelephonyManager & getLine1Number         \\
SMS                           & android.telephony.SmsManager       & sendTextMessage        \\
SSID                          & android.net.wifi.WifiInfo          & getSSID                \\
User Credential               & android.accounts.AccountManager    & getAccounts            \\
UserName                      & android.os.UserManager             & getUserName            \\ \bottomrule
\end{tabular}%
}
\label{tab:pi_api}
\end{table}
\end{comment}

\begin{comment}


\begin{table}[]
\caption{}
\label{tab:my-table}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{PI}       & \textbf{System Class}              & \textbf{Method}      \\ \midrule
Bluetooch address & android.bluetooth.BluetoothAdapter & getAddress           \\
\rowcolor[HTML]{EFEFEF} 
Camera            & android.hardware.Camera            & setPreviewDisplay    \\
Cell   Location   & android.telephony.TelephonyManager & getCellLocation      \\
\rowcolor[HTML]{EFEFEF} 
Contact           & android.provider.ContactsContract  & PhoneLookup          \\
                  & android.location.LocationManager   & getLastKnownLocation \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}requestLocationUpdates \\
                  & android.location.LocationManager   & getLongitude         \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude            \\
\multirow{-5}{*}{GPS Location} & android.location.Location                                & getLongitude                                   \\
\rowcolor[HTML]{EFEFEF} 
ICCID             & android.telephony.TElephonyManager & getSimSerialNumber   \\
IMEI              & android.telephony.TElephonyManager & getDeviceId          \\
\rowcolor[HTML]{EFEFEF} 
IMSE              & android.telephony.TElephonyManager & getSubscriberId      \\
Location          & java.util.Calendar                 & getTimeZone          \\
\rowcolor[HTML]{EFEFEF} 
MAC address       & android.net.wifi.WifiInfo          & getMacAddress        \\
                  & android.media.MediaRecorder        & getAudioSource       \\
\multirow{-2}{*}{MIC}          & \cellcolor[HTML]{EFEFEF}android.media.MediaRecorder      & \cellcolor[HTML]{EFEFEF}startRecording         \\
Phone   Number    & android.telephony.TelephonyManager & getLine1Number       \\
\rowcolor[HTML]{EFEFEF} 
Sensors           & android.hardware.SensorManager     & getDefaultSensor     \\
SMS               & android.telephony.SmsManager       & sendTextMessage      \\
\rowcolor[HTML]{EFEFEF} 
SSID              & android.net.wifi.WifiInfo          & getSSID              \\
User Credential   & android.accounts.AccountManager    & getAccounts          \\
\rowcolor[HTML]{EFEFEF} 
UserName          & android.os.UserManager             & getUserName          \\
Password          & android.accounts.AccountManager    & getPassword          \\ \bottomrule
\end{tabular}
\end{table}

\end{comment}

==> table/abbreviation_table.tex <==
\begin{table}[t]
\centering
\smaller
\vspace{3.5ex}
\caption{Abbreviation used in this papaer}
\label{tab:abb}
\begin{tabular}{@{}ll@{}}
\toprule
Abbreviation & Full name                \\ \midrule
ADUP         & abstract data usage pattern \\
CC           & coordinating conjunction \\
CRF          & conditional random field \\
DPT          & dependency parse tree    \\
GSF          &  Google Services Framework Identifier \\
NER          & named entity recognition \\
NP           & noun phase               \\
POS          & part of speech           \\
PI           & personal information     \\
PP           & privacy policy           \\
SSI          & signature of sink invocation\\

            %  &                          \\     
             \bottomrule
\vspace{-3.5ex}
\end{tabular}
\end{table}


==> table/action_sharing_words.tex <==
\begin{table}[]
\centering
\smaller
\vspace{2ex}
\caption{Data sharing and collecting words}
%p{0.9\columnwidth}
\begin{tabular}{p{0.23\columnwidth}p{0.67\columnwidth}}
\toprule
\textbf{Action Type} & \textbf{Keywords} \\ \midrule
Collect     &  access, check, collect, gather, know, obtain, receive, save, store, use \\ \hline
Sharing     &  accumulate, afford, aggregate, associate,  cache,  combine, convert, connect,  deliver, disclose, distribute, disseminate, exchange,  gather, get, give, keep, lease, obtain, offer, post, possess, proxy,  provide, protect against, receive,  rent, report, request, save, seek, sell, share, send, track,  trade, transport, transfer, transmit\\ \bottomrule
\end{tabular}
\label{tab:actionwords}
\end{table}

==> table/atpchecker_metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\smaller
\vspace{2ex}
\caption{Metrics of {\oursystem} for identifying host apps' interaction with TPLs}
\label{tab:metrics}
\begin{tabular}{@{}ccccc@{}}
\toprule
          & TP       & TN        & FN     & FP   \\ \midrule
TPL\_list & 95       & 0         & 0      & 9    \\
TPL\_data & 223      & 0         & 0      & 12    \\ \midrule
          & Accuracy & Precision & Recall & F1   \\ \midrule
TPL\_list & 0.91     &	0.91 &	1 &	0.95    \\
TPL\_data & 0.95 &	0.95 &	1 &	0.97
 \\ \bottomrule
\end{tabular}%
\label{tab:metrics}
\end{table}

==> table/data_type_table.tex <==
\begin{table}[]
\centering
\smaller
\vspace{2ex}
\caption{Tracked data types in static analysis}
\begin{tabular}{p{0.9\columnwidth}}
\toprule
\textbf{Data Type} \\ \midrule
Ad ID, username, password, name, location, contact, phone number, email address, IMEI, Wi-FiMAC address,  GSF ID, Android ID, serial number, SIM serial number \\ \bottomrule
\end{tabular}
\label{tab:data_type}
\end{table}

==> table/regulation_summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\smaller
\vspace{1ex}
\caption{Personal information protection related regulations}
\scalebox{0.95}{%
\begin{tabular}{@{}p{0.4\textwidth}c@{}}
\toprule
Regulations                                                                              & Enact date \\ \midrule
\rowcolor[HTML]{EFEFEF} 
California Consumer Privacy Act (CCPA)                                                   & Jun-2018   \\
California Privacy Rights Act of 2020 (CPRA)                                             & Nov-2020   \\
\rowcolor[HTML]{EFEFEF} 
EU General Data Protection Regulation (GDPR)                                             & May-2018   \\
China Cybersecurity Practices Guidelines – Security Guidelines for Using Software Development Kit (SDK) for Mobile Internet Applications & Nov-2020 \\
\rowcolor[HTML]{EFEFEF} 
China Information security technology - Basic requirements for collecting personal information   in mobile internet applications         & Jan-2020 \\
China Information security technology - Personal information (PI) security specification & Oct-2020   \\
\rowcolor[HTML]{EFEFEF} 
New Zealand International Covenant on Civil and Political Rights (ICCPR) Privacy Act     & Jun-2020   \\ \bottomrule
\end{tabular}%
}
\label{tab:regulation}
\end{table}

==> tmp/Intro_0105.tex <==
\section{Introduction}

% \input{table/regulation_summary}


% \vspace{0.5em}
% \begin{quote}
%     \emph{\textbf{``Hedges have eyes and walls have ears.''}}
%     \begin{flushright}
%     - Trusler, John, 1735-1820.
%     \end{flushright}
% \end{quote}
% \vspace{1em}




Nowadays, smartphone and mobile apps are playing essential roles in our daily lives~\cite{deepintent2019SIGSAC}. 
%
Besides, more and more developers tend to use many off-the-shelf third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE}.
%
However, developers may omit the privacy threat in TPLs. 
%
For example, the advertisement libraries may leak users' personal information (e.g., IMEI)~\cite{short2014android}.
%
Some TPLs (e.g., advertising and analytic libraries) rely on the personal information to provide better service~\cite{demetriou2016free}.
%
However, TPLs may collect user data that is not necessary for providing related services. 
%
Such behaviors may lead to privacy leakage or even security concerns~\cite{harty2021logging, tangtse:21a, zhao2021structural}.
%
Besides, the permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}.
%
Since the host apps share the same process space and permissions with TPLs, 
%
the mechanism violates the principle of least privilege, which leads to TPLs being over-privileged.
%
Recent papers find that permission abuse makes TPLs access users' personal information and causes potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
%
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} may cause serious personal information leakage. 
%
For example, a recent report~\cite{cybernews_dataleakage} discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties. 
%
Zhang et al.~\cite{zhang2020does} disclose 120 of 555 apps that share users' personal information to analytic service TPLs without encryption. 
%
Besides, linking and mining large amounts of unencrypted personal information probably pose threats to serious personal privacy leakage~\cite{kiranmayi2018reducing, chen2014information}.
%
Thus, it is urgent to design a system to check the data access behavior and privacy policies of TPLs so that we can determine if TPLs are compliant with privacy regulations.
%or not.


% To normalize apps' behaviors and prevent privacy leakage, various personal privacy  protection-related regulations (e.g., CCPA, CPRA, GDPR, ICCPR)~\cite{piss, zhSDKLaw, gdpr, ccpa} have been promulgated to protect people's personal information from abuse, which requires developers to clearly understand TPL behaviors and declare these sensitive behaviors in their privacy policy so as not to violate the regulations.
%
To normalize privacy-related behaviors and prevent privacy leakage, various privacy-related regulations 
% (e.g., CCPA, CPRA, GDPR, ICCPR, CFR)~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr}
(e.g., {\textsc{\small{California Consumer Privacy Act (CCPA), General Data Protection Regulation (GDPR)}}})~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr})
have been promulgated to protect people's personal information from being abused.
%
However, app developers may unconsciously violate regulations of used TPLs because they do not need to understand the execution logic of these TPLs, they just need to follow the user guidelines to invoke these TPLs. Due to a lack of security consciousness, developers may never check whether these used TPLs in their apps have a privacy policy and whether these TPLs may have security risks with respect to privacy leakage. 
% }
%
The latest \textit{\small{Google Play Developer Program policies (GPDP)}}~\cite{google_play_pp_update} asks developers to ensure the TPLs used in their apps are compliant with GPDP~\cite{gpdp}.
%
Developers of {\tpl}s are required to provide privacy policies and disclose data usage.
%
Otherwise, apps may violate regulation or market's requirements and be removed from the app market~\cite{googleplay_requirements, appgallery_requirements}.
%
To help TPLs comply with regulations and help developers correctly use TPLs,  it is necessary to analyze the consistency between {\tpl}s' data usage and privacy policies.


Previous work~\cite{ppcheck,ppchecker,andow2019policylint, yu2016can,nguyen2021share,zhang2020does,wang2021understanding} has proposed methods to analyze privacy issues of apps, such as analyzing the consistency between apps' privacy policy descriptions and behaviors.
%
However, existing methods cannot identify the app's privacy issues related to the usage of TPLs inside apps because existing methods fail to identify TPLs functionalities or analyze TPL privacy policies.
%
PoliCheck~\cite{ppcheck} performs dynamic analysis to get traffic flow for analyzing the apps' data usage.
Then, it applies data and entity dependency tree analysis to extract data usage statements from the privacy policy, and designs rules to identify the conflicts.
%
PPChecker~\cite{ppchecker} discovers the trustworthiness of apps' privacy policies, and identifies consistency of app's behavior and privacy policy statements and the consistency of privacy policies from different sources.
%
PPChecker concentrates on apps' privacy policies and is out-of-dated to satisfy the latest regulations.


Based on our study, we find there is still a research gap with respect to discrepancy analysis between the privacy-related behaviors of TPLs and regulations.
%
To this end, we propose a tool, named \oursystem ~(\underline{\textbf{A}}utomated \underline{\textbf{T}}hird-party library \underline{\textbf{P}}rivacy compliance \underline{\textbf{Checker}}) to automatically check whether the usages of in-app TPLs complies with privacy-related regulations (e.g., {GDPR Article I.(47), COPPA 312.2, CFR 332.6}).
%
As regulation analysis requires expert knowledge of both legal and software engineering, we invited 
one expert and one senior researcher to read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. 
%
Both of them have conducted research on software engineering and privacy policy analysis with experience over seven years and two years, respectively.
% 
{\oursystem} identifies the inconsistency between TPL and regulation by analyzing TPL's bytecode (\S\ref{sec:tpl_data}) and privacy policies (\S\ref{sec:tpl_pp}).
% 
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
% 
{\oursystem} discloses whether host app's TPL usage comply with regulations(\S\ref{sec:host_app_data}, \S\ref{sec:host_app_pp}). 





\kaifa{
It remains challenging to develop {\oursystem}. % due to multiple reasons.
%
First, it is non-trivial to get TPLs and corresponding privacy policies because TPLs are mainly published on 
% open source 
repositories, such as Maven Repository~\cite{mvnrepository} and GitHub, which do not require developers to provide privacy policies to describe their user privacy access behaviors.
%
To counter this issue, we first construct a data set that contains TPL repository and host app repository.
%
The TPL repository contains a) a TPL list, which contains 458 TPLs crawled from {\appbrain}~\cite{appbrain},  b) 187 TPL's binary files from {\maven}~\cite{mvnrepository}, and c) 351 TPL's privacy policies which are manually collected. The details of dataset components and relations are given  in \S\ref{sec:eva}. 
%
The host app repository contains a) 642 distinct host apps which are collected from {Google Play} based on the list from {\appbrain} and b) the host app's privacy policies.
%
Second, it is not easy to analyze TPL's user privacy access behavior because TPLs are mainly provided in the format of binary files, such as \textit{jar} and \textit{aar} in {\maven}, without source code and TPL's whole functions may not be executed independently without being triggered by host apps.
%
{\oursystem} performs static analysis~\cite{soot} to construct the TPL's function call graph and uses data flow analysis to trace TPLs personal information usage without source code (\S\ref{sec:tpl_data}).
% 
We exclude dynamic analysis since it cannot execute all possible paths in apps or TPLs~\cite{schindler2022privacy}.
%
Third, analyzing privacy policy is difficult because developers use various natural languages to describe the usage of personal information and TPLs.
%
To analyze data and TPL usage-related statements of privacy policies, {\oursystem} implements an expert system to extract abstract data usage patterns (\S\ref{sec:host_app_pp}) and analyzes TPL usage compliance.
}


Overall, our contributions are summarized as follows:


\begin{itemize}[leftmargin=*]


\item We propose a novel system named {\oursystem} to analyze the compliance of Android TPLs. 
%
{\oursystem} uses static analysis to identify TPL's user data access behaviors and host apps' data interaction with TPLs, and uses  NLP techniques to analyze TPLs' and host apps' privacy policies.
% TPLs' personal information accessing both individually and inside host apps, and applies NLP techniques to analyze TPLs' and host apps' privacy policies.
%
Combining the results of bytecode analysis and privacy policy analysis, {\oursystem} determines whether TPLs and usage of TPLs in host apps comply with regulation. 


\item To evaluate the performance of {\oursystem} and facilitate further research in this area, we construct a privacy dataset that includes 187 TPL's binary files and their privacy policies, and 642 host apps and their privacy policies.
% 
Our dataset contains TPL's privacy policies with related data access behavior.
%
Our dataset includes host app's privacy policies that contain labels related to host app's interaction with TPLs.
% TPL's privacy policies in our data set contain labeled corpus related to TPLs' data accessing behavior and the host app's privacy policies are labeled with used TPLs and data interaction with TPLs.
%
{\oursystem}'s website with instructions to request access is at:
%\url{https://github.com/zacharykzhao/TPL-PP}.
\url{https://atpchecker.github.io}.
% 

% \vspace{1em}
\item {\oursystem} discovers over 23\% of TPLs miss providing privacy policies and 37\% of TPL's privacy policies conceal data usage.
%
{\oursystem} finds over 65\% of host apps violate the regulation requirements for clearly disclosing data interactions with TPLs. 



\end{itemize}


==> tmp/Introduction_n.tex <==
\section{Introduction}

\input{table/regulation_summary}


Personal data protection-related regulations have been promulgated worldwide to protect people's personal information from misuse since 2020 (Table~\ref{tab:regulation}). 
%
However, there still exist popular Android apps with over 142.5 million installations lead to user data leakages that violate regulation requirements~\cite{cybernews_dataleakage}.
%
Some of those user data leakages are caused by the mis-configuration of third-party libraries ({\tpl}s)~\cite{zhang2020does, harty2021logging}. This report~\cite{cpr_mis_tpl} disclosed that developers' mis-configuration of third-party services causes over 100 million personal information leakage.
%
For example, apps directly use users' personally identifiable information (e.g., email) as a user ID to submit to TP Ls without configuring any anonymization or encryption~\cite{zhang2020does}
%












% \kaifa{rewritten as latest paragraph}
% \revise{As {\tpl}s are generally sets of methods, if we use dynamic analysis, we must find a host app that invokes all methods in the TPL and dynamically trigger all of those methods to analyze the data usage inside.}\xiancm{incorrect}
% %
% As 100\% dynamic trigger coverage is an open question~\cite{afianian2019malware},
% % and finding a satisfied host app \revise{can be regarded as a chicken-and-egg conundrum,}\xiancm{why I do not know} 
% {\oursystem} is constructed based on static analysis.
% %
% \revise{Static analysis needs to find or construct a main method or entry points to analyze the whole program.} \xiancm{totally wrong!!!! incorrect, I do not know where you see this. how about extract the opcode, APIs, there are also belonging to static analysis}
% %
% \revise{While TPLs are generally sets of separate methods or functionalities for convenient invocation, {\oursystem} designs new methods to construct entry points for each TPLs (\S~\ref{sec:tpl_data}) and uses data flow analysis to extract the all data usage in {\tpl}s.}
% \xiancm{incorrect, my paper and libd never say that, how it come?}

==> tmp/abs_0105.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}



The privacy of personal information has received significant attention in mobile software.
%
Although previous researchers have designed methods to identify the conflict between app behavior and privacy policies, little is known about investigating regulation requirements for third-party libraries (TPLs).
%
The regulators enacted articles to regulate the usage of personal information for TPLs (e.g., the 
% \textsc{{California Consumer Privacy Act}} 
CCPA requires businesses clearly notify consumers if they share consumers' data with third parties or not).
% 
However, it remains challenging to analyze the legality of TPLs due to three reasons:
%
1) Difficulties in collecting TPLs privacy policies. 
%
TPLs are mainly published on public repositories (e.g., Maven Repository, GitHub). % instead of app market (e.g., Google play). 
%
The repositories do not require providing privacy policies to describe artifacts' privacy access behaviors. 
%
Thus, there is no unique channel, like Google Play, to collect privacy policies of TPLs. 
2) Difficulties in analyzing TPL's user privacy access behaviors.
% and host app's privacy data interaction with TPLs.
%
TPLs are mainly provided in binary files, such as \textit{jar} or \textit{aar}, and TPL's whole functionalities are usually not executed independently without host apps.
%
3) Difficulties in identifying consistency between TPL's functionalities and privacy policies, and host app's privacy policy and data sharing with TPLs.
%
This not only requires analyzing privacy policies of TPLs and host apps, but also requires analyzing their functionalities.
% of host apps and TPLs.
%
% To overcome the above challenges, 
In this paper, we propose an automated system named {\oursystem} to analyze whether Android TPLs comply with the privacy-related regulations.
% or not.
%
We construct a data set that contains a list of 458 TPLs, 351 TPL's privacy policies, 187 TPL's binary files
% in format of jar or aar 
and 642 host apps and their privacy policies. 
%
Then, we analyze the bytecode of TPLs and host apps, design natural language processing systems to analyze privacy policies, and implement an expert system to identify TPL usage-related regulation compliance.
%
The experimental results show that 23\% TPLs violate regulation requirements for providing privacy policies. 
%
Over 37\% TPLs miss disclosing data usage in their privacy policies. 
Over 52\% host apps share user data with TPLs while 65\% of them miss disclosing interactions with TPLs.
%
Our findings remind developers to be mindful of TPL usage when developing apps or writing privacy policies to avoid violating regulations.




\begin{comment}


The privacy of personal information has received significant attention in mobile software.
%
Although previous researchers have designed some methods to identify the conflict between app behavior and privacy policies, little is known about investigating regulation requirements for third-party libraries (TPLs).
%
%Regulations enact Articles 
The regulators enacted multiple regulations to regulate the usage of personal information for TPLs (e.g., the \textsc{{California Consumer Privacy Act}} requires businesses clearly notify consumers if they share consumers' data with third parties or not).
% 
% However, the challenges of TPL's regulation complaints analysis mainly from three aspects: 
However, it remains challenging to analyze the legality of TPLs due to three reasons:
%
1) %Publication channel of TPLs. \revise{TPLs are mainly published on public repositories (e.g., Maven) instead of app market (e.g., Google play).}\xiancm{I think this description is not accurate, and should delete. 1. there are many open-source TPLs and also some private TPLs, closed-sourced TPls, TPLs can be written in different languages, for C TPLs, there is not a package manager for them,i.e., the public repo, so this sentence is not accurate. The package manager repo just for some TPLs (java, python, js XX not for C/C++).} 
% The public repositories do not perform privacy compliance analysis for each TPL. 
% \xiancm{This is status quo is not the challenges, you should add more description to say this situations but it is still a status quo, you should give effects about that, e.g., The privacy policy is not mandatory for many public repositories, therefore, many TPLs' developers did not offer the PP even some of them already use some sensitive date of users.}
\kaifa{
1) Difficulties in collecting TPLs privacy policies. 
%
TPLs are mainly published on public repositories (e.g., Maven, github) instead of app market (e.g., Google play). 
%
The repositories do not require providing privacy policies to describe code's privacy access behaviors.
%
Thus, there is no unique channel to collect privacy policy of TPLs.
}
2) %Independence of TPLs.
TPLs only provide independent functions or function sequences.
They cannot run independently, which limits the application of performing dynamic analysis.  
% \xiancm{even some TPLs cannot run independently but we still can conduct dynamic analysis for these TPLs, some TPLs even can run independently}
3) %Identification of privacy related functions of TPLs. 
Since not all the functions of TPLs are related to users' privacy, we must locate the functions of TPLs that access/process personal information before performing privacy compliance analysis. 
% \xiancm{I think only two challenges is reasonable. this one and the following one you have commented. 1. not all functionalities are related privacy usage, 2. not all functions can be invoked}
% \xiancm{above mentioned challenges should delete some is not the challenges some is not accurate}
% 3) Usage of TPLs in host apps. Host apps may not use all the functions of TPLs. 
% We need to locate the specific function of TPL to identify the complaints of privacy policies. 
%
To overcome the above challenges, in this paper, we propose an automated system named {\oursystem} to analyze whether the Android TPLs meet the privacy related regulations or not.
%to analyze the Android TPL-related regulation complaints.
%
% Specifically, we design {\oursystem} to analyze whether TPLs satisfy the requirements by analyzing the TPLs' privacy policies and functionalities and host apps' privacy policies, and host apps' usage of TPLs.
% First, 
We construct a data set that contains 458 TPLs and 642 host apps.
The privacy policies of 187 TPLs are collected and they are annotated with corpus labels.
The privacy policies of all host apps are collected and 256 of them are manually annotated.
%
Then, we analyze the bytecode of TPLs and host apps, design natural language processing systems to analyze privacy policies, and implement an expert system to identify the TPL usage related regulation complaints.
% First, {\oursystem} constructs a data set that contains 458 TPLs,  197 TPLs' privacy policies with corpus labels, 642 host apps with corresponding privacy policies and 256 host apps' privacy policies are manually labeled.
The experimental results show that 23\% TPLs violate regulation requirements for providing privacy policies. 
%{\oursystem} analyzes TPLs and host apps binary files, designs natural language processing systems to analyze privacy policies, and implements expert system to identify the regulation complaints related to TPL usage. {\oursystem} identifies 
Over 37\% TPLs miss disclosing data usage in their privacy policies. 
Over 60\% host apps share user data with TPLs while 65\% of those host apps miss disclosing interactions with TPLs.
%
Our findings remind developers to be mindful of TPL usage when developing apps or writing privacy policies to avoid violating regulations.
%
% {\oursystem} identifies 107 out of 458 TPLs violate the regulation requirements to provide privacy policies and 37\% of TPLs' privacy policies conceal their data usage.
% %
% Besides, {\oursystem} also discovers that 65\% host apps violate the regulation requirements for disclosure of their data interaction with TPLs.
\end{comment}

\end{abstract}

==> tmp/bchabs.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}


The privacy of personal information has received significant attention in mobile software.
%
Although previous researchers have designed some methods to identify the conflict between app behavior and privacy policies, little is known about investigating regulation requirements for third-party libraries (TPLs).
%
%Regulations enact Articles 
The regulators enacted multiple regulations to regulate the usage of personal information for TPLs (e.g., the \textsc{{California Consumer Privacy Act}} requires businesses clearly notify consumers if they share consumers' data with third parties or not).
% 
% However, the challenges of TPL's regulation complaints analysis mainly from three aspects: 
However, it remains challenging to analyze the legality of TPLs due to three reasons:
%
1) %Publication channel of TPLs. 
\revise{TPLs are mainly published on public repositories (e.g., Maven) instead of app market (e.g., Google play).}\xiancm{I think this description is not accurate, and should delete. 1. there are many open-source TPLs and also some private TPLs, closed-sourced TPls, TPLs can be written in different languages, for C TPLs, there is not a package manager for them,i.e., the public repo, so this sentence is not accurate. The package manager repo just for some TPLs (java, python, js XX not for C/C++).} The public repositories do not perform privacy compliance analysis for each TPL. \xiancm{This is status quo is not the challenges, you should add more description to say this situations but it is still a status quo, you should give effects about that, e.g., The privacy policy is not mandatory for many public repositories, therefore, many TPLs' developers did not offer the PP even some of them already use some sensitive date of users.}
2) %Independence of TPLs.
TPLs only provide independent functions or function sequences.\xiancm{I think this description is not accurate} They cannot run independently, which limits the application of performing dynamic analysis.  \xiancm{even some TPLs cannot run independently but we still can conduct dynamic analysis for these TPLs, some TPLs even can run independently}
3) %Identification of privacy related functions of TPLs. 
Since not all the functions of TPLs are related to users' privacy, we must locate the functions of TPLs that access/process personal information before performing privacy compliance analysis. \xiancm{I think only two challenges is reasonable. this one and the following one you have commented. 1. not all functionalities are related privacy usage, 2. not all functions can be invoked}
\xiancm{above mentioned challenges should delete some is not the challenges some is not accurate}
% 3) Usage of TPLs in host apps. Host apps may not use all the functions of TPLs. 
% We need to locate the specific function of TPL to identify the complaints of privacy policies. 
%
To overcome the above challenges, in this paper, we propose an automated system named {\oursystem} to analyze whether the Android TPLs meet the privacy related regulations or not.
%to analyze the Android TPL-related regulation complaints.
%
% Specifically, we design {\oursystem} to analyze whether TPLs satisfy the requirements by analyzing the TPLs' privacy policies and functionalities and host apps' privacy policies, and host apps' usage of TPLs.
% First, 
We construct a data set that contains 458 TPLs and 642 host apps.
The privacy policies of 187 TPLs are collected and they are annotated with corpus labels.
The privacy policies of all host apps are collected and 256 of them are manually annotated.
\xiancm{I do not understand the relationship between the 458 TPLs and 642 apps and the 187 TPLs and 256 apps. the 187 TPls belongs to the 458 TPLs? and 642 apps include the 256? if yes, We should add among the dataset, the privacy policies of 187 TPLs are collected and they are annotated with corpus labels XXX ... Besides, it is too dangerous, cannot match the data in introduction, why? }
Then, we analyze the bytecode of TPLs and host apps, design natural language processing systems to analyze privacy policies, and implement an expert system to identify the TPL usage related regulation complaints.
% First, {\oursystem} constructs a data set that contains 458 TPLs,  197 TPLs' privacy policies with corpus labels, 642 host apps with corresponding privacy policies and 256 host apps' privacy policies are manually labeled.
The experimental results show that 23\% \xiancm{can we give a ratio here? XX/XX, /187 or /458, the results are misleading} TPLs violate regulation requirements for providing privacy policies. 
%{\oursystem} analyzes TPLs and host apps binary code, designs natural language processing systems to analyze privacy policies, and implements expert system to identify the regulation complaints related to TPL usage. {\oursystem} identifies 
Over 37\%\revise{XX/XX} TPLs miss disclosing data usage in their privacy policies. \xiancm{the same issues of the proportion}
Over 60\% \revise{XX/XX}host apps share user data with TPLs while 65\% of those host apps miss disclosing interactions with TPLs.
%
Our findings remind developers to be mindful of TPL usage when developing apps or writing privacy policies to avoid violating regulations.
%
% {\oursystem} identifies 107 out of 458 TPLs violate the regulation requirements to provide privacy policies and 37\% of TPLs' privacy policies conceal their data usage.
% %
% Besides, {\oursystem} also discovers that 65\% host apps violate the regulation requirements for disclosure of their data interaction with TPLs.



\end{abstract}

==> tmp/exp_0105.tex <==
\section{Evaluation}
\label{sec:eva}
% \subsection{Dataset Collection and Experimental Setup}
\label{sec:dataset}




We evaluate the performance of {\oursystem} by answering the following research questions:

\noindent\textbf{RQ1: Normativeness Analysis of TPLs.} 
%
\textit{How many TPLs provide privacy policy documents?} 
%
 

\noindent\textbf{RQ2: Legality Analysis of TPLs.}  
%
\textit{Do TPLs’ privacy policies meet regulation requirements, and do TPLs’ privacy policies correctly claim data usage actions?}

%
\noindent\textbf{RQ3: Host {\app}s behavior analysis.} \textit{Whether do host {\app}s conduct privacy data interaction with TPLs?}

%
\noindent\textbf{RQ4: Legality of host app's privacy policies.} 
\textit{Whether do host app's privacy policies comply with  requirements for disclosure of TPL usage?}




\input{table/TPL_without_PP_list}

\subsection{RQ1: Normativeness Analysis of TPLs.}
\label{sec:rq1}


\noindent\textbf{Experimental Setup.}
This research question evaluates all Android TPLs listed in AppBrain~\cite{appbrain} including three types: Ad networks, social libraries, and development tools.
%
The list gives the TPLs that are widely used by top 500 installed apps in Google Play. 
%
The data set contains 458 TPLs that include 141 ad networks, 25 social libraries, and 292 development tools.
%
Then, we gather the privacy policies of those TPLs by visiting the homepage provided by each TPL information page on AppBrain.
%
We manually crawl information of TPLs whose homepages are not provided. 
%
For open-source TPLs in Github or Bitbucket, we visit their public repositories and check whether privacy policies are provided.
%
During visiting the homepage of TPLs, we search the homepage with keywords, such as \textit{privacy, policy, legal} and \textit{policies}, to find potential privacy policy links on the homepage. 
%
Besides, we also manually check whether policy links are given in the typical layout ~\cite{harkous2018polisis}, such as the bottom of the website.
%
Finally, we collect 201 unique privacy policies as some TPLs are built by the same companies or developers.



\noindent\textbf{Results.}
%
According to regulation requirements (\S\ref{sec:bb_regulation_req}), data controllers should clearly disclose their data usage in privacy policies.
%
This research question discloses whether TPLs satisfy the requirements of regulations, i.e., do TPLs correctly provide privacy policies.
%
With the TPL list and  privacy policies, {\oursystem} discovers that 2 of 141 Ad network TPLs, 2 of 25 social libraries, and 103 of 292 development tools TPLs do not provide privacy policy websites. 
%
We find that some TPLs are created by individual developers and released on {\github}~\cite{github}.
%
We manually crawl their privacy policies for {\github} repositories.
%
Tab.~\ref{tab:tpl_no_pp} summarizes partial TPL names and the reasons that the TPLs do not provide privacy policies.
%
Tab.~\ref{tab:tpl_no_pp} demonstrates that 16 of 22 TPLs that do not provide privacy policies are published as Github repositories (GNP).
%
Five TPLs without privacy policies miss official websites (NOS), and the left does not provide privacy policy documents on their websites (NPOS).
%
For development tool TPLs, we also observe that 66 TPLs from \textit{Google Inc.} share the same privacy policy~\cite{googlepp} that may lead to over-claiming the personal information usage for specific TPLs.
%
For nine TPLs from \textit{Apache}, six TPLs (6/9) do not provide privacy policies and two TPLs' (2/9) websites are Not Found.



\answer{1}{
{\oursystem} reveals  23\% TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
}



% \answer{1}{
% {\oursystem} finds that 6\% English TPLs and 11\% Chinese TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
% }






\begin{figure}[t]
    \centering
    \vspace{-1ex}
    \includegraphics[width=0.4\textwidth]{figures/FCG_compare.pdf}
    \vspace{-1.5ex}
    \caption{Evaluation of function call graph construction.}
    % \vspace{-2ex}
    \label{fig:fcg_compare}
\end{figure}


\subsection{RQ2: Legality Analysis of TPLs.}


\noindent\textbf{Experimental Setup.}
We collect the resources of TPLs from Maven Repository~\cite{mvnrepository} based on the TPL list from AppBrain (\S\ref{sec:rq1}).
%
We manually crawl TPL binary files from Maven Repository by searching the TPL's name in Appbrain's list and finally get 187 different TPLs including 85 "aar" and 102 "jar" files.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Results.}
%
{\oursystem} discloses whether the TPLs' privacy policies satisfy the regulation requirements by comparing TPLs' binary files analysis results (\S\ref{sec:tpl_data}) and privacy policies analysis results (\S~\ref{sec:tpl_pp}).
%
{\oursystem} analyzes TPLs' privacy policies and obtains the ADUP of personal information usage-related statements.
%
{\oursystem} identifies personal information in the TPL through static analysis (\S\ref{sec:tpl_data}).
%
Finally, {\oursystem} matches the consistency between AUDP and personal information.



% \begin{figure}[t]
%     \centering
%     \vspace{1ex}
%     \includegraphics[width=0.47\textwidth]{figures/TPL_PP_data_freq.pdf}
%     % \vspace{1ex}

%     \caption{Popularity of data types that are most mentioned in TPLs' PP}
%     % \vspace{-2ex}
%     \label{fig:tpl_pp_data_freq}
% \end{figure}




\noindent{\small{\textit{\textbf{TPL privacy policies analysis.}}}}
%
{\oursystem} analyzes privacy policy documents of 187 TPL whose binary files and privacy policies are both available.
%
We analyze 42,895 sentences with sharing and collection (SAC) words, and each privacy policy has an average of 420.5 sentences and 136 SAC words.
%
Among sentences with SAC words, 19,750 sentences start with 5W1H (who, why, when, whether, what, how) words that are considered as data usage actions.
%
Besides, 1,654 sentences only vaguely state that the TPL will collect personal information without specific data types.
%
For example, $com.xiledsystems$  only claims \textit{``We collect your personal information in order to provide and continually improve our products and services,"} but no specific personal information is given.
%
In data usage-related actions, {\oursystem} analyzes the personal information that is mostly used by TPLs.
%
Fig.~\ref{fig:tpl_data_freq} shows the times that are mentioned in TPLs' privacy policies.
%23
It can be observed that \texttt{contact} are the most  used personal information.
%
This may be  caused by the fact that, by getting contact, the TPLs can easily expand and prompt their services.
%
Account, address and email are the second most popular data mentioned in TPLs' privacy policies.
%
Among the statements that claim to collect  accounts, addresses, and email, 21.13\% of sentences claim that they collect related data for contacting users. 
%
For example, one of them claims that \textit{``we will use your email, phone number, or other contact information you provide us by written or oral means for contacting you and providing you with the services and information that             you request"}.









\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/TPL_PP_data_freq.pdf}
    % \vspace{1ex}

    \caption{Popularity of data types that are used in TPLs' data flow and PP.}
    \vspace{-1ex}
    \label{fig:tpl_data_freq}
\end{figure}


\vspace{1ex}
\noindent{\small{\textit{\textbf{TPL data usage analysis.}}}}
%% analyze whether our fcg construction method effective/improved
As the basis of data flow analysis, we first evaluate the effectiveness of {\oursystem} in improving the FCG construction performance.
%34
We analyze TPLs' FCG quality through comparing the a) FCG coverage and b) the number of edges between the raw FCG built by soot and our optimized FCG.
%
FCG coverage is calculated by:
%FCG coverage : the number of nodes in FCG/ the number of methods 
\begin{equation}
    \label{eq:fcg_cov}
    cov_{FCG} = \frac{\#Nodes_{FCG}}{\#Nodes_{TPL}},
\end{equation}
where {\smaller{$\#Nodes_{FCG}$}} is the number of nodes (methods) in FCG and {\smaller{$\#Nodes_{TPL}$}} is the total number of TPLs' methods.
%
Fig.~\ref{fig:fcg_compare} illustrates the box plots of {\oursystem}'s performance in  optimizing  FCG construction, and the number at the top of boxes denotes measuring units of the data for better illustration.
%
Fig.~\ref{fig:fcg_compare} demonstrates that {\oursystem}'s FCG coverage achieves an average performance of 55\%, while the FCG coverage of raw FCG only achieves an average of 0.34\%, which  means it nearly fails to construct the FCG of TPLS.
%
{\smaller{$raw_{\#edge}$}} denotes the raw FCG only contains the 159 average edges, while the {\smaller{${\oursystem}_{\#edge}$}} shows the improved FCG can extract 12,960 edges.
%
The results indicate that the soot nearly fails to analyze the FCG of TPLs, and {\oursystem} optimizes construction performance and improves the FCG quality.



% Then, 
{\oursystem} analyzes the data usage of TPLs to identify the consistency with their privacy policy statements.
%
{\oursystem} analyzes the data flow of TPLs and discovers that 65 out of 187 TPLs access users' personal information.
%
{\oursystem} identifies 146 data usage from 2,396 traces.
%
Among data usage behavior, 31 out of 146 invokes Android APIs (such as \textit{``android.telephony.TelephonyManager: java.lang.String getSimSerialNumber()"}) to access Android \texttt{Sim Serial number}.
%
Fig.~\ref{fig:tpl_data_freq} shows the data frequencies that are mostly used in TPLs' data flow (shown in orange color).
%
It can also be observed that TPLs' privacy policies tend to disclose non-identical information, such as \texttt{contact}, while their actions tend to access identical information. 

 
\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.43\textwidth]{figures/tpl_propa.pdf}
    % \vspace{1ex}

    \caption{TPL Privacy Policy Non-compliance Propagation. The first column is raw TPLs identified by ATPChecker that potentially violate regulation requirements. The second column is TPLs affected by raw TPLs and the number above the arrow is the number of TPLs infected by raw TPLs. The third column is TPLs affected by the TPLs in the second column.}
    % \vspace{-2ex}
    \label{fig:tpl_pp_dep}

\end{figure}

% \begin{comment}


{\oursystem} identifies the compliance of TPLs by combing the privacy policies analysis results and data flow analysis results.
% 
Specifically, {\oursystem} identifies how many TPLs comply with regulations by identifying whether the PI in data flow is also mentioned in ADUP. 
%
{\oursystem} concentrates on 65 TPLs that access users' personal information identified by {\oursystem} and discovers that 24 out of 65 (37\%) TPLs violate the regulation requirements, i.e., the TPLs collect at least one PI without clearly disclosing them in privacy policies.  





% \vspace{1ex}
\noindent{\small{\textit{\textbf{Investigation on perniciousness of TPLs' non-compliant behavior.}}}}
%
After identifying TPLs that do not satisfy the regulation requirements, we also identify the  harm of TPLs' non-compliant behavior on a large scale.
%
% It is well known that 
TPLs may integrate other TPLs to enhance their functionalities or facilitate usability~\cite{atvhunter2021ICSE}.
%
Thus, once one TPL ($TPL_v$) violates the regulation, other artifacts integrated $TPL_v$ may spread the threats and make their privacy policies violate regulation requirements.
%
To expose the impacts, {\oursystem} analyzes the dependencies among TPLs. 
%
Specifically, {\oursystem} crawls the TPLs ($TPL_U$) that use $TPL_v$, that are analyzed in \S\ref{sec:tpl_data}-\ref{sec:tpl_pp}, from {\maven}.
%
Then starting from $TPL_U$, {\oursystem} crawls the list of artifacts that use $TPL_U$.
%
In this way, {\oursystem} investigates the propagation of $TPL_v$'s threats under two times integration and visualizes it in Fig.~\ref{fig:tpl_pp_dep}.
%
{\oursystem} starts analysis with 25 unconventional TPLs.
%
Fig.~\ref{fig:tpl_pp_dep} demonstrates the harm of that privacy policy inconsistency  propagation with five selected TPLs.  
%
It can be observed that after one round of propagation, even five TPLs will affect 24,737 TPLs (25 TPLs affects extra 79,471 TPLs). After two rounds of propagation, the threats even spread to 18,323 TPLs (25 to 447,300).
%
Fig.~\ref{fig:tpl_pp_dep} also demonstrates that not only the popular TPLs demonstrate infective (be widely used by other TPLs), such as \textit{``common-io/commons-io"}, 
% 
some minority TPLs, such as \textit{``com.google.gdata/gdata-clien"} are directly used by only 11 TPLs.
%
After two rounds of propagation, the number of TPLs they affect increases exponentially.
%
This observation indicates that developers should pay attention to the usage data of TPLs, especially the functions that are related to privacy.



\answer{2}{
{\oursystem} identifies over 37\% TPLs miss disclosing their data usage in privacy policy documents.
%
{\oursystem} investigates that the perniciousness of privacy policy non-compliance harms spread exponentially.
}


\subsection{RQ3: Analysis of host apps' interaction with TPLs}
\label{sec:rq3}

\noindent\textbf{Experimental Setup.}
%
We collect the host apps of TPLs from AppBrain to investigate host apps' interaction with TPLs.
%
We gather the host app list using the mapping relations between host apps and used in-app TPLs provided in AppBrain.
%
We can access the top ten installation host app list for each TPL and then download the apps.
%
Finally, we gather a total of 642 distinct apps because some apps may use multiple TPLs and one TPL can be used by different apps.
%
% \kaifa{
% We evaluate {\oursystem} on apks whose size is smaller than 100MB due to the limited memory capacity.
% % because flowdroid's capacity~\cite{arzt2014flowdroid} will be limited for analyzing large apks.
% }




\begin{figure}[t]
    \centering
   %  \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/host_app_interaction_1214.pdf}
    \vspace{-1ex}
    \caption{Statistics of host apps' data interaction with TPLs.}
    % \vspace{-2ex}
    \label{fig:app_int_tpl}
\end{figure}



\noindent\textbf{Results.}
{\oursystem} uses data flow analysis to investigate whether host apps conduct personal information interaction with TPLs and what kinds of PI are shared with TPLs.
%
{\oursystem} analyzes 642 distinct apps. % with labels, i.e., which TPLs are used.
%
However, limited to computation resources and flowdroid's capacity, we finally successfully analyzed 354 apps while 174 out of 642 apps are in the form of ".xapk"~\cite{apkpure} which cannot be analyzed by flowdroid and 114 out of 642 apps cannot be analyzed because some apps apply protection methods and some apps are too large which exhaust our computation resources.
%
{\oursystem} identifies over 52.8\% (187 out of 354) host apps share PI with TPLs.
% and as is illustrated in Fig.~\ref{fig:app_int_tpl}.
%
{\oursystem} measures the suspicious behavior by counting the times of PI-related invocations in apps' data flow and traces 2,216 times data-sharing behaviors with TPLs and finds that over 53.1\% traces share users' \textit{sim serial number} with TPLs such as \textit{``Google Analytics"}.
%
Although \textit{``Google Analytics"} is a well know TPL that provides users abundant Google services, the sharing of \textit{sim serial number} is sensitive to identify one individual.
%
Fig.~\ref{fig:app_int_tpl} shows the top five data shared by host apps with TPLs.
% 
Fig.~\ref{fig:app_int_tpl} shows that the secondary data the host app need to share with TPLs is network status, as TPLs may connect the server to provide services, like advertising or data analytics.
%
{\oursystem} also observes that \textit{``Google Analytics"} is the TPL that accesses the most PI from host apps.
%
Although \textit{``Google Analytics"} provides abundant functionalities, such as gmail and music, TPLs should avoid collecting information like SIM serial number that is easy to identify an individual and provide privacy policies to state the purpose of data access.
%
TPLs should not ask for unnecessary data which out of the scope of their services~\cite{zhSDKLaw,gdpr,ccpa,piss}.
% more data than is required for the content of their services~\cite{zhSDKLaw,gdpr,ccpa,piss}.




\answer{3}{
{\oursystem} identifies that over 52.8\% of host apps share personal information with TPLs.
%
Among shared PI, sim serial number accounts for over 53.1\%  of traces in identified user data access actions.
%
{\oursystem} also discovers that while well-known TPLs provide rich functionalities, they also request personal information.
}





\subsection{RQ4: Host apps privacy policy analysis.}
\label{exp:host_app_pp}


\noindent\textbf{Experimental Settings.}
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior is consistent with the privacy policies.
% and violate the regulation requirements or not. 
%
For each host app in our dataset, we  get its privacy policy by crawling the homepage from Google Play.
%
To evaluate the performance of {\oursystem}, we collect extra 256 apps and corresponding privacy policies. 
%
Then, one expert and one senior researcher in software engineering and privacy policy analysis manually label the privacy policies. 
% to evaluate the performance of {\oursystem}. 

\begin{comment}
    
\begin{figure}[t]
    \centering
    %\vspace{-2ex}
    \includegraphics[width=0.42\textwidth]{figures/mssing_TPL.pdf}
    % \vspace{-2.5ex}
    % \caption{Statistics of missing TPLs in host apps' PP.}
    \caption{Percentage of the TPLs not mentioned in host apps’ PP}
    \vspace{-0.5ex}
    \label{fig:miss_tpl}
\end{figure}
\end{comment}

\noindent\textbf{Results.}
{\oursystem} identifies whether host apps' privacy policies comply with regulation requirements concerning descriptions about TPLs by analyzing whether privacy policies disclosure their usage and interaction with TPLs.
%
{\oursystem} implements this 
% by discovering the problems of privacy policy descriptions concerning TPL usage
by combining the static analysis results (\S\ref{sec:rq3}) and privacy policy analysis results.
%
{\oursystem} identifies 
a) whether apps integrate TPLs in their code without disclosure in privacy policies and 
b) whether TPLs access sensitive PI without descriptions.
%
We collect extra 256 apps to annotate the privacy policies and evaluate the identification performance.
%
To annotate the privacy policies, one expert and senior researcher, who have conducted research on privacy policy and software engineering for over seven years and two years respectively, manually label the sentences that include data usage, TPL usage, and data interaction wit TPLs.
%
The annotation process is conducted in an in-house manner~\cite{sorokin2008utility,zhao22ca4p} that guarantees the quality and agreement of the labels.
% Then, we manually labeled privacy policies that include the data usage, TPL usage and data interaction with TPLs.
%


{\oursystem} identifies 65.63\% (168/256) apps violating the regulation requirements, i.e., their privacy policies miss disclosing TPL usage in their privacy policies.
%
% Fig.~\ref{fig:miss_tpl} shows the most popular 17 TPLs that are missed being disclosed by host apps.
%
{\oursystem} identifies over 25\% privacy policy's user data access conceal behavior is related to the TPL, i.e.,  ``{\small{Alipay SDK Java}}".
% (``{\small{Alipay SDK Java}}".). 
%
This may lie in the fact host apps only use the TPL for payment and do not use the TPL for user data access behavior. 
%
Even so, host apps are still required to claim TPL usage in their privacy policies~\cite{zhSDKLaw}.
%
Among concealed data interaction with TPLs, the most popular PI data, that the app interacts with TPL but not discloses in the PP, are \textit{device ID}, \textit{mac address}, and \textit{sim serial number}, which account for 95.82\% (321/335) conflicts.







To this end, we also evaluate the performance of {\oursystem}.
%
We evaluate the eight metrics (i.e., true-positive, true-negative, false-positive, false-negative, accuracy, recall, precision and F1-score) concerning the identification performance of {\oursystem} on a) identifying the mis-disclosure of TPLs in host apps' privacy policy and b) identifying the mis-disclosure of PI interaction with TPLs (Tab.~\ref{tab:metrics}).
%
% Specifically, \textit{True-positive} denotes that {\oursystem} identifies TPLs or data sharing with TPLs in host apps' data flow and host apps' privacy policies claim the TPL or data sharing with TPLs.
% %
% \textit{False-positive} denotes that {\oursystem} identifies 
%
To calculate the metrics, we manually labeled host apps' privacy policies related to TPL usage and PI interaction with TPLs.
%
The ground truth of the TPL list is obtained from {\appbrain}.
%
It is not easy to access the ground truth of host apps sharing what kinds of PI with which TPL. We can only identify the existence of the identified TPL list or PI interaction with TPLs in privacy policies.
%
Thus, we can only identify the false-positive rate of host apps' data interaction with TPLs, i.e., the detected usage in apps' code is not disclosed in privacy policies.
%
Tab.~\ref{tab:metrics} demonstrates that {\oursystem} achieves 95\% F1 score for identifying used TPL in apps and privacy policies, and achieve  95\% accuracy for identifying apps' PI interaction with TPLs.

\answer{4}{
{\oursystem} identifies over 65\% apps comply with the regulations requirements for disclosing data interaction with TPLs.
}
%
% todo: build a table/figure; illustrate the 
% 不一致的数量，这些不一致性存在在多少app中，主要是哪些数据，来自哪些tpl






% \begin{itemize}
%     \item analyze the consistency with labels in appbrain and apps privacy policy
%     \item analyze the consistency with pp analysis results and apps privacy policy
% \end{itemize}
% %
% To figure out whether the TPLs privacy policy clearly states the usage of sensitive personal information (PI), we first built a data set based on the {\appbrain}.
% % 
% Specifically, we crawl the website of each TPL in {\appbrain} and obtain the top ten apps that use the TPL.
% %
% Thus, we can obtain the 



% 介绍方法的准确率
% \input{table/atpchecker_metrics}
\begin{table}[t]
\vspace{3.5ex}
\centering
\smaller

\caption{Metrics of {\oursystem} for identifying host apps' interaction with TPLs.}
\label{tab:metrics}
\begin{tabular}{@{}ccccc@{}}
\toprule
          & TP       & TN        & FN     & FP   \\ \midrule
TPL\_list & 95       & 0         & 0      & 9    \\
TPL\_data & 223      & /         & /      & 12    \\ \midrule
          & Accuracy & Precision & Recall & F1   \\ \midrule
TPL\_list & 0.91     &	0.91 &	1 &	0.95    \\
TPL\_data &  / &	0.95 &	/ &	/
 \\ \bottomrule
\end{tabular}%
% \label{tab:metrics}
\vspace{-2ex}
\end{table}






==> tmp/exp_1212.tex <==
\section{Evaluation}

% \subsection{Dataset Collection and Experimental Setup}
\label{sec:dataset}

\begin{comment}


\noindent\textbf{Collection of Third party libraries.}
We first get the TPLs from AppBrain~\cite{appbrain} that lists three types (Ad networks, social libraries and development tools) of TPLs that are used by top 500 apps (based on  installs) in Google Play. 
%
We collect a list of 458 TPLs that includes 141 ad networks, 25 social libraries and 292 development tools.
%
Based on the TPL list we get from AppBrain, we crawl the corresponding off-the-shelf TPL packages with the latest version file at the time from Maven Repository~\cite{mvnrepository} including the 85 \textit{``aar''} and 102 \textit{``jar''} files. 
%
In this way, we get 187 different TPLs from Maven Repository.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Collection of Host Apps.}
Meanwhile, the AppBrain also provides the mapping relations between the host app and its corresponding used in-app TPLs.
%
Based on the collected TPLs from AppBrain and the mapping relationship, we can pick out the host apps. 
%
For each TPL, we select the top 10 apps based on the installations and download these apps from Google Play. 
%
Finally, we collected a total of 642 distinct apps. Note that, some apps may use multiple TPLs and one TPL can be used by different apps.

\noindent\textbf{Privacy policies of TPLs.}
To get the privacy policies of TPLs listed in {\appbrain}, we visiting the homepage provided by each TPL information page on {\appbrain}.
%
For some TPLs, we can get the link of homepage of TPLs from {\appbrain}~\cite{appbrain}. 
For these TPLs we cannot get the homepage link from the {\appbrain}, we manually search their homepage by using search engine. 
For some open source TPLs, we can visit these published repositories (e.g., Github~\cite{github}, Bitbucket~\cite{bitbucket}) and check the privacy policies from their repositories. 





We manually collect TPLs' privacy policy to analyze whether their data usage are consistent with privacy policies.
%
Specifically, we manually visit the home page of target TPLs list in {\appbrain}~\cite{appbrain}.
%
Then, we search the homepage with keywords: \textit{privacy, policy, legal, and policies}.
%
For one TPL whose homepage does not give in {\appbrain}, we manually search its website.
%
For open source TPLs that are published in Github, we also visit their repositories to search their privacy policy.
% 




\noindent\textbf{Privacy policies of host apps.}
% We also collect the privacy policy of host apps to analyze whether the app's data collection and sharing behavior are consistent with their statements in privacy policy and whether they clearly clarify the usage of
%We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with their statements in privacy policies, and whether they clearly disclose the usage of TPLs.
%
%After obtaining the host apps' package name from AppBrain, we crawl the privacy policies of apps from Google Play~\cite{googleplay}.
%
%Finally, we collect 642 host apps' privacy policies.
%
% TPLs correctly and consistent with the statements of TPLs' privacy policy.
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with the privacy policies and violate the regulation requirements or not. For each host app in our dataset, we can get its privacy policy by crawling the homepage from Google Play.

\end{comment}


We evaluate the performance of {\oursystem} by answering the following research questions:

\noindent\textbf{RQ1: Normativeness Analysis of TPLs.} 
%
\textit{How many TPLs provide privacy policy documents?} 
%
% This research 


% \noindent\textbf{RQ2: TPLs' privacy policy analysis.} 
% %
% \textit{Whether do TPLs' privacy policies correct claim data usage actions?}


\noindent\textbf{RQ2: Legality Analysis of TPLs.}  
%
\textit{Do TPLs’ privacy policies meet regulation requirements, and do TPLs’ privacy policies correctly claim data usage actions?}


% %
% \noindent\textbf{RQ2: TPL privacy policy analysis.} Whether do TPLs contain privacy policies, and are privacy policies consistent with their behavior?

%
\noindent\textbf{RQ3: Host {\app}s behavior analysis.} \textit{Whether do host {\app}s conduct privacy data interaction with TPLs?}
% xian: 这里改为主要和TPL的数据交互行为，哪些违反 pp、哪些 regulation

%
\noindent\textbf{RQ4: Legality of host app's privacy policies.} 
\textit{Whether do host app's privacy policies comply with  requirements for disclosure of TPL usage?}




\input{table/TPL_without_PP_list}

\subsection{RQ1: Normativeness Analysis of TPLs.}
\label{sec:rq1}


\noindent\textbf{Experimental Setup.}
This research question evaluates all Android TPLs listed in AppBrain~\cite{appbrain} including three types: Ad networks, social libraries and development tools.
%
The list gives the TPLs that are widely used by top 500 installed apps in Google Play. 
%
The data set contains 458 TPLs that include 141 ad networks, 25 social libraries and 292 development tools.
%
%
Then, we gather the privacy policies of those TPLs by visiting the homepage provided by each TPL information page on AppBrain.
%
% For TPLs without homepage, we manually search their information.
We manually crawl information of TPLs whose homepages are not provided.  
%
For open source TPLs in Github or Bitbucket, we visit their public repositories and check whether the privacy policies are provided.
%
During visiting the homepage of TPLs, we search the homepage with keywords, such as \textit{privacy, policy, legal} and \textit{policies}, to find potential privacy policy links on the homepage. 
%
Besides, we also manually check whether policy links are given in the typical layout ~\cite{harkous2018polisis}, such as the bottom of the website.
%
Finally, we collect 201 unique privacy policies as some TPLs are built by the same companies or developers.



\noindent\textbf{Results.}
%
According to regulation requirements (\S~\ref{sec:bb_regulation_req}), data controllers should clearly disclose their data usage in privacy policies.
%
% When {\app}s build their functionalities based on TPLs, TPLs take on the role of data controllers~\cite{gdpr, ccpa,piss}.
%
% Besides, GDPR and CCPA also regard TPLs as data controller in their Articles.
%
This research question discloses whether TPLs satisfy the requirements of regulations, i.e., do TPLs correctly provide privacy policies.
%
With the TPL list and  privacy policies, {\oursystem} discovers that 2 of 141 Ad network TPLs, 2 of 25 social libraries, and 103 of 292 development tools TPLs do not provide the privacy policy websites. 
%
We find that some TPLs are created by individual developers and released on {\github}~\cite{github}.
%
% For {\github} repositories, we manually crawl their privacy policies with the data gathering method in .
We manually crawl their privacy policies for {\github} repositories.
% with the data gathering method in \S\ref{sec:dataset}. 
%
Tab.~\ref{tab:tpl_no_pp} summarizes the TPL name and the reasons that the TPLs do not provide privacy policies.
%
Tab.~\ref{tab:tpl_no_pp} demonstrates that 16 of 22 TPLs that do not provide privacy policies are published as Github repositories (GNP).
%
% Single developers mainly develop the TPLs to provide functionalities for other developers. 
%
5 TPLs without privacy policies miss official websites (NOS), and the left does not provide privacy policy documents on their websites (NPOS).
%
For development tool TPLs, we also observe that 66 TPLs from \textit{Google Inc.} share the same privacy policy~\cite{googlepp} that may lead to over claim the personal information usage for specific TPLs.
%
For 9 TPLs from Apache, 6 of them do not provide the privacy policies
% on their official websites 
and two of their websites are Not Found.



\begin{comment}


For Chinese version TPLs, we first collect the data set for analysis as {\appbrain} conducts the statistics mainly on English version TPLs. 
%
As there are no public available statistic websites for Chinese TPLs, we extract them through a snowball collections method~\cite{johnson2014snowball}. 
%
When we manually check the aforementioned privacy policies of TPLs, we also check whether the TPLs' privacy policy websites contain a Chinese version.
%
Besides, we also extract the TPL list from apps' privacy policy documents as some apps' privacy policies may provide the TPL list they used and the corresponding privacy policy links. 
% (Fig~\ref{fig:pp_tpl_list}).
%
When we analyze the Chinese privacy policies of {\app}s, once the privacy policy is an unseen TPL, we will add it to our dataset.
%
We also manually crawl TPLs without privacy policy hyperlinks in host apps' privacy policies.
%
Finally, we gather 130 TPLs, and 115 of them contain the privacy policies.
\end{comment}


\answer{1}{
{\oursystem} reveals  23\% TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
}



% \answer{1}{
% {\oursystem} finds that 6\% English TPLs and 11\% Chinese TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
% }



\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/TPL_PP_data_freq.pdf}
    % \vspace{1ex}

    \caption{Popularity of data types that are used in TPLs' data flow and PP.}
    \vspace{-1ex}
    \label{fig:tpl_data_freq}
\end{figure}


\subsection{RQ2: Legality Analysis of TPLs.}


\noindent\textbf{Experimental Setup.}
We collect the resources of TPLs from Maven Repository~\cite{mvnrepository} based on TPL list from AppBrain (\S\ref{sec:rq1}).
%
We get 187 different TPLs including 85 "aar" and 102 "jar" files.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Results.}
{\oursystem} discloses whether the TPLs' privacy policies satisfy the regulation requirements by comparing TPLs' binary code analysis results (\S\ref{sec:tpl_data}) and privacy policies analysis results (\S~\ref{sec:tpl_pp}).
%
% To analyze whether TPLs privacy policies clearly states the data usage, {\oursystem} analyzes 
%
{\oursystem} analyzes TPLs' privacy policies and obtains the ADUP of personal information usage-related statements.
%
{\oursystem} identifies personal information in the TPL through static analysis (\S\ref{sec:tpl_data}).
%
Finally, {\oursystem} matches the consistency between AUDP and personal information.



% \begin{figure}[t]
%     \centering
%     \vspace{1ex}
%     \includegraphics[width=0.47\textwidth]{figures/TPL_PP_data_freq.pdf}
%     % \vspace{1ex}

%     \caption{Popularity of data types that are most mentioned in TPLs' PP}
%     % \vspace{-2ex}
%     \label{fig:tpl_pp_data_freq}
% \end{figure}




\noindent{\textit{TPL privacy policies analysis.}}
%
{\oursystem} analyzes 187 unique TPLs' privacy policy documents.
%
We analyze 42,895 sentences with sharing and collection (SAC) words, and each privacy policy has an average of 420.5 sentences and 136 SAC words.
%
Among sentences with SAC words, 19,750 sentences start with 5W1H words that are not related to data usage actions.
%
Besides, 1654 sentences only vaguely state that the TPL will collect personal information without specific data types.
%
For example, $com.xiledsystems$  only claims \textit{``We collect your personal information in order to provide and continually improve our products and services,"} but no specific personal information is given.
%
In data usage-related actions, {\oursystem} analyzes the personal information 
% (Tab.~\ref{tab:data_type}) 
that are mostly used by TPLs.
%
Fig.~\ref{fig:tpl_data_freq} shows the times that are mentioned in TPLs' privacy policies.
%23
It can be observed that \textit{contact} are the most  used personal information.
%
This may be  caused by the fact that, by getting contact, the TPLs can easily expand and prompt their services.
%
Account, address and email are the second most popular data mentioned in TPLs' privacy policies.
%
Among the statements that claim to collect  accounts, addresses, and email, 21.13\% of sentences claim that they collect related data for contacting users. 
%
For example, one of them claims that \textit{``we will use your email, phone number, or other contact information you provide us by written or oral means for contacting you and providing you with the services and information that             you request"}.









\begin{figure}[t]
    \centering
    \vspace{-1ex}
    \includegraphics[width=0.42\textwidth]{figures/FCG_compare.pdf}
    \vspace{-1.5ex}
    \caption{Evaluation of function call graph construction.}
    % \vspace{-2ex}
    \label{fig:fcg_compare}
\end{figure}


\vspace{1ex}
\noindent{\textit{TPL data usage analysis.}}
%% analyze whether our fcg construction method effective/improved
As the basis of data flow analysis, we first evaluate the effectiveness of {\oursystem} in improving the FCG construction performance.
%34
We analyze TPLs' FCG quality through comparing the a) FCG coverage and b) the number of edges between the raw FCG built by soot and our optimized FCG.
%
FCG coverage is calculated by:
%FCG coverage : the number of nodes in FCG/ the number of methods 
\begin{equation}
    \label{eq:fcg_cov}
    cov_{FCG} = \frac{\#Nodes_{FCG}}{\#Nodes_{TPL}},
\end{equation}
where {\smaller{$\#Nodes_{FCG}$}} is the number of nodes (methods) in FCG and {\smaller{$\#Nodes_{TPL}$}} is the total number of TPLs' methods.
%
Fig.~\ref{fig:fcg_compare} illustrates the box plots of {\oursystem}'s performance in  optimizing  FCG construction, and the number at the top of boxes denotes measuring units of the data for better illustration.
%
Fig.~\ref{fig:fcg_compare} demonstrates that {\oursystem}'s FCG coverage achieves an average performance of 55\%, while the FCG coverage of raw FCG only achieves an average of 0.34\%, which  means it nearly fails to construct the FCG of TPLS.
%
{\smaller{$raw_{\#edge}$}} denotes the raw FCG only contains the 159 average edges, while the {\smaller{${\oursystem}_{\#edge}$}} shows the improved FCG can extract 12,960 edges.
%
The results indicate that the soot nearly fails to analyze the FCG of TPLs, and {\oursystem} optimizes construction performance and improves the FCG quality.



% Then, 
{\oursystem} analyzes the data usage of TPLs to identify the consistency with their privacy policy statements.
%
{\oursystem} analyzes the data flow of TPLs and discovers that 65 out of 187 TPLs access users' personal information.
%
{\oursystem} identifies 146 data usage from 2,396 traces.
%
Among data usage behavior, 31 out of 146 invokes Android APIs (such as \textit{``android.telephony.TelephonyManager: java.lang.String getSimSerialNumber()"}) to access Android Sim Serial number.
%
Fig.~\ref{fig:tpl_data_freq} shows the data frequencies that are mostly used in TPLs' data flow (shown in orange color).
%
% It can also be observed that TPLs' privacy policies tend to disclose information that is not directly related to users' personal information, such as \textit{contact}, while their actions tend to access the information that is identical to the users, such as \textit{SimSerialNumber}.
It can also be observed that TPLs' privacy policies tend to disclose non-identical information, such as \textit{contact}, while their actions tend to access identical information. 
% , such as \textit{SimSerialNumber}.


\begin{figure}[t]
    \centering
    \vspace{1ex}
    \includegraphics[width=0.46\textwidth]{figures/tpl_propa.pdf}
    % \vspace{1ex}

    \caption{TPL Privacy Policy Non-compliance Propagation.}
    % \vspace{-2ex}
    \label{fig:tpl_pp_dep}

\end{figure}

% \begin{comment}


{\oursystem} identifies the compliance of TPLs by combing the privacy policies analysis results and data flow analysis results.
%
%  {\oursystem} identifies whether the personal information usage in TPLs' binary code are consistent with the statements that claim PI collections in their privacy policies.
%
Specifically, {\oursystem} identifies how many TPLs comply with regulations by identifying whether the PI in data flow are also mentioned in ADUP. 
%
{\oursystem} discovers that 24 out of 65 (37\%) TPLs violate the regulation requirements, i.e., the TPLs collect at least one PI in their binary code  without clearly disclosing them in privacy policies.  
% \end{comment}



% \vspace{1ex}
\noindent{\textit{Investigation on perniciousness of TPLs' incompliant behavior.}}
%
After identifying TPLs that do not satisfy the regulation requirements, we also identify the  harm of TPLs' incompliant behavior on a large scale.
%
% It is well known that 
TPLs may integrate other TPLs to enhance their functionalities or facilitate usability~\cite{atvhunter2021ICSE}.
%
Thus, once one TPL ($TPL_v$) violates the law, other artifacts integrated $TPL_v$ may spread the threats and make their privacy policies violate regulation requirements.
%
To expose the impacts, {\oursystem} analyzes the dependencies among TPLs. 
%
Specifically, {\oursystem} crawls the TPLs that use $TPL_v$, that are analyzed in \S\ref{sec:tpl_data}-\ref{sec:tpl_pp}, from {\maven}.
%
Then starting from these TPLs ($TPL_v$), {\oursystem} crawls the list of TPLs that integrate $TPL_U$.
%
In this way, {\oursystem} investigates the propagation of $TPL_v$'s threats under two times invocations and visualizes it in Fig.~\ref{fig:tpl_pp_dep}.
%
% Specifically, 
{\oursystem} starts analysis with 25 unconventional TPLs.
%
Fig.~\ref{fig:tpl_pp_dep} demonstrates the harm of that privacy policy inconsistency  propagation 
% (i.e., the TPL is directly used by another TPL) 
with five selected TPLs.  
%
It can be observed that after one round of propagation, even five TPLs will affect 24,737 TPLs (25 TPLs affects extra 79,471 TPLs). After two rounds of propagation, the threats even spread to 18,323 TPLs (25 to 447,300).
%
Fig.~\ref{fig:tpl_pp_dep} also demonstrates that not only the popular TPLs demonstrate infective (be widely used by other TPLs), such as \textit{``common-io/commons-io"}, 
% developed by \textit{apache}
some minority TPLs, such as \textit{``com.google.gdata/gdata-clien"} are directly used by only 11 TPLs.
%
After two rounds of propagation, the number of TPLs they affect increases exponentially.
%
This observation indicates that developers should pay attention to the usage data of TPLs, especially the functions that are related to privacy.


% \subsection{Legality of TPLs}



\answer{2}{
{\oursystem} identifies over 37\% TPLs miss disclosing their data usage in privacy policy documents.
%
{\oursystem} investigates that the perniciousness of privacy policy non-compliance harms spread exponentially.
}


\subsection{RQ3: Analysis of host apps' interaction with TPLs}
\label{sec:rq3}

\noindent\textbf{Experimental Setup.}
%
We collect the host apps of TPLs from AppBrain to investigate host apps' interaction with TPLs.
%
We gather the host app list using the mapping relations between host apps and used in-app TPLs provided in AppBrain.
%
We can access the top ten installation host app list for each TPL and then download the apps.
%
Finally, we gather a total of 642 distinct apps because some apps may use multiple TPLs and on TPL can be used by different apps.






\noindent\textbf{Results.}
{\oursystem} uses data flow analysis to investigate whether host apps conduct personal information interaction with TPLs and what kinds of PI are shared with TPLs.
%
{\oursystem} analyzes 642 distinct apps with labels, i.e., which TPLs are used.
%
% {\oursystem} analyzes the data flow of apps (\S\ref{sec:host_app_data}).
%
% Besides, we also collect 256 extra apps with Chinese privacy policies for analysis.




\begin{figure}[t]
    \centering
   %  \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/host_app_TPL_data_interaction.pdf}
    % \vspace{-1ex}
    \caption{Statistics of host apps' interaction with TPLs.}
    % \vspace{-2ex}
    \label{fig:app_int_tpl}
\end{figure}


{\oursystem} identifies over 60.5\% host apps share PI with TPLs and as is illustrated in Fig.~\ref{fig:app_int_tpl}.
%
{\oursystem} traces 2,216 data sharing behaviors with TPLs and finds that over 53.1\% traces share users' \textit{sim serial number} with TPLs such as \textit{``com.google.android.gms", ``com.applovin", ``com.onesignal"}.
%
Although \textit{``com.google.android.gms"} is a well know TPL that provides users abundant Google services, the sharing of \textit{sim serial number} is sensitive to identify one individual.
%
Fig.~\ref{fig:app_int_tpl} demonstrates the top five data shared by host apps with TPLs.
% 
Fig.~\ref{fig:app_int_tpl} shows that the secondary data the host app need to share with TPLs is network status, as TPLs will need to connect server to provide services, like advertising or data analytic.
%
{\oursystem} also observes that \textit{``com.google.android.gms"} is the TPL that accesses the most PI from host apps.
%
% Although \textit{``com.google.android.gms"} provides abundant functionalities such as gmail, music, TPLs should avoid collecting information like SIM serial number that is easy to identify an individual.
%
TPLs should not ask for more data than is required for the content of their services~\cite{zhSDKLaw,gdpr,ccpa,piss}.




\answer{3}{
{\oursystem} identifies that over 60.5\%  of  host apps share personal information with TPLs.
%
Among shared PI, sim serial number accounts for over 53.1\%  of traces in identified user data access actions.
%
{\oursystem} also discovers that while well-known TPLs provide rich functionalities, they also request the personal information.
}


\begin{figure}[t]
    \centering
    %\vspace{-2ex}
    \includegraphics[width=0.42\textwidth]{figures/mssing_TPL.pdf}
    \vspace{-2.5ex}
    \caption{Statistics of missing TPLs in host apps' PP.}
    \vspace{-0.5ex}
    \label{fig:miss_tpl}
\end{figure}


\subsection{RQ4: Host apps privacy policy analysis.}
\label{exp:host_app_pp}


\noindent\textbf{Experimental Settings.}
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior is consistent with the privacy policies.
% and violate the regulation requirements or not. 
%
For each host app in our dataset, we  get its privacy policy by crawling the homepage from Google Play.
%
Then, one expert and one senior researcher in software engineering and privacy policy analysis manually label the privacy policies to evaluate the performance of {\oursystem}. 



\noindent\textbf{Results.}
{\oursystem} identifies whether host apps' privacy policies comply with regulation requirements concerning descriptions about TPLs by analyzing whether privacy policies disclosure their usage and interaction with TPLs.
%
{\oursystem} implements this 
% by discovering the problems of privacy policy descriptions concerning TPL usage
by combining the static analysis results (\S\ref{sec:rq3}) and privacy policy analysis results.
%
{\oursystem} identifies 
a) whether apps integrate TPLs in their code without disclosure in privacy policies and 
b) whether TPLs access sensitive PI without descriptions.
%
We randomly selected 256 apps to annotate the privacy policies and evaluate the identification performance.
%
To annotate the privacy policies, one expert and senior researcher, who have conducted research on privacy policy and software engineering for over seven years and two years respectively, manually label the sentences that include data usage, TPL usage and data interaction wit TPLs.
%
The annotation process is conduct in an in-house manner~\cite{sorokin2008utility} that guarantees the quality and agreement of the labels.
% Then, we manually labeled privacy policies that include the data usage, TPL usage and data interaction with TPLs.
%

\kaifa{
{\oursystem} identifies 65.63\% (168/256) apps violating the regulation requirements, i.e., their privacy policies miss disclosing TPL usage in their privacy policies.
%
Fig.~\ref{fig:miss_tpl} shows the most popular 15 TPLs that are missed being disclosed by host apps.
%
It can be observed that over 25\% privacy policy's user data access conceal behavior is related to the TPL (\textit{``com.alipay"}). 
%
This may lie in the fact that host apps only use the TPL to launch the \textit{alipay} app for payment and do not use the TPL for user data access behavior. 
%
Even so, host apps are still required to claim their usage of the TPL in their privacy policies~\cite{zhSDKLaw}.
%
Among concealed data interaction with TPLs, the most popular PI data, that the app interacts with TPL but not discloses in the PP, are \textit{device ID}, \textit{mac address}, and \textit{sim serial number}, which account for 95.82\% (321/335) conflicts.
}






To this end, we also evaluate the performance of {\oursystem}.
%
We evaluate the eight metrics (i.e., true-positive, true-negative, false-positive, false-negative, accuracy, recall, precision and F1-score) concerning the identification performance of {\oursystem} on a) identifying the mis-disclosure of TPLs in host apps' privacy policy and b) identifying the mis-disclosure of PI interaction with TPLs (Tab.~\ref{tab:metrics}).
%
To calculate the metrics, we manually labeled host apps' privacy policies related to TPL usage and PI interaction with TPLs.
%
The ground truth of the TPL list is obtained from {\appbrain}.
%
It is not easy to access the ground truth of host apps sharing what kinds of PI with which TPL. We can only identify the existence of the identified TPL list or PI interaction with TPLs in privacy policies.
%
Thus, we can only identify the false-positive rate of host apps' data interaction with TPLs, i.e., the detected usage in apps' code is not disclosed in privacy policies.
%
Tab.~\ref{tab:metrics} demonstrates that {\oursystem} achieves 95\% F1 score for identifying used TPL in apps and privacy policies, and achieve  95\% accuracy for identifying apps' PI interaction with TPLs.

\answer{4}{
{\oursystem} identifies over 65\% apps comply with the regulations requirements for disclosing apps data interaction with TPLs.
}
%
% todo: build a table/figure; illustrate the 
% 不一致的数量，这些不一致性存在在多少app中，主要是哪些数据，来自哪些tpl






% \begin{itemize}
%     \item analyze the consistency with labels in appbrain and apps privacy policy
%     \item analyze the consistency with pp analysis results and apps privacy policy
% \end{itemize}
% %
% To figure out whether the TPLs privacy policy clearly states the usage of sensitive personal information (PI), we first built a data set based on the {\appbrain}.
% % 
% Specifically, we crawl the website of each TPL in {\appbrain} and obtain the top ten apps that use the TPL.
% %
% Thus, we can obtain the 



% 介绍方法的准确率
% \input{table/atpchecker_metrics}
\begin{table}[t]
\vspace{3.5ex}
\centering
\smaller

\caption{Metrics of {\oursystem} for identifying host apps' interaction with TPLs.}
\label{tab:metrics}
\begin{tabular}{@{}ccccc@{}}
\toprule
          & TP       & TN        & FN     & FP   \\ \midrule
TPL\_list & 95       & 0         & 0      & 9    \\
TPL\_data & 223      & /         & /      & 12    \\ \midrule
          & Accuracy & Precision & Recall & F1   \\ \midrule
TPL\_list & 0.91     &	0.91 &	1 &	0.95    \\
TPL\_data &  / &	0.95 &	/ &	/
 \\ \bottomrule
\end{tabular}%
% \label{tab:metrics}
\vspace{-2ex}
\end{table}






==> tmp/exp_old-0902.tex <==
\section{Evaluation}

% \subsection{Dataset Collection and Experimental Setup}
\label{sec:dataset}

\begin{comment}


\noindent\textbf{Collection of Third party libraries.}
We first get the TPLs from AppBrain~\cite{appbrain} that lists three types (Ad networks, social libraries and development tools) of TPLs that are used by top 500 apps (based on  installs) in Google Play. 
%
We collect a list of 458 TPLs that includes 141 ad networks, 25 social libraries and 292 development tools.
%
Based on the TPL list we get from AppBrain, we crawl the corresponding off-the-shelf TPL packages with the latest version file at the time from Maven Repository~\cite{mvnrepository} including the 85 \textit{``aar''} and 102 \textit{``jar''} files. 
%
In this way, we get 187 different TPLs from Maven Repository.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Collection of Host Apps.}
Meanwhile, the AppBrain also provides the mapping relations between the host app and its corresponding used in-app TPLs.
%
Based on the collected TPLs from AppBrain and the mapping relationship, we can pick out the host apps. 
%
For each TPL, we select the top 10 apps based on the installations and download these apps from Google Play. 
%
Finally, we collected a total of 642 distinct apps. Note that, some apps may use multiple TPLs and one TPL can be used by different apps.

\noindent\textbf{Privacy policies of TPLs.}
To get the privacy policies of TPLs listed in {\appbrain}, we visiting the homepage provided by each TPL information page on {\appbrain}.
%
For some TPLs, we can get the link of homepage of TPLs from {\appbrain}~\cite{appbrain}. 
For these TPLs we cannot get the homepage link from the {\appbrain}, we manually search their homepage by using search engine. 
For some open source TPLs, we can visit these published repositories (e.g., Github~\cite{github}, Bitbucket~\cite{bitbucket}) and check the privacy policies from their repositories. 





We manually collect TPLs' privacy policy to analyze whether their data usage are consistent with privacy policies.
%
Specifically, we manually visit the home page of target TPLs list in {\appbrain}~\cite{appbrain}.
%
Then, we search the homepage with keywords: \textit{privacy, policy, legal, and policies}.
%
For one TPL whose homepage does not give in {\appbrain}, we manually search its website.
%
For open source TPLs that are published in Github, we also visit their repositories to search their privacy policy.
% 




\noindent\textbf{Privacy policies of host apps.}
% We also collect the privacy policy of host apps to analyze whether the app's data collection and sharing behavior are consistent with their statements in privacy policy and whether they clearly clarify the usage of
%We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with their statements in privacy policies, and whether they clearly disclose the usage of TPLs.
%
%After obtaining the host apps' package name from AppBrain, we crawl the privacy policies of apps from Google Play~\cite{googleplay}.
%
%Finally, we collect 642 host apps' privacy policies.
%
% TPLs correctly and consistent with the statements of TPLs' privacy policy.
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with the privacy policies and violate the regulation requirements or not. For each host app in our dataset, we can get its privacy policy by crawling the homepage from Google Play.

\end{comment}


We evaluate the performance of {\oursystem} by answering the following research questions:

\noindent\textbf{RQ1: Normativeness Analysis of TPLs.} 
%
\textit{How many TPLs provide privacy policy documents?} 
%
% This research 


% \noindent\textbf{RQ2: TPLs' privacy policy analysis.} 
% %
% \textit{Whether do TPLs' privacy policies correct claim data usage actions?}


\noindent\textbf{RQ2: Legality Analysis of TPLs.}  
%
\textit{Do TPLs’ privacy policies meet regulation requirements, and do TPLs’ privacy policies correctly claim data usage actions?}


% %
% \noindent\textbf{RQ2: TPL privacy policy analysis.} Whether do TPLs contain privacy policies, and are privacy policies consistent with their behavior?

%
\noindent\textbf{RQ3: Host {\app}s behavior analysis.} \textit{Whether do host {\app}s conduct privacy data interaction with TPLs?}
% xian: 这里改为主要和TPL的数据交互行为，哪些违反 pp、哪些 regulation

%
\noindent\textbf{RQ4: Legality of host app's privacy policies.} 
\textit{Whether do host app's privacy policies comply with  requirements for disclosure of TPL usage?}




\input{table/TPL_without_PP_list}

\subsection{RQ1: Normativeness Analysis of TPLs.}
\label{sec:rq1}


\noindent\textbf{Experimental Setup.}
This research question evaluates all Android TPLs listed in AppBrain~\cite{appbrain} including three types: Ad networks, social libraries and development tools.
%
The list gives the TPLs that are widely used by top 500 installed apps in Google Play. 
%
The data set contains 458 TPLs that include 141 ad networks, 25 social libraries and 292 development tools.
%
%
Then, we gather the privacy policies of those TPLs by visiting the homepage provided by each TPL information page on AppBrain.
%
% For TPLs without homepage, we manually search their information.
We manually crawl information of TPLs whose homepages are not provided.  
%
For open source TPLs in Github or Bitbucket, we visit their public repositories and check whether the privacy policies are provided.
%
During visiting the homepage of TPLs, we search the homepage with keywords, such as \textit{privacy, policy, legal} and \textit{policies}, to find potential privacy policy links on the homepage. 
%
Besides, we also manually check whether policy links are given in the typical layout ~\cite{harkous2018polisis}, such as the bottom of the website.
%
Finally, we collect 201 unique privacy policies as some TPLs are built by the same companies or developers.



\noindent\textbf{Results.}
%
According to regulation requirements (\S~\ref{sec:bb_regulation_req}), data controllers should clearly disclose their data usage in their privacy policies.
%
% When {\app}s build their functionalities based on TPLs, TPLs take on the role of data controllers~\cite{gdpr, ccpa,piss}.
%
% Besides, GDPR and CCPA also regard TPLs as data controller in their Articles.
%
This research question disclovers whether TPLs satisfy the requirements of regulations, i.e., do TPLs correctly provide privacy policies.
%
%In this research question, we concentrates on the TPLs listed in AppBrain and TPLs list that we obtained through the snowball search.




% {\oursystem} analyzes publicly used TPLs as are listed in {\appbrain}~\cite{appbrain} that include three categories: Ad networks, social libraries, and development tool.
%
With the TPL list and TPL's privacy policy collection methods described in \S\ref{sec:dataset}, {\oursystem} discovers that 2 of 141 Ad network TPLs, 2 of 25 social libraries, and 103 of 292 development tools TPLs do not provide the privacy policy websites. 

%
Besides, we observe that some TPLs are created by individual developers and released on {\github}~\cite{github}.
%
% For {\github} repositories, we manually crawl their privacy policies with the data gathering method in .
We manually crawl their privacy policies for {\github} repositories with the data gathering method in \S\ref{sec:dataset}. 
%
Tab.~\ref{tab:tpl_no_pp} summarizes the TPL name and the reasons that the TPLs do not provide privacy policies.
%
Tab.~\ref{tab:tpl_no_pp} demonstrates that 16 of 22 TPLs that do not provide privacy policies are published as Github repositories (GNP).
%
% Single developers mainly develop the TPLs to provide functionalities for other developers. 
%
5 TPLs without privacy policies miss official websites (NOS), and the left does not provide privacy policy documents on their websites (NPOS).
%
For development tool TPLs, we also observe that 66 TPLs from \textit{Google Inc.} share the same privacy policy~\cite{googlepp} that may lead to over claim the personal information usage for specific TPLs.
%
For 9 TPLs from Apache, 6 of them do not provide the privacy policies
% on their official websites 
and two of their websites are Not Found.



\begin{comment}


For Chinese version TPLs, we first collect the data set for analysis as {\appbrain} conducts the statistics mainly on English version TPLs. 
%
As there are no public available statistic websites for Chinese TPLs, we extract them through a snowball collections method~\cite{johnson2014snowball}. 
%
When we manually check the aforementioned privacy policies of TPLs, we also check whether the TPLs' privacy policy websites contain a Chinese version.
%
Besides, we also extract the TPL list from apps' privacy policy documents as some apps' privacy policies may provide the TPL list they used and the corresponding privacy policy links. 
% (Fig~\ref{fig:pp_tpl_list}).
%
When we analyze the Chinese privacy policies of {\app}s, once the privacy policy is an unseen TPL, we will add it to our dataset.
%
We also manually crawl TPLs without privacy policy hyperlinks in host apps' privacy policies.
%
Finally, we gather 130 TPLs, and 115 of them contain the privacy policies.
\end{comment}


\answer{1}{
{\oursystem} reveals  23\% TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
}



% \answer{1}{
% {\oursystem} finds that 6\% English TPLs and 11\% Chinese TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
% }



\begin{figure}[t]
    \centering
    \vspace{1ex}
    \includegraphics[width=0.44\textwidth]{figures/TPL_PP_data_freq.pdf}
    % \vspace{1ex}

    \caption{Popularity of data types that are used in TPLs' data flow and PP}
    \vspace{-1ex}
    \label{fig:tpl_data_freq}
\end{figure}


\subsection{RQ2: Legality Analysis of TPLs.}


\noindent\textbf{Experimental Setup.}
We first gather the TPLs from Maven Repository~\cite{mvnrepository} based on TPL list from AppBrain (\S\ref{sec:rq1}).
%
We get 187 different TPLs that include 85 "aar" and 102 "jar" files.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Results.}
{\oursystem} analyzes whether the TPLs' privacy policies satisfy the regulation requirements by comparing TPLs' functionality (\S\ref{sec:tpl_data}) and privacy policies (\S~\ref{sec:tpl_pp}).
%
% To analyze whether TPLs privacy policies clearly states the data usage, {\oursystem} analyzes 
%
{\oursystem} analyzes TPLs' privacy policies and obtains the ADUP of personal information usage-related statements.
%
{\oursystem} identifies personal information in the TPL through static analysis (\S\ref{sec:tpl_data}).
%
Finally, {\oursystem} matches the consistency between AUDP and personal information.



% \begin{figure}[t]
%     \centering
%     \vspace{1ex}
%     \includegraphics[width=0.47\textwidth]{figures/TPL_PP_data_freq.pdf}
%     % \vspace{1ex}

%     \caption{Popularity of data types that are most mentioned in TPLs' PP}
%     % \vspace{-2ex}
%     \label{fig:tpl_pp_data_freq}
% \end{figure}




\noindent{\textit{TPL privacy policies analysis.}}
%
{\oursystem} analyzes 187 unique TPLs' privacy policy documents.
%
We analyze 42,895 sentences with sharing and collection (SAC) words in 7,864 sentences, and each privacy policy has an average of 420.5 sentences and 136 SAC words.
%
Among sentences with SAC words, 19,750 sentences start with 5W1H (\S\ref{sec:tpl_pp}) words that are not related to data usage actions.
%
Besides, 1654 sentences only vaguely state that the TPL will collect personal information rather than specific data types.
%
For example, $com.xiledsystems$  only claims \textit{"We collect your personal information in order to provide and continually improve our products and services,"} but no specific personal information is  given.
%
In data usage-related actions, {\oursystem} analyzes the personal information (Tab.~\ref{tab:data_type}) that are used by TPLs.
%
Fig.~\ref{fig:tpl_data_freq} shows the times that are mentioned in TPLs' privacy policies.
%23
It can be observed that \textit{contact} are the most  used personal information.
%
This may be  caused by the fact that, by getting contact, the TPLs can easily expand and prompt their services.
%
Account, address and email are the second most popular data mentioned in TPLs' privacy policies.
%
Among the statements that claim to collect  accounts, addresses, and email, 21.13\% of sentences claim that they collect related data for contacting users. 
%
For example, one of them claims that \textit{"we will use your email, phone number, or other contact information you provide us by written or oral means for contacting you and providing you with the services and information that             you request"}.









\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.40\textwidth]{figures/FCG_compare.pdf}
    \vspace{-1.5ex}
    \caption{Evaluation of function call graph construction}
    % \vspace{-2ex}
    \label{fig:fcg_compare}
\end{figure}


\vspace{1ex}
\noindent{\textit{TPL data usage analysis.}}
%% analyze whether our fcg construction method effective/improved
As the basis of data flow analysis, we first evaluate the effectiveness of {\oursystem} in improving the FCG construction performance.
%34
We analyze TPLs' FCG quality through comparing the a) FCG coverage and b) the number of edges between the raw FCG built by soot and our optimized FCG.
%
FCG coverage is calculated by:
%FCG coverage : the number of nodes in FCG/ the number of methods 
\begin{equation}
    \label{eq:fcg_cov}
    cov_{FCG} = \frac{\#Nodes_{FCG}}{\#Nodes_{TPL}},
\end{equation}
where $\#Nodes_{FCG}$ is the number of nodes (methods) in FCG and $\#Nodes_{TPL}$ is the total number of TPLs' methods.
%
Fig.~\ref{fig:fcg_compare} illustrates the box plots of {\oursystem}'s performance in  optimizing  FCG construction, and the number at the top of boxes denotes measuring units of the data for better illustration.
%
Fig.~\ref{fig:fcg_compare} demonstrates that  {\oursystem}'s FCG coverage achieves an average performance of 55\%, while the FCG coverage of raw FCG only achieves an average of 0.34\%, which  means it nearly fails to construct the FCG of TPLS.
%
The $raw_{\#edge}$ denotes the raw FCG only contains the 159 average edges, while the ${\oursystem}_{\#edge}$ shows the improved FCG can extract 12,960 edges.
%
The results indicate that the soot nearly fails to analyze the FCG of TPLs, and {\oursystem}'s optimizes construction performance methods and improves the FCG quality.



% Then, 
{\oursystem} analyzes the data usage (\S\ref{sec:tpl_data}) of TPLs to identify the consistency with their privacy policy statements.
%
{\oursystem} analyzes the data flow of TPLs and discovers that 65 out of 187 TPLs access users' personal information.
%
{\oursystem} identifies 146 data leakages from 2,396 traces.
%
Among data leakage behavior, 31 out of 146 invokes Android APIs (such as \textit{"$\langle$android.telephony.Tele-phonyManager: java.lang.String getSimSerialNumber()$rlangle$"}) to access Android Sim Serial number.
%
Fig.~\ref{fig:tpl_data_freq} shows the data frequencies that are mostly used in TPLs' data flow (shown in orange color).
%
% It can also be observed that TPLs' privacy policies tend to disclose information that is not directly related to users' personal information, such as \textit{contact}, while their actions tend to access the information that is identical to the users, such as \textit{SimSerialNumber}.
It can also be observed that TPLs' privacy policies tend to disclose personally identical information, such as \textit{contact}, while their actions tend to access identical information, such as \textit{SimSerialNumber}.


\begin{figure}[t]
    \centering
    \vspace{1ex}
    \includegraphics[width=0.46\textwidth]{figures/tpl_propa.pdf}
    % \vspace{1ex}

    \caption{TPL Privacy Leakage Propagation}
    % \vspace{-2ex}
    \label{fig:tpl_pp_dep}
\end{figure}

% \begin{comment}


{\oursystem} identifies the compliance of TPLs by combing the privacy policies analysis results and data flow analysis results.
%
%  {\oursystem} identifies whether the personal information usage in TPLs' binary code are consistent with the statements that claim PI collections in their privacy policies.
%
Specifically, {\oursystem} identifies how many TPLs comply with regulations by identifying whether the PI in data flow are also mentioned in ADUP. 
%
{\oursystem} discovers that 24 out of 65 (37\%) TPLs violate the regulation requirements, i.e., the TPLs collect at least one PI in their binary code  without clearly disclosing them in privacy policies.  
% \end{comment}


% \vspace{1ex}
\noindent{\textit{Investigation on perniciousness of TPLs' incompliant behavior.}}
%
After identifying TPLs that do not satisfy the regulation requirements, we also identify the  harm of TPLs' incompliant behavior on a large scale.
%
% It is well known that 
TPLs may integrate other TPLs to enhance their functionalities or facilitate usability~\cite{atvhunter2021ICSE}.
%
Thus, once one TPL ($TPL_v$) violates the law and carries potential data leakage vulnerabilities, other artifacts integrated $TPL_v$ may spread the vulnerabilities.
%
To expose the vulnerabilities, {\oursystem} analyzes the dependencies among TPLs. 
%
Specifically, {\oursystem} crawls the TPLs that use vulnerable TPL ($TPL_v$), that are analyzed in \S\ref{sec:tpl_data}-\ref{sec:tpl_pp}, from {\maven}.
%
Then starting from these TPLs ($TPL_v$), {\oursystem} crawls the list of TPLs that integrate $TPL_U$.
%
In this way, {\oursystem} investigates the propagation of the vulnerabilities of TPLs under two times invocations and visualizes it in Fig.~\ref{fig:tpl_pp_dep}.
%
% Specifically, 
{\oursystem} starts analysis with 25 unconventional TPLs.
%
Fig.~\ref{fig:tpl_pp_dep} demonstrates the harm of that privacy leakage propagation 
% (i.e., the TPL is directly used by another TPL) 
with five selected TPLs.  
%
It can be observed that after one round of propagation, even five TPLs will affect 24,737 TPLs (25 TPLs affects extra 79,471 TPLs). After two rounds of propagation, the vulnerabilities even spread to 18,323 TPLs (25 to 447,300).
%
Fig.~\ref{fig:tpl_pp_dep} also demonstrates that not only the popular TPLs demonstrate infective (be widely used by other TPLs), such as \textit{"common-io/commons-io"}, 
% developed by \textit{apache}
some minority TPLs, such as \textit{"com.google.gdata/gdata-clien"} are directly used by only 11 TPLs.
%
After two rounds of propagation, the number of TPLs they affect increases exponentially.
%
This observation indicates that developers should pay attention to the usage data of TPLs, especially the functions that are related to privacy.


% \subsection{Legality of TPLs}



\answer{2}{
{\oursystem} identifies over 37\% TPLs miss disclosing their data usage in privacy policy documents.
%
{\oursystem} investigates that the perniciousness of potential data leakage behavior in privacy policy spread exponentially.
}


\subsection{RQ3: Analysis of host apps' interaction with TPLs}
\label{sec:rq3}

\noindent\textbf{Experimental Setup.}
%
We collect the host apps of TPLs from AppBrain to investigate host apps' interaction with TPLs.
%
We gather the host app list using the mapping relations between host apps and used in-app TPLs provided in AppBrain.
%
We can access the top ten installation host app list for each TPL and then download the apps.
%
Finally, we gather a total of 642 distinct apps because some apps may use multiple TPLs and on TPL can be used by different apps.






\noindent\textbf{Results.}
{\oursystem} uses data flow analysis to investigate whether host apps conduct personal information interaction with TPLs and what kinds of PI are shared with TPLs.
%
{\oursystem} analyzes 642 distinct apps with labels, i.e., which TPLs are used.
%
% {\oursystem} analyzes the data flow of apps (\S\ref{sec:host_app_data}).
%
% Besides, we also collect 256 extra apps with Chinese privacy policies for analysis.




\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/host_app_TPL_data_interaction.pdf}
    % \vspace{-1ex}
    \caption{Statistics of host apps' interaction with TPLs}
    % \vspace{-2ex}
    \label{fig:app_int_tpl}
\end{figure}


{\oursystem} identifies over 60.5\% host apps share PI with TPLs and as is illustrated in Fig.~\ref{fig:app_int_tpl}.
%
{\oursystem} traces 2,216 data sharing behaviors with TPLs and finds that over 53.1\% traces share users' \textit{sim serial number} with TPLs such as \textit{"com.google.android.gms", "com.applovin", "com.onesignal"}.
%
Although \textit{"com.google.android.gms"} is a well know TPL that provides users abundant Google services, the sharing of \textit{sim serial number} is sensitive to identify one individual.
%
Fig.~\ref{fig:app_int_tpl} demonstrates the top five data shared by host apps with TPLs.
% 
Fig.~\ref{fig:app_int_tpl} shows that the secondary data the host app need to share with TPLs is network status, as TPLs will need to connect server to provide services, like advertising or data analytic.
%
{\oursystem} also observes that \textit{"com.google.android.gms"} is the TPL that accesses the most PI from host apps.
%
% Although \textit{"com.google.android.gms"} provides abundant functionalities such as gmail, music, TPLs should avoid collecting information like SIM serial number that is easy to identify an individual.
%
TPLs should not ask for more data than is required for the content of their services~\cite{zhSDKLaw,gdpr,ccpa,piss}.




\answer{3}{
{\oursystem} identifies that over 60.5\%  of  host apps share personal information with TPLs.
%
Among shared PI, sim serial number accounts for over 53.1\%  of traces in identified data leakage actions.
%
{\oursystem} also discovers that while well-known TPLs provide rich functionalities, they also request the most personal information.
}


\begin{figure}[t]
    \centering
    % \vspace{-2ex}
    \includegraphics[width=0.42\textwidth]{figures/mssing_TPL.pdf}
    % \vspace{-1.5ex}
    \caption{Statistics of missing TPLs in host apps' PP}
    % \vspace{-2ex}
    \label{fig:miss_tpl}
\end{figure}


\subsection{RQ4: Host apps privacy policy analysis.}
\label{exp:host_app_pp}


\noindent\textbf{Experimental Settings.}
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior is consistent with the privacy policies.
% and violate the regulation requirements or not. 
%
For each host app in our dataset, we  get its privacy policy by crawling the homepage from Google Play.
%
Then, one expert and one senior researcher in software engineering and privacy policy analysis manually label the privacy policies to evaluate the performance of {\oursystem}. 



\noindent\textbf{Results.}
{\oursystem} identifies whether host apps' privacy policies comply with regulation requirements concerning descriptions about TPLs by analyzing whether privacy policies disclosure their usage and interaction with TPLs.
%
{\oursystem} implements this 
% by discovering the problems of privacy policy descriptions concerning TPL usage
by combining the static analysis results (\S\ref{sec:rq3}) and privacy policy analysis results.
%
{\oursystem} identifies 
a) whether apps integrate TPLs in their code without disclosure in privacy policies and 
b) whether TPLs access sensitive PI without descriptions.
%
We randomly selected 256 apps to annotate the privacy policies and evaluate the identification performance.
%
To annotate the privacy policies, one expert and senior researcher, who have conducted research on privacy policy and software engineering for over seven years and two years respectively, manually label the sentences that include data usage, TPL usage and data interaction wit TPLs.
%
The annotation process is conduct in an in-house manner~\cite{sorokin2008utility} that guarantees the quality and agreement of the labels.
% Then, we manually labeled privacy policies that include the data usage, TPL usage and data interaction with TPLs.
%


{\oursystem} identifies 65.63\% (168/256) apps violating the regulation requirements, i.e., their privacy policies miss disclosing TPL usage in their privacy policies.
%
Fig.~\ref{fig:miss_tpl} shows the most popular 15 TPLs that are missed being disclosed by host apps.
%
It can be observed that over 25\% of concealed data leakage is related to the TPL (\textit{"com.alipay"}). % developed by \textit{Alipay}. %, which is one of the most popular IT companies in China.
%
Among concealed data interaction with TPLs, the most popular PI data, that the app interacts with TPL but not discloses in the PP, are \textit{device ID}, \textit{mac address}, and \textit{sim serial number}, which account for 95.82\% (321/335) conflicts.







To this end, we also evaluate the performance of {\oursystem}.
%
We evaluate the eight metrics (i.e., true-positive, true-negative, false-positive, false-negative, accuracy, recall, precision and F1-score) concerning the identification performance of {\oursystem} on a) identifying the mis-disclosure of TPLs in host apps' privacy policy and b) identifying the mis-disclosure of PI interaction with TPLs (Tab.~\ref{tab:metrics}).
%
To calculate the metrics, we manually labeled host apps' privacy policies related to TPL usage and PI interaction with TPLs.
%
The ground truth of the TPL list is obtained from {\appbrain}.
%
It is not easy to access the ground truth of host apps sharing what kinds of Pi with which TPL. We can only identify the existence of the identified TPL list or PI interaction with TPLs in privacy policies.
%
Thus, we can only identify the false-positive rate of host apps' data interaction with TPLs, i.e., the detected usage in apps' code is not disclosed in privacy policies.
%
Tab.~\ref{tab:metrics} demonstrates that {\oursystem} achieves 95\% F1 score for identifying used TPL in apps and privacy policies, and achieve  95\% accuracy for identifying apps' PI interaction with TPLs.

\answer{4}{
{\oursystem} identifies over 65\% apps complain  the regulations requirements for disclosing apps data interaction with TPLs.
}
%
% todo: build a table/figure; illustrate the 
% 不一致的数量，这些不一致性存在在多少app中，主要是哪些数据，来自哪些tpl






% \begin{itemize}
%     \item analyze the consistency with labels in appbrain and apps privacy policy
%     \item analyze the consistency with pp analysis results and apps privacy policy
% \end{itemize}
% %
% To figure out whether the TPLs privacy policy clearly states the usage of sensitive personal information (PI), we first built a data set based on the {\appbrain}.
% % 
% Specifically, we crawl the website of each TPL in {\appbrain} and obtain the top ten apps that use the TPL.
% %
% Thus, we can obtain the 



% 介绍方法的准确率
% \input{table/atpchecker_metrics}
\begin{table}[t]
\vspace{3.5ex}
\centering
\smaller

\caption{Metrics of {\oursystem} for identifying host apps' interaction with TPLs}
\label{tab:metrics}
\begin{tabular}{@{}ccccc@{}}
\toprule
          & TP       & TN        & FN     & FP   \\ \midrule
TPL\_list & 95       & 0         & 0      & 9    \\
TPL\_data & 223      & /         & /      & 12    \\ \midrule
          & Accuracy & Precision & Recall & F1   \\ \midrule
TPL\_list & 0.91     &	0.91 &	1 &	0.95    \\
TPL\_data & 0.95 &	/ &	/ &	/
 \\ \bottomrule
\end{tabular}%
% \label{tab:metrics}
\vspace{-2ex}
\end{table}






==> tmp/experiments_old.tex <==
\section{Evaluation}

% \subsection{Dataset Collection and Experimental Setup}
\label{sec:dataset}

% \begin{comment}


\noindent\textbf{Collection of Third party libraries.}
We first get the TPLs from AppBrain~\cite{appbrain} that lists three types (Ad networks, social libraries and development tools) of TPLs that are used by top 500 apps (based on  installs) in Google Play. 
%
We collect a list of 458 TPLs that includes 141 ad networks, 25 social libraries and 292 development tools.
%
Based on the TPL list we get from AppBrain, we crawl the corresponding off-the-shelf TPL packages with the latest version file at the time from Maven Repository~\cite{mvnrepository} including the 85 \textit{``aar''} and 102 \textit{``jar''} files. 
%
In this way, we get 187 different TPLs from Maven Repository.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Collection of Host Apps.}
Meanwhile, the AppBrain also provides the mapping relations between the host app and its corresponding used in-app TPLs.
%
Based on the collected TPLs from AppBrain and the mapping relationship, we can pick out the host apps. 
%
For each TPL, we select the top 10 apps based on the installations and download these apps from Google Play. 
%
Finally, we collected a total of 642 distinct apps. Note that, some apps may use multiple TPLs and one TPL can be used by different apps.

\noindent\textbf{Privacy policies of TPLs.}
To get the privacy policies of TPLs listed in {\appbrain}, we visiting the homepage provided by each TPL information page on {\appbrain}.
%
For some TPLs, we can get the link of homepage of TPLs from {\appbrain}~\cite{appbrain}. 
For these TPLs we cannot get the homepage link from the {\appbrain}, we manually search their homepage by using search engine. 
For some open source TPLs, we can visit these published repositories (e.g., Github~\cite{github}, Bitbucket~\cite{bitbucket}) and check the privacy policies from their repositories. 





We manually collect TPLs' privacy policy to analyze whether their data usage are consistent with privacy policies.
%
Specifically, we manually visit the home page of target TPLs list in {\appbrain}~\cite{appbrain}.
%
Then, we search the homepage with keywords: \textit{privacy, policy, legal, and policies}.
%
For one TPL whose homepage does not give in {\appbrain}, we manually search its website.
%
For open source TPLs that are published in Github, we also visit their repositories to search their privacy policy.
% 

\revise{Finally, we collect 227 unique privacy policy as some TPLs are built by the same companies or developers.
%
In details, 112 out of 141 are related to network libraries (19 of which are not written in English), 103 out of 292 are development (7 not in English) and 12 out of 25 are social libraries (13 not in English).}
% \xiancm{rewrite this part to let the two part data consistency}
% 
\revise{Besides, we also use a snowball method~\cite{johnson2014snowball} to collect Chinese version privacy policy dataset.
%
Specifically, we analyze the privacy policy of host apps and extract the related TPL names. % (Figure~\ref{fig:pp_tpl_list}).
%
For the TPLs that provide privacy policy website, we directly crawl them, and for the TPLs without web site, we save the TPL name first and then manually search the privacy policy website as aforementioned.}




\noindent\textbf{Host apps of TPLs.}
\revise{To analyze whether the {\app}s use TPLs correctly, we collect top 10 host apps listed in {\appbrain} for each TPL.
%
We collect a total of 855 distinct apps as some apps may use multiple TPLs.}\xiancm{the process is not correct}


%First, we download 500 most popular apps from Google play as of 19 January.

%2) For aforementioned 775 TPLs, we download the apps that  listed in AppBrain. Specifically, for each TPLs, we download TOP 10 apps that contain target TPL.


\noindent\textbf{Privacy policies of host apps.}
% We also collect the privacy policy of host apps to analyze whether the app's data collection and sharing behavior are consistent with their statements in privacy policy and whether they clearly clarify the usage of
%We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with their statements in privacy policies, and whether they clearly disclose the usage of TPLs.
%
%After obtaining the host apps' package name from AppBrain, we crawl the privacy policies of apps from Google Play~\cite{googleplay}.
%
%Finally, we collect 642 host apps' privacy policies.
%
% TPLs correctly and consistent with the statements of TPLs' privacy policy.
We also collect the privacy policy of host apps to analyze whether the apps' data usage behavior are consistent with the privacy policies and violate the regulation requirements or not. For each host app in our dataset, we can get its privacy policy by crawling the homepage from Google Play.

% \end{comment}


We evaluate the performance of {\oursystem} by answering the following research questions:

\noindent\textbf{RQ1: Normativeness Analysis of TPLs.} 
%
\textit{How many TPLs provide privacy policy documents?} 
%
% This research 


% \noindent\textbf{RQ2: TPLs' privacy policy analysis.} 
% %
% \textit{Whether do TPLs' privacy policies correct claim data usage actions?}


\noindent\textbf{RQ2: Legality Analysis of TPLs.}  
%
\textit{Whether do TPLs' privacy policies meet regulation requirements and whether do TPLs' privacy policies correctly claim data usage actions?}


% %
% \noindent\textbf{RQ2: TPL privacy policy analysis.} Whether do TPLs contain privacy policies, and are privacy policies consistent with their behavior?

%
\noindent\textbf{RQ3: Host {\app}s behavior analysis.} \textit{Whether do host {\app}s conduct privacy data interaction with TPLs?}
% xian: 这里改为主要和TPL的数据交互行为，哪些违反 pp、哪些 regulation

%
\noindent\textbf{
% RQ4: Host {\app}s privacy policy analysis.
RQ4: Legality of host app's privacy policies.
} 
\textit{Whether do host app's privacy policies meet  requirements for disclosure of TPL usage?}




\input{table/TPL_without_PP_list}

\subsection{RQ1: Normativeness Analysis of TPLs.}
\label{sec:rq1}


\noindent\textbf{Experimental Setup.}
This research question covers all Android TPLs listed in AppBrain~\cite{appbrain} that lists three types (i.e., Ad networks, social libraries and developmetn tool).
%
The list gives the TPLs that are widely used by top 500 installed apps in Google Play.
%
The data set includes 458 TPLs that includes 141 ad networks, 25 social libraries and 292 development tools.
%
%
Then, we gather the privacy policies of those TPLs through visiting the homepage provided by each TPL information page on AppBrain.
%
For TPLs without homepage links, we manually search their information.
%
For open source TPLs that published in Github or Bitbucked, we visit their public repositories and check whether the privacy policies are provided.
%
During visiting the homepage of TPLs, we search the homepage with keywords, such as \textit{privacy, policy, legal} and \textit{policies} to find potential privacy policy links in the homepage. 
%
Besides, we also manually check whether privacy policy links are given at common layout~\cite{harkous2018polisis}, such as the bottom of the website.
%
Finally, we collect 201 unique privacy policies as some TPLs are built by the same companies or developers.



\noindent\textbf{Results.}
%
According to regulation requirements (\S~\ref{sec:bb_regulation_req}), data controllers should clearly disclose their data usage in their privacy policies.
%
When {\app}s build their functionalities based on TPLs, TPLs take on the role of data controllers~\cite{gdpr, ccpa,piss}.
%
% Besides, GDPR and CCPA also regard TPLs as data controller in their Articles.
%
This research question figures out whether TPLs satisfy the requirements of regulations, i.e., whether TPLs provide privacy policies.
%
%In this research question, we concentrates on the TPLs listed in AppBrain and TPLs list that we obtained through the snowball search.




% {\oursystem} analyzes publicly used TPLs as are listed in {\appbrain}~\cite{appbrain} that include three categories: Ad networks, social libraries, and development tool.
%
With the collected TPL list and TPL's privacy policy collection methods described in \S\ref{sec:dataset}, {\oursystem} discovers that 2 of 141 Ad network TPLs, 2 of 25 social libraries, and 103 of 292 development tools TPLs do not provide the privacy policy websites.
%
Besides, we observe that some TPLs are created by individual developers and released in {\github}~\cite{github}.
%
For {\github} repositories, we manually crawl their privacy policies with the data gathering method in \S\ref{sec:dataset}.
%
Table~\ref{tab:tpl_no_pp} summarizes the TPL name and the reasons that the TPLs do not provide privacy policies.
%
Table~\ref{tab:tpl_no_pp} demonstrates that 16 of 22 TPLs that do not provide privacy policies are published as Github repositories (GNP).
%
The TPLs are mainly developed by single developers to provide functionalities for other developers.
%
5 TPLs without privacy policies miss official websites (NOS), and the left does not provide privacy policy documents on their websites (NPOS).
%
For development tool TPLs, we also observe that 66 TPLs from \textit{Google Inc.} share the same privacy policy~\cite{googlepp} that may lead to over claim the personal information usage for specific TPLs.
%
For 9 TPLs from Apache, six of them do not provide the privacy policies on their official websites and two of their websites are Not Found.



\begin{comment}


For Chinese version TPLs, we first collect the data set for analysis as {\appbrain} conducts the statistics mainly on English version TPLs. 
%
As there are no public available statistic websites for Chinese TPLs, we extract them through a snowball collections method~\cite{johnson2014snowball}. 
%
When we manually check the aforementioned privacy policies of TPLs, we also check whether the TPLs' privacy policy websites contain a Chinese version.
%
Besides, we also extract the TPL list from apps' privacy policy documents as some apps' privacy policies may provide the TPL list they used and the corresponding privacy policy links. 
% (Fig~\ref{fig:pp_tpl_list}).
%
When we analyze the Chinese privacy policies of {\app}s, once the privacy policy is an unseen TPL, we will add it to our dataset.
%
We also manually crawl TPLs without privacy policy hyperlinks in host apps' privacy policies.
%
Finally, we gather 130 TPLs, and 115 of them contain the privacy policies.
\end{comment}


\answer{1}{
{\oursystem} reveals  6\% TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
}



% \answer{1}{
% {\oursystem} finds that 6\% English TPLs and 11\% Chinese TPLs do not provide privacy policies. Over 14\% TPLs from the same company provide one general privacy policy.
% }



\begin{figure}[t]
    \centering
    \vspace{1ex}
    \includegraphics[width=0.44\textwidth]{figures/TPL_PP_data_freq.pdf}
    % \vspace{1ex}

    \caption{Popularity of data types that are used in TPLs' data flow and PP}
    \vspace{-1ex}
    \label{fig:tpl_data_freq}
\end{figure}


\subsection{RQ2: Legality Analysis of TPLs.}


\noindent\textbf{Experimental Setup.}
We first gather the TPLs from Maven Repository~\cite{mvnrepository} based on collected TPL list from AppBrain (\S\ref{sec:rq1}).
%
We get 187 different TPLs that include 85 "aar" and 102 "jar" files.
%
More specifically, we get 45 ad networks, 132 development tool libraries and 10 social libraries.




\noindent\textbf{Results.}
{\oursystem} analyzes whether the TPLs' privacy policies satisfy the regulation requirements by comparing TPLs' functionality (\S\ref{sec:tpl_data}) and privacy policies (\S~\ref{sec:tpl_pp}).
%
% To analyze whether TPLs privacy policies clearly states the data usage, {\oursystem} analyzes 
%
{\oursystem} analyzes TPLs' privacy policies and obtains the ADUP of personal information usage-related statements.
%
{\oursystem} gets used personal information in the TPL through static analysis (\S\ref{sec:tpl_data}).
%
Finally, {\oursystem} matches the consistency between AUDP and personal information.



% \begin{figure}[t]
%     \centering
%     \vspace{1ex}
%     \includegraphics[width=0.47\textwidth]{figures/TPL_PP_data_freq.pdf}
%     % \vspace{1ex}

%     \caption{Popularity of data types that are most mentioned in TPLs' PP}
%     % \vspace{-2ex}
%     \label{fig:tpl_pp_data_freq}
% \end{figure}




\noindent\textbf{\textit{TPL privacy policies analysis.}}
%
{\oursystem} analyzes 187 unique TPLs' privacy policy documents.
%
We analyze 42,895 sentences with sharing and collection (SAC) words, and each privacy policy has an average of 420.5 sentences and 136 SAC words.
%
Among sentences with SAC words, 19,750 sentences start with 5W1H (\S\ref{sec:tpl_pp}) words that are not related to data usage actions.
%
Besides, 1654 sentences only vaguely state that the TPL will collect users' personal information rather than specific data types.
%
For example, $com.xiledsystems$  only claims \textit{"We collect your personal information in order to provide and continually improve our products and services"} but no specific personal information is  given.
%
In data usage-related actions, {\oursystem} analyzes the personal information (Table.~\ref{tab:data_type}) that are used by TPLs.
%
Figure.~\ref{fig:tpl_data_freq} shows the times that are mentioned in TPLs' privacy policies.
%
It can be observed that \textit{contact} are the most  used personal information.
%
This may be  caused by the fact that, by getting  users' contact, the TPLs can easily expand and prompt their services.
%
Account, address and email are the second-popular data that are mentioned in TPLs' privacy policies.
%
Among the statements that claim to collect users' accounts, addresses, and email, 21.13\% of sentences claim that they collect related data for contacting users. 
%
For example, one of them claims that \textit{"we will use your email, phone number, or other contact information you provide us by written or oral means for contacting you and providing you with the services and information that you request"}.









\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.40\textwidth]{figures/FCG_compare.pdf}
    \vspace{-1.5ex}
    \caption{Evaluation of function call graph construction}
    % \vspace{-2ex}
    \label{fig:fcg_compare}
\end{figure}


\vspace{1ex}
\noindent\textbf{\textit{TPL data usage analysis.}}
%% analyze whether our fcg construction method effective/improved
As the basic of our data flow analysis, we first evaluate the effectiveness of {\oursystem} on improving the FCG construction performance.
%
Specifically, we analyze TPLs' FCG quality by compare the a) FCG coverage and b) the number of edges between the raw FCG build by soot and our optimized FCG.
%
FCG coverage is calculated by:
%FCG coverage : the number of nodes in FCG/ the number of methods 
\begin{equation}
    \label{eq:fcg_cov}
    cov_{FCG} = \frac{\#Nodes_{FCG}}{\#Nodes_{TPL}},
\end{equation}
where $\#Nodes_{FCG}$ is the number of nodes (methods) in FCG and $\#Nodes_{TPL}$ is the total number of TPLs' methods.
%
Figure.~\ref{fig:fcg_compare} illustrates the box plots of {\oursystem}'s performance in  optimizing  FCG construction and the number at the top of boxes the denotes the measuring units of the data for better illustration.
%
Figure.~\ref{fig:fcg_compare} demonstrates that  {\oursystem}'s FCG coverage achieves an average performance of 55\%, while the FCG coverage of raw FCG only achieves an average of 0.34\%, which  means it nearly fails to construct the FCG of TPLS.
%
The $raw_{\#edge}$ denotes the raw FCG only contains the 159 average edges, while the ${\oursystem}_{\#edge}$ shows the improved FCG can extract 12,960 edges.
%
The results indicate that the soot nearly fails to analyze the FCG of TPLs, and {\oursystem}'s optimizes construction performance methods and improves the FCG quality.


% Then, 
{\oursystem} analyzes the data usage (\S\ref{sec:tpl_data}) of TPLs to identify the consistency with their privacy policy statements.
%
{\oursystem} analyzes the data flow of TPLs and discovers that 65 out of 187 TPLs access users' personal information.
%
{\oursystem} identify 146 data leakages from 2,396 traces.
%
Among data leakage behavior, 31 out of 146 invokes Android APIs (such as \textit{"<android.telephony.Tele-phonyManager: java.lang.String getSimSerialNumber()>"}) to access Android Sim Serial number.
%
Figure.~\ref{fig:tpl_data_freq} shows the data frequencies that are mostly used in TPLs' data flow (shown in orange color).
%
% It can also be observed that TPLs' privacy policies tend to disclose information that is not directly related to users' personal information, such as \textit{contact}, while their actions tend to access the information that is identical to the users, such as \textit{SimSerialNumber}.
It can also be observed that TPLs' privacy policies tend to disclose personally identical information, such as \textit{contact}, while their actions tend to access the information that is identical to the users, such as \textit{SimSerialNumber}.


\begin{figure}[t]
    \centering
    \vspace{1ex}
    \includegraphics[width=0.46\textwidth]{figures/tpl_propa.pdf}
    % \vspace{1ex}

    \caption{TPL Privacy Leakage Propagation}
    % \vspace{-2ex}
    \label{fig:tpl_pp_dep}
\end{figure}

% \begin{comment}


{\oursystem} identifies the compliance of TPLs by combing the privacy policies analysis results and data flow analysis results.
%
%  {\oursystem} identifies whether the personal information usage in TPLs' binary code are consistent with the statements that claim PI collections in their privacy policies.
%
Specifically, {\oursystem} identifies how many TPLs comply with regulations by identifying whether the PI in data flow are also mentioned in ADUP. 
%
{\oursystem} discovers that 37\% TPLs violate the regulation requirements, i.e., the TPLs collect at least one PI in their binary code  without clearly disclosing them in privacy policies.  
% \end{comment}

\vspace{1ex}
\noindent\textbf{\textbf{Investigation on perniciousness of TPLs' incompliant behavior.}}
%
After identifying TPLs that do not satisfy the regulation requirements, we also identify the  harm of TPLs' incompliant behavior on a large scale.
%
% It is well known that 
TPLs may integrate other TPLs to enhance their functionalities or facilitate usability~\cite{atvhunter2021ICSE}.
%
Thus, once one TPL ($TPL_v$) violates the law and carries potential data leakage vulnerabilities, other TPLs integrated $TPL_v$ may spread the vulnerabilities.
%
To expose the vulnerabilities, {\oursystem} analyzes the dependencies among TPLs .
%
Specifically, {\oursystem} crawls the TPLs that use vulnerable TPL ($TPL_v$), that are analyzed in \S\ref{sec:tpl_data}-\ref{sec:tpl_pp}, from {\maven}.
%
Then starting from these TPLs ($TPL_v$), {\oursystem} crawls the list of TPLs that integrate $TPL_U$.
%
In this way, {\oursystem} investigates the propagation of the vulnerabilities of TPLs under two-times invocations and visualizes it in Fig.~\ref{fig:tpl_pp_dep}.
%
% Specifically, 
{\oursystem} starts analysis with 25 unconventional TPLs.
%
Fig~\ref{fig:tpl_pp_dep} demonstrates the harm of that privacy leakage propagation 
% (i.e., the TPL is directly used by another TPL) 
with five selected TPLs.  
%
It can be observed that after one round of propagation, even five TPLs will affect 24,737 TPLs (25 TPLs affects extra 79,471 TPLs). After two rounds of propagation, the vulnerabilities even spread to 18,323 TPLs (25 to 447,300).
%
Fig.~\ref{fig:tpl_pp_dep} also demonstrates that not only the popular TPLs demonstrate infective (be widely used by other TPLs), such as \textit{"common-io/commons-io"}
% developed by \textit{apache}
,  some minority TPLs, such as \textit{"com.google.gdata/gdata-clien"} are directly used by only 11 TPLs.
%
After two rounds of propagation, the number of TPLs they affect is also growing exponentially.
%
This observation inspires us that developers should pay attention to the usage data of TPLs, especially the functions that are related to privacy.


% \subsection{Legality of TPLs}



\answer{2}{
{\oursystem} identifies over 37\% TPLs miss disclosing their data usage in privacy policy documents.
%
{\oursystem} investigates that the perniciousness of potential data leakage behavior in privacy policy spread exponentially.
}


\subsection{RQ3: Host apps behavior analysis}
\label{sec:rq3}

\noindent\textbf{Experimental Setup.}
%
We collect the host apps of TPLs from AppBrain to investigate host apps' interaction with TPLs.
%
We gather the host app list using the mapping relations between host apps and used in-app TPLs provided in AppBrain.
%
We can access top ten installation host app list for each TPL and then download the apps.
%
Finally, we gather a total of 642 distinct apps because some apps may use multiple TPLs and on TPL can be used by different apps.






\noindent\textbf{Results.}
{\oursystem} uses data flow analysis to investigate whether host apps conduct personal information interaction with TPLs and what kinds of PI are shared with TPLs.
%
{\oursystem} analyzes 642 distinct apps with labels, i.e., which TPLs are used.
%
% {\oursystem} analyzes the data flow of apps (\S\ref{sec:host_app_data}).
%
% Besides, we also collect 256 extra apps with Chinese privacy policies for analysis.




\begin{figure}[t]
    \centering
    % \vspace{1ex}
    \includegraphics[width=0.4\textwidth]{figures/host_app_TPL_data_interaction.pdf}
    % \vspace{-1ex}
    \caption{Statistics of host apps' interaction with TPLs}
    % \vspace{-2ex}
    \label{fig:app_int_tpl}
\end{figure}


{\oursystem} identifies over 60.5\% host apps share PI with TPLs and as is illustrated in Figure~\ref{fig:app_int_tpl}.
%
{\oursystem} traces 2,216 data sharing behaviors with TPLs and finds that over 53.1\% traces share users' \textit{sim serial number} with TPLs such as \textit{"com.google.android.gms", "com.applovin", "com.onesignal"}.
%
Although \textit{"com.google.android.gms"} is a well know TPL that provides users abundant Google services, the sharing of \textit{sim serial number} is sensitive to identify one individual.
%
Figure.~\ref{fig:app_int_tpl} demonstrates the top five data shared by host apps with TPLs.
% 
Figure.~\ref{fig:app_int_tpl} shows that the secondary data the host app need to share with TPLs is network status as TPLs will need to connect with host apps to provide services, like advertising or data analytic.
%
{\oursystem} also observes that \textit{"com.google.android.gms"} is the TPL that accesses the most PI from host apps.
%
% Although \textit{"com.google.android.gms"} provides abundant functionalities such as gmail, music, TPLs should avoid collecting information like SIM serial number that is easy to identify an individual.
%
TPLs should not ask for more data than is required for the content of their services~\cite{zhSDKLaw,gdpr,ccpa,piss}.




\answer{3}{
{\oursystem} identifies that over 60.5\%  of  host apps share personal information with TPLs.
%
Among shared PI, sim serial number accounts for over 53.1\%  of traces in identified data leakage actions.
%
{\oursystem} also discovers that while well-known TPLs provide rich functionalities, they also request the most personal information.
}


\begin{figure}[t]
    \centering
    % \vspace{-2ex}
    \includegraphics[width=0.42\textwidth]{figures/mssing_TPL.pdf}
    % \vspace{-1.5ex}
    \caption{Statistics of missing TPLs in host apps' PP}
    % \vspace{-2ex}
    \label{fig:miss_tpl}
\end{figure}


\subsection{RQ4: Host apps privacy policy analysis.}
\label{exp:host_app_pp}




{\oursystem} identifies whether host apps' privacy policies complain regulation requirements concerning descriptions about TPLs by analyzing whether privacy policies disclosure their usage and interaction with TPLs.
%
% {\oursystem} discovers the problems of privacy policy descriptions concerning TPL usage by combining the static analysis results (\S\ref{sec:rq3}) and privacy policy analysis results.
{\oursystem} achieves this goal by discovering the problems of privacy policy descriptions concerning TPL usage by combining the static analysis results (\S\ref{sec:rq3}) and privacy policy analysis results.
%
{\oursystem} identifies 
a) whether the apps integrate TPLs in their code without disclosure in privacy policies and 
b) whether the TPLs access sensitive PI without descriptions.
%
We randomly selected 256 apps with privacy policies to evaluate the identification performance.
%
Then, we manually labeled privacy policies that include the data usage, TPL usage and data interaction with TPLs.
%


{\oursystem} identifies 65.63\% (168/256) apps violating the regulation requirements, i.e., their privacy policies miss disclosing TPL usage in their privacy policies.
%
Figure.~\ref{fig:miss_tpl} shows the most popular 15 TPLs that are missed being disclosed by host apps.
%
It can be observed that over 25\% of concealed data leakage is related to the TPL (\textit{"com.alipay"}). % developed by \textit{Alipay}. %, which is one of the most popular IT companies in China.
%
Among concealed data interaction with TPLs, the most popular PI data, that the app interacts with TPL but not disclosures in the PP, are \textit{device ID}, \textit{mac address}, and \textit{sim serial number} that account for 95.82\% (321/335) conflicts.







To this end, we also evaluate the performance of {\oursystem}.
%
We evaluate the eight metrics (i.e., true-positive, true-negative, false-positive, false-negative, accuracy, recall, precision and F1-score) concerning the identification performance of {\oursystem} on a) identifying the mis-disclosure of TPLs in host apps' privacy policy and b) identifying the mis-disclosure of PI interaction with TPLs (Table~\ref{tab:metrics}).
%
To calculate the metrics, we manually labeled host apps' privacy policies related to TPL usage and PI interaction with TPLs.
%
The ground truth of the TPL list is obtained from {\appbrain}.
%
It not easy to access the ground truth of host apps sharing what kinds of Pi with which TPL. We can only identify the existence of the identified TPL list or PI interaction with TPLs in privacy policies.
%
Thus, we can only identify the false-positive rate, i.e., the detected usage in apps' code is not disclosed in privacy policies.
%
Table~\ref{tab:metrics} demonstrates that {\oursystem} can achieves over 95\% F1 score for identifying used TPL in apps and privacy policies, and achieve over 97\% F1 score for identifying apps' PI interaction with TPLs.

\answer{4}{
{\oursystem} identifies over 65\% apps complain  the regulations requirements for disclosing apps data interaction with TPLs.
%

}
%
% todo: build a table/figure; illustrate the 
% 不一致的数量，这些不一致性存在在多少app中，主要是哪些数据，来自哪些tpl






% \begin{itemize}
%     \item analyze the consistency with labels in appbrain and apps privacy policy
%     \item analyze the consistency with pp analysis results and apps privacy policy
% \end{itemize}
% %
% To figure out whether the TPLs privacy policy clearly states the usage of sensitive personal information (PI), we first built a data set based on the {\appbrain}.
% % 
% Specifically, we crawl the website of each TPL in {\appbrain} and obtain the top ten apps that use the TPL.
% %
% Thus, we can obtain the 



% 介绍方法的准确率
% \input{table/atpchecker_metrics}
\begin{table}[t]
\vspace{3.5ex}
\centering
\smaller

\caption{Metrics of {\oursystem} for identifying host apps' interaction with TPLs}
\label{tab:metrics}
\begin{tabular}{@{}ccccc@{}}
\toprule
          & TP       & TN        & FN     & FP   \\ \midrule
TPL\_list & 95       & 0         & 0      & 9    \\
TPL\_data & 223      & 0         & 0      & 12    \\ \midrule
          & Accuracy & Precision & Recall & F1   \\ \midrule
TPL\_list & 0.91     &	0.91 &	1 &	0.95    \\
TPL\_data & 0.95 &	0.95 &	1 &	0.97
 \\ \bottomrule
\end{tabular}%
% \label{tab:metrics}
\vspace{-2ex}
\end{table}




==> tmp/intro_1208.tex <==
\section{Introduction}

% \input{table/regulation_summary}


% \vspace{0.5em}
% \begin{quote}
%     \emph{\textbf{``Hedges have eyes and walls have ears.''}}
%     \begin{flushright}
%     - Trusler, John, 1735-1820.
%     \end{flushright}
% \end{quote}
% \vspace{1em}



\begin{comment}


% Nowadays, the smartphone is ubiquitous, and mobile apps, as a significant part of mobile ecology, are playing essential roles in our daily life, from living, working, and education to business~\cite{deepintent2019SIGSAC}. 
Nowadays, the smartphone and mobile apps are playing essential roles in our daily lives~\cite{deepintent2019SIGSAC}. 
% \xiancm{suggest use daily lives}
Besides, more and more developers tend to use many off-the-shelf 
% \revise{toolkits or}\xiancm{can delete this part, we just say TPLs is ok , let everything close to your topic}
third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE,libdetect2020ASE}.
% Have you ever thought about the security of these third-party libraries (TPLs) used in your apps? 
% TPLs probably leak your personal privacy. 
%
However, developers may omit the privacy threat in TPLs. 
%
For example, the advertisement libraries may leak users' personal information (e.g., IMEI)~\cite{short2014android}.
%
Some TPLs (e.g., advertising and analytic libraries) rely on the personal information to provide better service~\cite{demetriou2016free}.
% \xiancm{add reference here} 
%
However, some TPLs may collect user data that is not necessary for providing related services. 
Such behaviors may lead to privacy leakage or even security concerns~\cite{deepintent2019SIGSAC, harty2021logging, tangtse:21a}.
%
% However, behaviors of those TPLs are undesirable or even harmful, including disclosing users' sensitive information such as location and personal profiles without informing users~\cite{deepintent2019SIGSAC,harty2021logging, tangtse:21a, tang:ase19}. 
%
% For the dominant mobile operating system Android~\cite{mobile_operating_system}, \xiancm{rewrite this sentence but should delete this sentence}\xian{Nowadays, Android, as the dominate mobile operating system~\cite{mobile_operating_system}}\xiancm{even that, IMHO, I still cannot find the connection between the two sentences, Android as the dominant mobile operation system so? why this can lead to the permission mechanism issues??}
% Android, the privacy leakage from TPLs is more serious.
% the permission mechanism also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}. 
% \xian{
Besides, the permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}.
% }
%
Since the host apps share the same process space and permissions with TPLs, 
% the mechanism  leads to over-privileged TPLs. 
% \xian{
the mechanism violates the principle of least privilege, which leads to TPLs is over-privileged.
% }
%
Recent papers find that the permissions abuse makes TPLs access users' personal information and causes potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
%
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} may cause serious personal information leakage. 
% from host apps. 
%
For example, a recent report~\cite{cybernews_dataleakage} discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties. 
%
Zhang et al.~\cite{zhang2020does} disclose 120 of 555 apps that share users' personal information to analytic service TPLs without encryption.
%
Besides, linking and mining large amounts of unencrypted personal information probably pose threats to serious personal privacy leakage~\cite{kiranmayi2018reducing, chen2014information}.
% will \xiancm{pay attention to the accurate expression, do that may cause but not necessary}\revise{lead to}\xian{probably pose threats to} serious personal privacy leakage~\cite{kiranmayi2018reducing, chen2014information}.
%
% Thus, it is urgent to identify TPLs' data sharing and collection actions to protect user privacy.
Thus, it is urgent to design a system to check the data access behavior and privacy policies of TPLs so that we can determine if TPLs are compliant with the privacy regulations or not.

%analyze the compliance of TPLs data access behavior and privacy policies with regulations to protect user privacy.
%
% Even the unencrypted personal data are only shared with trusted TPLs that do not abuse the data, linking and mining of a large amount of unencrypted personal information also could lead to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
% }
\end{comment}

Nowadays, the smartphone and mobile apps are playing essential roles in our daily lives~\cite{deepintent2019SIGSAC}. 
%
Besides, more and more developers tend to use many off-the-shelf 
%
third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE,libdetect2020ASE}.
%
However, developers may omit the privacy threat in TPLs. %
For example, the advertisement libraries may leak users' personal information (e.g., IMEI)~\cite{short2014android}.
%
Some TPLs (e.g., advertising and analytic libraries) rely on the personal information to provide better service~\cite{demetriou2016free}.
%
However, TPLs may collect user data that is not necessary for providing related services. 
Such behaviors may lead to privacy leakage or even security concerns~\cite{harty2021logging, tangtse:21a}.
%
Besides, the permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}.
%
Since the host apps share the same process space and permissions with TPLs, 
%
the mechanism violates the principle of least privilege, which leads to TPLs being over-privileged.
%
Recent papers find that permission abuse makes TPLs access users' personal information and causes potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
%
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} may cause serious personal information leakage. 
%
For example, a recent report~\cite{cybernews_dataleakage} discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties. 
%
Zhang et al.~\cite{zhang2020does} disclose 120 of 555 apps that share users' personal information to analytic service TPLs without encryption.
%
Besides, linking and mining large amounts of unencrypted personal information probably pose threats to serious personal privacy leakage~\cite{kiranmayi2018reducing, chen2014information}.
%
Thus, it is urgent to design a system to check the data access behavior and privacy policies of TPLs so that we can determine if TPLs are compliant with the privacy regulations or not.


% To normalize apps' behaviors and prevent privacy leakage, various personal privacy  protection-related regulations (e.g., CCPA, CPRA, GDPR, ICCPR)~\cite{piss, zhSDKLaw, gdpr, ccpa} have been promulgated to protect people's personal information from abuse, which requires developers to clearly understand TPL behaviors and declare these sensitive behaviors in their privacy policy so as not to violate the regulations.
%
To normalize 
% software's 
privacy-related behaviors and prevent privacy leakage, various privacy-related regulations 
% (e.g., CCPA, CPRA, GDPR, ICCPR, CFR)~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr}
(e.g., {\textsc{\small{California Consumer Privacy Act (CCPA), General Data Protection Regulation (GDPR)}}})~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr})
have been promulgated to protect people's personal information from being abused.
%
% \revise{
% However, app developers may unconsciously violate regulations since they cannot understand all TPLs' functionalities and do not have privacy-related background knowledge.}\xiancm{rewrite} \xian{
However, app developers may unconsciously violate regulations of used TPLs because they do not need to understand the execution logic of these TPLs, they just need to follow the user guidelines to invoke these TPLs. Due to a lack of security consciousness, developers may never check whether these used TPLs in their apps have a privacy policy and whether these TPLs may have security risks with respect to privacy leakage. 
% }
%
The latest \textit{\small{Google Play Developer Program policies (GPDP)}}~\cite{google_play_pp_update} ask developers to ensure the TPLs used in their apps are compliant with GPDP~\cite{gpdp}.
% 
% Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}. 
%
Developers of {\tpl}s are required to provide privacy policies and disclose data usage.
%
Otherwise, the apps violate regulation or market's requirements and they may be removed from the app market~\cite{googleplay_requirements, appgallery_requirements}.
% are queried to withdraw the apps. 
%
To help TPLs comply with regulations and help developers correctly use TPLs,  it is necessary to analyze the consistency between {\tpl}s' data usage and privacy policies.

% \revise{To make {\tpl}s comply with regulations and help developers correctly use {\tpl}s, it is necessary to analyze the consistency between {\tpl}s' data usage and privacy policies.}\xiancm{the logic is not ok, you cannot make the TPL comply with the regulations, you are not the authors, or developers of TPLs, you just want to conduct the analysis, how do you make the TPLs comply with the regulations}


Previous work~\cite{ppcheck,ppchecker,andow2019policylint, yu2016can,nguyen2021share,zhang2020does,wang2021understanding} has proposed methods to analyze privacy issues of apps, such as analyzing the consistency between apps privacy policy descriptions and behaviors.
%
However, existing methods cannot identify the app's privacy issues related to the usage of TPLs inside apps because existing methods fail to identify TPLs functionalities or analyze TPL privacy policies.
%
PoliCheck~\cite{ppcheck} performs dynamic analysis to get traffic flow for analyzing the apps' data usage.
Then, it applies data and entity dependency tree analysis to extract data usage statements from the privacy policy, and designs rules to identify the conflicts.
%
PPChecker~\cite{ppchecker} discovers the trustworthiness of apps' privacy policies, and identifies consistency of app's behavior and privacy policy statements and the consistency of privacy policies from different sources.
%
PPChecker concentrates on apps' privacy policies and is out-of-dated to satisfy the latest regulations.


\begin{comment}

% 介绍现有的 app pp 分析
% Recent research~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding} propose methods to identify the legality of apps, i.e., the apps are required to disclose personal information usage in their privacy policies. 
%
% \revise{Some methods have been proposed to identify the privacy issues\xiancm{privacy issues are not equal to privacy policy analysis, which one you want to say ,use accurate expression} of mobile apps~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding}.}\xiancm{based on your comments, I can see you want to say the pp analysis of app based on previous research. however, the key issues is that the privacy issues are not equal to pp analysis, your English still need to improve. please learn my English writing}
%
However, they cannot identify the conflict between TPLs and regulations because they either failed to identify TPLs functionalities or analyze TPL privacy policies.   
% \xiancm{the logic of this sentence is totally incorrect, current work cannot identify the conflict between TPLs and regulations, we need to analysis the conflicts between TPLs' behaviors and regulations, this is one solution. but failed to analyze policies cannot solve your issues. there are several conflicts, the behaviors between the TPLs' behaviors and pp, the tpls' behaviors and regulations, the pp and regulations. so we need to give a clear target at the beginning, and then we just can organize our paper}
% 
% However, those systems can not identify TPL-related privacy leakage issues because the systems miss analyzing TPL functionalities and privacy policies, and analyzing the consistency between TPLs' code and privacy policy statements.
%
PoliCheck~\cite{ppcheck} performs dynamic analysis to get traffic flow for analyzing the apps' data usage.
Then, it applies data and entity dependency tree analysis to extract data usage statements from the privacy policy, and designs rules to identify the conflicts. \xiancm{this part is about the app pp analysis}
% checks the consistency between the apps' data collection and sharing behaviors with the privacy policy.
%
PAMDRroid~\cite{zhang2020does} identifies the TPLs' misconfiguration caused by personally identifiable information (PII) leakage.
%
PAMDroid investigates whether the PII is preprocessed, such as anonymization and encryption, before sharing with analytic service libraries. \xiancm{this one is about the TPL misconfiguration analysis}
%
PPChecker~\cite{ppchecker} discovers the trustworthiness of apps' privacy policies, and identifies consistency of app's behavior and privacy policy statements and the consistency of privacy policies from different sources.
% Specifically, PPChecker identifies a) whether apps' privacy policies cover all apps' personal information (PI) usage behaviors (\textbf{completeness}), b) whether apps' privacy policies correctly claim the personal information(PI) that the app uses or does not use (\textbf{correctness}), c) whether privacy policies' description uses vague words (\textbf{preciseness}), d) whether apps' privacy policies consistent other sources, such as TPL and Google Play, (\textbf{consistency}), and e) whether the privacy policies are easy-to-read.
%
PPChecker concentrates on apps' privacy policies and is out-of-dated to satisfy the latest regulations.\xiancm{and this one is about tht app pp analysis agin}
% Existing methods can not identify TPL-related regulation violations since they 
\xiancm{have you found your writing issues, the logic is not fluent and coherent, the TPL and app pp analysis are across each other, the logic is not ok. If I were you, I will write the app pp analysis first and then give the status quo of tpl pp analysis and the present the research gap so that we can introduce our tool}


\xiancm{I rewrite this part but also need to your help to summarize two papers which also talk about the pp analysis on tpls}

\xianw{The most earlier research usually focus on the privacy policy analysis of mobile apps~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding}. In sum, previous studies mainly can divided into four directions: 1) inconsistent analysis between privacy policy and apps' behaviors, 2) inconsistent analysis between regulations and apps' behaviors, 3) inconsistent analysis between privacy policy and regulations, 4) automatic generate privacy policy for apps. Recently, more and more researchers started to focus on privacy policy analysis of TPLs as well. PAMDRroid~\cite{zhang2020does} mainly focuses on the personally identifiable information (PII) leakage due to misconfiguration from analytic service libraries.
\xiancm{Besides, please summary the two papers}
\xian{X. Liu, J. Liu, S. Zhu, W. Wang and X. Zhang, "Privacy Risk Analysis and Mitigation of Analytics Libraries in the Android Ecosystem," in IEEE Transactions on Mobile Computing, vol. 19, no. 5, pp. 1184-1199, 1 May 2020, doi: 10.1109/TMC.2019.2903186.
%%%
%%
C. Schindler, M. Atas, T. Strametz, J. Feiner and R. Hofer, "Privacy Leak Identification in Third-Party Android Libraries," 2022 Seventh International Conference On Mobile And Secure Services (MobiSecServ), February 2022, pp. 1-6, doi: 10.1109/MobiSecServ50855.2022.9727217.}
}
\end{comment}


% Existing methods are limited to identifying the consistency between apps' behavior and privacy policies~\cite{yu2016revisiting,ppcheck,ppchecker} and ignore the regulation requirements for {\tpl}s.
% Existing methods can not identify TPL-related regulation violations 
%

Based on our study, we find there is still a research gap with respect to discrepancy analysis between the privacy related behaviors of TPLs and regulations. 
To this end, we propose a tool, named \oursystem ~(\underline{\textbf{A}}utomated \underline{\textbf{T}}hird-party library \underline{\textbf{P}}rivacy leakage \underline{\textbf{Checker}}) to automatically  check whether the usages of in-app TPLs complies with privacy-related regulations (e.g., {GDPR Article I.(47), COPPA 312.2, CFR 332.6}).
%
As regulation analysis requires expert knowledge of both legal and software engineering, we invited 
one expert and one senior researcher to help us read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. Both of them have conducted research on software engineering and privacy policy analysis with experience for over seven years and two years, respectively.
%
{\oursystem} identifies the inconsistency between TPL and regulation by analyzing TPL's bytecode (\S\ref{sec:tpl_data}) and privacy policies (\S\ref{sec:tpl_pp}).
%
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
%
{\oursystem} discloses whether host app's TPL usage comply with regulations(\S\ref{sec:host_app_data}, \S\ref{sec:host_app_pp}). 



\begin{comment}
To regulate TPL usage and help developers better understand TPLs' functionalities\xiancm{we cannot regulate TPL usage, because this work's purpose is to detect the conflicts, how we regulate the TPL usgae, they have many setup readme files can help users to use them}, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically check the consistency\xiancm{inconsistency} between regulation requirements and TPLs, and they determine whether the host app's usage of TPLs complies with regulations.\xiancm{two sentences is the same meaning, should combine and optimize it}
%
We analyze privacy and security-related laws~\cite{gdpr, ccpa, cpra,  piss,petitcolas1883cryptographie,iccpr}. 
% (\S\ref{sec:bb_regulation_req}).  
% 
%, and the regulations that normalizing software applications~\cite{zhSDKLaw} (\S\ref{sec:bb_regulation_req}). 
% 
We concentrate on TPL-related regulations, e.g., the scope of TPL (\textsc{\small{GDPR Article I.(47), COPPA 312.2}}), and requirements for TPL-related privacy policy statements (\textsc{\small{CFR 332.6}}).
%
\revise{As regulation analysis requires expert knowledge of both legal and software engineering, one expert and one senior researcher, who has conducted research on software engineering and privacy policy analysis for over seven years and two years, respectively, \xian{were invited to} read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. }\xiancm{delete the clause, the sentence is not coherent,}
%
{\oursystem} identifies the inconsistency between TPL and regulation by analyzing TPL's bytecode (\S\ref{sec:tpl_data}) and privacy policies (\S\ref{sec:tpl_pp}).
%
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
%
{\oursystem} discloses whether host app's TPL usage comply with regulations(\S\ref{sec:host_app_data}, \S\ref{sec:host_app_pp}). 
% checks the consistency between host app's privacy policies and TPL-related regulation requirements.
%
% By analyzing the host app's privacy policies and binary code, {\oursystem} identifies whether the host app's privacy policy clearly claims TPL usage.
% , e.g., what kinds of data are shared with TPLs rather than only identifying the existence of used TPLs' privacy links~\cite{ppchecker}. 
%
% {\oursystem} implements the following functionalities to achieve such goal and tackles the limitations of existing works accordingly.

\xiancm{I rewrote the above paragraph }

\xianw{Based on our study, we find there is still a research gap with respect to discrepancy analysis between the privacy related behaviors of TPLs and regulations. 
To this end, we propose a tool, named \oursystem ~(\underline{\textbf{A}}utomated \underline{\textbf{T}}hird-party library \underline{\textbf{P}}rivacy leakage \underline{\textbf{Checker}}) to automatically  check whether the usages of in-app TPLs complies with privacy-related regulations (e.g., {GDPR Article I.(47), COPPA 312.2, CFR 332.6}).
%
As regulation analysis requires expert knowledge of both legal and software engineering, we invited 
one expert and one senior researcher to help us read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. Both of them have conducted research on software engineering and privacy policy analysis with experience for over seven years and two years, respectively.
}

\end{comment}



\kaifa{
It is challenging to develop {\oursystem} due to multiple reasons.
%
First, it is non-trivial to get TPLs and corresponding privacy policies because TPLs are mainly published on open source repositories, such as Maven~\cite{mvnrepository} and github, which do not require developers to provide privacy policies to describe their user privacy access behaviors.
%
To counter this issue, we first construct a data set that contains TPL repository and host app repository.
%
The TPL repository contains a) a TPL list, which contains 458 TPLs crawled from {\appbrain}~\cite{appbrain},  b) 187 TPL's binary files from {\maven}~\cite{mvnrepository}, and c) 351 TPL's privacy policies which are manually collected.
%
The host app repository contains a) 642 distinct host apps which are collected from {Google Play} based on the list from {\appbrain} and b) the host app's privacy policies.
%
Second, it is not easy to analyze TPL's user privacy access behavior because TPLs are mainly provided in format of binary files, such as \textit{jar} and \textit{aar} in {\maven}, without source code and TPL's whole functions can not be executed independently without being triggered.
%
{\oursystem} performs static analysis~\cite{soot} to construct the TPL's function call graph and uses data flow analysis to trace TPLs personal information usage without source code (\S\ref{sec:tpl_data}).
% 
We do not conduct dynamic analysis since it cannot execute all possible paths in apps or TPLs~\cite{schindler2022privacy}.
%
Third, analyzing privacy policy is difficult because developers use various natural language to describe the usage of personal information and TPL.
%
To analyze data and TPL usage related statements of privacy policies, {\oursystem} implements an expert system to extract abstract data usage patterns (\S\ref{sec:host_app_pp}) and analyzes the compliance of TPL usage.
}


\begin{comment}
It is challenging to develop {\oursystem} due to multiple reasons.
%
First, no standardized data are publicly available for analyzing TPL compliance.
% no dataset is available for research in this area.
%
To counter this issue, we create a novel data set containing 187 TPLs and 642 distinct host apps.\xiancm{why this data is not match the abstract, one is 458 TPLs}
%
All TPLs' privacy policies are collected and annotated with labeled tokens. \xiancm{but you just collect 23\% of 458, why here you can say all?}
%\textbf{c}) 642 distinct host apps labeled with an integrated TPL list, and 
All host apps' privacy policies are also included.
% \textbf{b}) corresponding privacy policies with labeled tokens,
% \textbf{c}) 642 distinct host apps labeled with an integrated TPL list, and 
% \textbf{d}) corresponding host apps' privacy policies.
%
\revise{Second, it is non-trivial to get TPL data usage because TPLs are usually closed source. }
\xiancm{do you have any reference? or proofs? based on my knowledge, most TPLs are oss. most TPLs in an Android app are open-source as well}
\xiancm{why your challenges here cannot match the abstract you said. there are four challenges, but I think we can use two in abs, but why here you give two new}
% usually provided as compiled code without source code. 
% and it is challenging to trace data usage in close source TPLs. 
{\oursystem} performs static analysis~\cite{soot} to construct the TPL's function call graph and uses data flow analysis to trace TPLs personal information usage without source code (\S\ref{sec:tpl_data}).
% 
We do not conduct dynamic analysis since it cannot execute all possible paths in software~\cite{schindler2022privacy}.
%and it also requires executing the target software and analyzing the data changes during runtime.
%
Moreover, TPLs provide APIs that relies on the host app to trigger them. 
%
Dynamic analysis cannot execute the TPL directly.
%
% {\oursystem} uses static analysis~\cite{soot} to construct the TPL's function call graph, and uses data flow analysis to trace TPLs personal information usage (\S\ref{sec:tpl_data}).
% conducts data flow analysis(\S\ref{sec:tpl_data}).
%
Third, analyzing privacy policy is difficult because developers use various natural language to describe the usage of personal information and TPL.
\xiancm{why these challenges cannot match the abstract}
%
To analyze data and TPL usage related statements of privacy policies, {\oursystem} implements an expert system to extract abstract data usage patterns (\S\ref{sec:host_app_pp}) and analyzes the compliance of TPL usage.
\xiancm{there are several issues that make this paper choas. 1. do this paper should consider the single TPL, the independent TPL analysis, or we just consider the in-app TPLs, there are two different things, I do not understand the key targets that the paper want to handle. 
should we consider the pp analysis, but this paper say we just analyze the inconsistencies between TPLs and regulations? what do you means the TPLs here, the behaviors of TPLs, the TPLs consider as the independent software or a part of host app? I still not understand.
}
% {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
% {\oursystem} implements abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).



% \xiancm{based on your description the legality analysis is clearly say PI usage in PP in previous paragraph and this paragraph is to say ignore the regulation requirements analysis for TPLs, here, you did not say anything about that. need to detailed description about the functions involving the pp analysis and laws consistency analysis}
% \xiancm{Why \oursystem need to explain here}
%
% For legality identification, {\oursystem} checks whether the {\tpl} contains a privacy policy and uses static analysis to analyze its functionalities to identify the consistency with PP.
% %
% For correctness usage of {\tpl}s, {\oursystem} identifies 1) what {\tpl}s are used by host apps, 2) what kinds data are interacted with {\tpl}s, and 3) whether hosp apps' privacy policy clearly state {\tpl}s' data usage.
%
% \xiancm{I remember your paper need to consider the laws analysis, I cannot find any description about laws analysis in this introduction}
%However, there still exist challenges to be countered when designing {\oursystem}.
% \xian{To achieve such goals, we need to solve the following challenges:}
%



We address the following challenges in the development of {\oursystem}.
%
First, there is no available dataset for research in this area.
%
To counter this issue, we gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{d}) 642 distinct host apps labeled with an integrated TPL list and \textbf{f}) %642 
corresponding host apps' privacy policies.
%
% We will release the dataset after the paper gets published.
%
Second, it is non-trivial to track the data usage of TPLs because 1) TPLs are usually provided as compiled code without source code and 2) it is difficult to construct a call graph that contains all important edges (invocation relations)~\cite{reif2016call}.
%
To tackle the challenge, {\oursystem} is built on {\soot}~\cite{soot} that is a popular static analysis tool and does not require the source code.
%
To construct a comprehensive callgraph of the TPL to facilitate personal information track, {\oursystem} implements new methods (\S\ref{sec:tpl_data})  to optimize TPLs’ FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Third, privacy policy analysis remains challenging as a natural language processing task, because privacy policies use different patterns (\S\ref{sec:host_app_pp}) to describe the usage,and the usage of TPLs.% and data sharing with TPLs.
%
To counter the challenge, {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
{\oursystem} designs abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).
%





% \noindent\textbf{Availability of dataset.}


\noindent\textbf{Data leakage analysis in third-party  libraries.}
%
\xiancm{Based on your description, I cannot see any challenges here, challenges should be the point that difficult to solve, where is it}
As TPLs are usually provided as compiled code~\cite{qiu2021libcapsule} without source code, {\oursystem} uses {\soot}~\cite{soot} to analyze TPLs that does not require source code.
%
{\oursystem} applies static analysis to identify the data leakage in third-party libraries.
%
{\oursystem} analyzes the data flow of TPLs to identify the definition and usage chain~\cite{pande1994interprocedural} (\S\ref{sec:tpl_data}) of personal information (PI).
%
As {\oursystem} uses function call graphs (FCG) to better trace the usage of target variables, we propose new methods (\S\ref{sec:tpl_data}) to optimize TPLs' FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Excepting PI name matching with predefined data types, we also construct a mapping knowledge set that builds connections with PI name and Android APIs to improve the variable locating precision.
% 



% \noindent\textbf{Identification of host apps' PI interaction with TPLs.}
%
% \cite{wei2018amandroid}


\end{comment}



\begin{comment}

\noindent\textbf{TPL usage identification in host apps.}
%
Taint analysis is widely used to identify data leakage in software with predefined sources and sinks.
%
However, it is still a challenge to locate the destination of those data leakages while it is necessary to locate them to further identify the correctness of host apps' usage of TPLs. 
%
{\oursystem} first builds a knowledge set to match {\tpl} related invocations in binary code.% (\kaifa{revise it}).
%
Combining the data flow of personal information and {\tpl}s, {\oursystem} determines the destination of PI data (\S\ref{sec:host_app_data})

%
% \xiancm{I am dying if I just read more lines..... I do not know what are you doing...... many things are totally incorrect}
% \xiancm{The figure cannot show any useful information and ugly }
% % 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/tpl_enumeration_in_host_app_pp_new.png}
%     \caption{TPL usage in privacy policy of \textit{jp.ne.ibis.ibis-paintx.app}}
%     \label{fig:pp_tpl_list}
% \end{figure}


\noindent\textbf{TPL related statements extraction in host apps' privacy policies.}
%
\revise{Existing data-related statements extraction methods~\cite{ppcheck, andow2019policylint} are generally constructed on named entity recognition techniques that require a large amount of labeled corpus for model training.
%
Besides, existing methods are usually based on predefined sharing and collecting verbs to locate those data-related sentences. \xiancm{you just say the existing method, where is the challenges of your work}
%
Although those methods achieves desirable performance for analyzing apps' data collection statements in privacy policy, those methods may omit information related to {\tpl}s because host apps may provide {\tpl}s' information in form of table or enumeration.} \xiancm{this is limitation of existing work is not your work's challenges. logic chaos}
%(as is illustrated in 
% Fig.~\ref{fig:pp_table} and 
% Fig.~\ref{fig:pp_tpl_list} separately).  
%
Besides extending the existing sharing and collection words list to locate data usage-related statements in the privacy policy, {\oursystem} also designs \revise{heuristic patterns}\xiancm{when anytime you use heuristic you need to explain the heuristic patterns first} to precisely extract {\tpl} related statements for further flow-to-policy analysis.
\xiancm{I still cannot see any challenges here}



\end{comment}
% write a paragraph to summarize the performance of our tool

\vspace{0.5em}
Overall, our contributions are summarized as follows:


\begin{itemize}[leftmargin=*]


\item We propose a novel system named {\oursystem} to analyze the compliance of Android TPLs. 
%
{\oursystem} uses static analysis to identify TPL's user data access behavior and host apps' data interaction with TPLs, and uses  NLP techniques to analyze TPLs' and host apps' privacy policies.
% TPLs' personal information accessing both individually and inside host apps, and applies NLP techniques to analyze TPLs' and host apps' privacy policies.
%
Combining the results of bytecode analysis and privacy policy analysis, {\oursystem} determines whether TPLs and usage of TPLs in host apps comply with regulation. 


\item To evaluate the performance of {\oursystem} and facilitate further research in this area, we construct a privacy dataset that includes 187 TPL's binary code and their privacy policies, and 642 host apps and their privacy policies.
% 
Our dataset contains TPL's privacy policies with related data access behavior.
%
Our dataset includes host app's privacy policies that contains labels related to host app's interaction with TPLs.
% TPL's privacy policies in our data set contain labeled corpus related to TPLs' data accessing behavior and the host app's privacy policies are labeled with used TPLs and data interaction with TPLs.
%
% 
{\oursystem}'s website with instructions to request access is at:
\url{https://github.com/zacharykzhao/TPL-PP}.
% 

% \vspace{1em}
\item {\oursystem} discovers over 23\% of TPLs miss providing privacy policies, 37\% of TPL's privacy policies conceal data usage.
%
{\oursystem} discovers over 65\% of host apps violate the regulation requirements for disclosing data interactions with TPLs. 
% \item {\oursystem} discovers over 23\% (107 out of 458) of TPLs miss providing privacy policies, 37\% (24 out of 65) of TPL's privacy policies conceal data usage.
%
% {\oursystem} discovers over 65\% (168 out of 256) of host apps violate the regulation requirements for disclosing data interactions with TPLs. 



\end{itemize}









\begin{comment}
%
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.






This is introduction
\subsection{Our target}


\begin{itemize}
    \item We have to identify whether the action of {\tpl} is consistent with {\tpl}'s privacy policy.
     
    \item We need to detect all data usage (at least sensitive data usage) in APP. And specify which groups are used by app and which groups are used by {\tpl}.
    
    \item
\end{itemize}


Tool name: {\oursystem} Android Third party libraries misuse and Privacy policy conflict checker.

\subsection{Challenges}

\textbf{1. {\tpl} information extraction}: Information about the usage of {\tpl}, the data related to {\tpl} are usually formatted as a table or organized as form of explanations (for example, facebook: data1, data2 \kaifa{put a case study in Appendix}).
%
% We apply \texttt{Tablemaster} to extract information from tables and \kaifa{a new NLP technique} to merge information in form of explanations.
\kaifa{not suitable. I analyze 3502 privacy policy. Only 471/3502 privacy policy contains html tag \textit{table}. I manually checked 200/471. Only 6/200 contains table are related to data usage that cannot be analyzed by the method in PolicyLint.}

PolicyLint~\cite{andow2019policylint} deals with the table data by merging the formatted lists into sentences.
%
This preprocessing method fails when only noun phrase on the table because the method in PolicyLint directly merges the items together without considering the characteristics of table, i.e., the data in each item shares same attributes. \kaifa{give an example in appendix}
%


\textbf{2. Data analysis in third party libraries. }
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
For dynamic analysis,  we must find the apk that uses the {\tpl} and leverage the data usage of {\tpl}. 
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.
%
\kaifa{details, how to design such a tool}


\textbf{3. Consistency analysis} We focus on two aspect of consistency analysis: a) whether the app's privacy policy covers all {\tpl} usage. 
%
To relax condition, the app's privacy policy should contain all {\tpl}s that collect or share data.
%
b) If the app's privacy policy covers the {\tpl} usage, does the data usage in privacy policy consistent with the {\tpl}'s real data usage.

\end{comment}

==> tmp/intro_old.tex <==
\section{Introduction}

% \input{table/regulation_summary}


% \vspace{0.5em}
\begin{quote}
    \emph{\textbf{``Hedges have eyes and walls have ears.''}}
    \begin{flushright}
    - Trusler, John, 1735-1820.
    \end{flushright}
\end{quote}
% \vspace{1em}




Nowadays, smartphone is ubiquitous, and mobile apps, as a significant part of mobile ecology, are playing essential roles in our daily life, from living, working, education to  business~\cite{deepintent2019SIGSAC}. 
Besides, more and more developers tend to use many off-the-shelf toolkit or third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE,libdetect2020ASE}.
Have you ever thought about the security of these third-party libraries (TPLs) used in your apps? 
TPLs probably leak your personal privacy. 



Some special TPLs, such as advertising and analytic libraries usually use personal information to provide better service. 
%
However, some behaviors of those TPLs are undesirable or even harmful, including disclosing users' sensitive information such as location, personal profile without informing users~\cite{deepintent2019SIGSAC,harty2021logging, tangtse:21a, tang:ase19}. 
%
Considering the dominating mobile operating system~\cite{mobile_operating_system}, Android, the privacy leakage from TPLs is more serious.
%
The permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, xian2021taxonomyTSE, sun2014nativeguard}. 
%
Since the host apps share the same process space and the same permissions with TPLs, the mechanism leads to the over-privileged of TPLs. 
%
Recent research has demonstrated that the permissions abuse makes TPLs access users' personal information and cause potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} will also cause serious personal information leakage from host apps. 
A recent report~\cite{cybernews_dataleakage} also discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties, such as Firebase~\cite{firebase}.
%
PAMDroid~\cite{zhang2020does} discloses 120 of 555 apps shares users' personal identifiable information to analytic service TPLs without encryption. 
Even the unencrypted personal data are only shared with trusted TPLs that do not abuse the data, linking and mining of large amount of unencrypted personal information also could lead to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
% }



%%%%%%%%%%%%

\begin{comment}


\kaifa{
Android permission mechanism provides the same permissions to Android applications (apps) and the third-party libraries (TPL) used in the app~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android}.
%
The TPLs can abuse host apps’ permissions~\cite{qiu2021libcapsule, xu2022lie, li2021embedding} to access users' personal information (PI).
%
Recent research has demonstrated that the permissions abuse~\cite{xu2022lie, qiu2021libcapsule, di2021influencing, seneviratne2015measurement,cybernews_dataleakage} makes TPLs access users' personal information without user consent.
%
This will expose users' personal information to easy leakage situations.
%
Besides, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} will also cause serious personal information leakage from host apps.
%
A recent report~\cite{cybernews_dataleakage} also discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties, such as Firebase~\cite{firebase}.
%
PAMDroid~\cite{zhang2020does} discloses 120/555 apps shares users' personal identifiable information to analytic service TPLs without encryption.
%
Even the unencrypted personal data are only shared with trusted TPLs that will not abuse the data, linking and mining of large amount of unencrypted personal information leads to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
}
\end{comment}
%%%%%%

% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{comment}


\begin{table}[t]
\centering
\smaller
\vspace{2ex}
\caption{Personal information protection related regulations}
\scalebox{0.95}{%
\begin{tabular}{@{}p{0.4\textwidth}c@{}}
\toprule
\textbf{Regulations}                                                                             & \textbf{Enact Date} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
California Consumer Privacy Act (CCPA)                                                   & Jun-2018   \\
California Privacy Rights Act of 2020 (CPRA)                                             & Nov-2020   \\
\rowcolor[HTML]{EFEFEF} 
EU General Data Protection Regulation (GDPR)                                             & May-2018   \\
China Cybersecurity Practices Guidelines – Security Guidelines for Using Software Development Kit (SDK) for Mobile Internet Applications & Nov-2020 \\
\rowcolor[HTML]{EFEFEF} 
China Information security technology - Basic requirements for collecting personal information   in mobile internet applications         & Jan-2020 \\
China Information security technology - Personal information (PI) security specification & Oct-2020   \\
\rowcolor[HTML]{EFEFEF} 
New Zealand International Covenant on Civil and Political Rights (ICCPR) Privacy Act     & Jun-2020   \\ \bottomrule
\end{tabular}%
}
\label{tab:regulation}
\end{table}
\end{comment}

\begin{comment}
Personal data protection-related regulations have been promulgated worldwide to protect people's personal information from misuse since 2020 (Table~\ref{tab:regulation}). 
%
However, there still exist popular Android apps with over 142.5 million installations lead to user data leakages that violate regulation requirements~\cite{cybernews_dataleakage}.
%
%
Some of those user data leakages are caused by the mis-configuration of third-party libraries ({\tpl}s)~\cite{zhang2020does, harty2021logging}. This report~\cite{cpr_mis_tpl} disclosed that developers' mis-configuration of third-party services causes over 100 million personal information leakage.
%
\kaifa{For example, apps directly use users' personally identifiable information (e.g., email) as a user ID to submit to TP Ls without configuring any anonymization or encryption~\cite{zhang2020does}}.
%
%\xiancm{still need the misconfiguration's reference. Besides, what dd? you mean the misconfiguration, I think some readers may misunderstand or cannot know the misconfiguration}, %such as Firebase~\cite{firebase}.
% ~\cite{XXXX}\xiancm{still need add the firebase link}
% \xiancm{add the reference of firebase and cite the lili wei's paper about the firebase 'Logging Practices with Mobile Analytics: An Empirical Study on Firebase'}
%
%Besides, another report~\cite{cpr_mis_tpl} also disclosed that developers' mis-configuration of third-party services causes over 100 million personal information leakage.
%
% Although third-party libraries (TPLs) provide abundant functionalities to facilitate developers perfect their applications, the misconfigurations of TPLs will cause serious data leakage and conflicts with legal requirements.
%
% Zhang et al.~\cite{zhang2020does} exposed the misconfiguration of analytic TPLs lead to compromising privacy policies.
%\xiancm{what do you mean misconfiguration? since you have use many pages to introduce the misconf, I think you need to explain the misconfiguration at the begin. As far as I know, I know TPL especially ads can read the Personal information is not due to misconf. meanwhile, I think yutian tang's paper also give some reasons about the TPL can lead to privacy leakage.There are some reasons due to the Android permission mechanism. The TPLs and host apps share the same process, therefore ,they share the privilege that host apps have}



% 介绍 TPL
While third-party libraries ({\tpl}s) provide abundant functionalities to facilitate developers developing their applications, the vulnerabilities of {\tpl}s also threaten the security of users' personal information.
% and lead to violations of regulations.
% of apps' functionality with regulation requirements.
%
\kaifa{
For example, video apps, such as Youtube, integrate sharing functions to share the content with social apps, such as Whatsapp, that provide TPLs to facilitate sharing experience~\cite{xu2022lie}.
%
However, the sharing mechanism provides adversaries opportunities to steal the sharing content and thus lead to users' personal information leakage.
%
}
\end{comment}
%
% \cite{backes2016reliable}
%
% \revise{ATVHunter~\cite{atvhunter2021ICSE} investigate that 9,050/104,446 apps contain vulnerable TPLs with over 60 thousand vulnerabilities and security bugs.}
%\xiancm{rewrite this paragraph, this paper focuses on privacy leakage, you need to give the real example that the CVE can lead to the information leakage, the security bugs and CVE cannot say anything about info leakage.}
%
% \revise{Even so, nearly half of users~\cite{Balash2022security} are unaware of using {\tpl}s while enjoying the convince the {\tpl}s' functionalities provide.}
% \xiancm{ can delete without any logic. the forward sentences and backward sentences cannot say anything. I think you need read more papers, this introduction just show you cannot get deep understanding about current work and cannot present any key points that real related your work.} 
% {there are tons of papers about TPL's privacy leakage, I am curious why do you use them. It seems like you did not do a solid work at the beginning}
%
% \revise{Fortunately, regulations~\cite{piss, zhSDKLaw, gdpr, ccpa} enact Articles to enforce apps disclose data usage by {\tpl}s to protect users' personal information.}->



% \xian{

To normalize apps' behaviors and decrease the privacy leakage, various personal privacy  protection-related regulations (e.g., CCPA, CPRA, GDPR, ICCPR)~\cite{piss, zhSDKLaw, gdpr, ccpa} %(as shown in Table~\ref{tab:regulation}) 
have been promulgated to protect people's personal information from abuse, which requires developers to clearly know the functions and behaviors of TPLs and declare these sensitive behaviors in their privacy policy so as not to violate the regulations.
%
Besides, latest Google Play Developer Program policies (GPDP) ~\cite{google_play_pp_update} also ask developers to ensure the TPLs used in their apps are compliant with GPDP~\cite{gpdp}.
% \kaifa{todo: Maybe we can add the google's update of privacy polic requirements in April 6 2022, \url{https://support.google.com/googleplay/android-developer/answer/11899428}}
%
%
Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}. 
%
Thus, developers of {\tpl}s are required to provide privacy policies and disclose data usage in the privacy policies. To make {\tpl}s satisfy regulation requirements and help developers correctly use {\tpl}s, it is urgent to identify the consistency between {\tpl}s' data usage and privacy policies.
% }





%to limit apps disclosing over-privileged data to {\tpl}s for protecting users' personal information, which requires developers to clearly know the functions and behaviors of TPLs and declare them correctly in their privacy policy so as not to violate the foul requirements.
%Personal data protection-related regulations have been promulgated to protect people's personal information from abuse since 2018 (Table~\ref{tab:regulation}). 
%\xian{I think you should give up ASE, this paper cannot be accepted}

% 介绍现有的 app pp 分析
Recent research~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding} has proposed methods to identify the legality of apps, 
i.e., the apps are required to clearly disclose apps' personal information usage in their privacy policies.
% \xiancm{still miss a lot of papers, such as YL's paper, why do you miss these papers, there are also related to PP analysis}
%
% \revise{PoliCheck~\cite{ppcheck} checks the consistency of apps' data collection and \revise{sharing behavior with the apps' PP.}\xiancm{really, why? hard to read like grammar error} } -->\xian{
PoliCheck~\cite{ppcheck} checks the consistency between the apps' data collection and sharing behaviors with apps' privacy policy.
% }
%
% \revise{PAMDroid~\cite{zhang2020does} is designed to identify whether apps anonymize users' personally identifiable information (PII) when sharing the PII with TPLs.}
PAMDRroid identifies the TPLs' misconfiguration caused by personally identifiable information (PII) leakage.
%
Specifically, PAMDroid investigates whether the PII is preprocessed, such as anonymization and encryption, before shared with analytic service libraries.
%
%
PPChecker~\cite{ppchecker} discovers the trustwothiness of apps' privacy policies.
%
Specifically, PPChecker identifies a) whether apps' privacy policies cover all apps' personal information (PI) usage behaviors (\textbf{completeness}), b) whether apps' privacy policies correctly claims the personal information(PI) that the app uses or does not use (\textbf{correctness}), c) whether privacy policies' description uses vague words (\textbf{preciseness}), d) whether apps' privacy policies consistent other sources, such as TPL and Google Play, (\textbf{consistency}), and e) whether the privacy policies are easy-to-read.
%\revise{seay reading (\textbf{PP})}
%
However, PPChecker only concentrates on apps' privacy policies and is out-of-dated to satisfy latest regulation requirements.
%
% \revise{Specifically, PPChecker identifies whether app's PP covers all of the apps' data usage clearly and comprehensively and whether the apps' PP covers data usage in PP of TPLs used in the app.}\xiancm{hard to read, I did not understand the last sentence}
% However, existing works ignore the regulation requirements for TPLs.


\begin{comment}

\xiancm{delete this part}
\revise{Recent research~\cite{ppcheck, zhang2020does, nguyen2021share, andow2019policylint} has proposed methods to verify the consistency between apps' functionalities, privacy policies, and regulation requirements to make the apps in the markets satisfy the regulatory requirements, and help developers normalize apps implementation.}
\xian{are these papers verified these relations, I think maybe some paper just verified the relation between pp and functionalities. 
These paragraph can delete since they are repeated with the following paragraph}
\xiancm{write these papers separately}
%
\xian{Current research also has paid attention to the privacy policy analysis. Andow et al.~\cite{andow2019policylint} identified the conflicts XXXXX
}
\xiancm{rewrite}
Those methods either identify the conflicts within apps' privacy policies~\cite{andow2019policylint} or identify the inconsistency between apps' functionalities and their privacy policies, and further identify~\cite{zhang2020does, ppcheck} whether the app violates regulation requirements.
%
PPCheck~\cite{ppcheck} also reports that over 54\% apps disclose their usage of {\tpl}s in vague tones and Nguyen et al.~\cite{nguyen2021share} use dynamic analysis to identify whether the apps' data sharing behavior achieved users' explicit consent that is required by regulations~\cite{gdpr}.
\xiancm{rewrite}
%
These works widely\xiancm{what do you mean widely} analyze whether the apps' privacy policies on the market meet the regulation requirements, and help developers to write legal privacy policy documents more accurately. 
%
\revise{Those\xiancm{those indicate who, these indicate who} studies use dynamic analysis to extract apps' data usage behavior and natural language processing methods to extract data usage statements in privacy policies.}
%
Then flow-to-policy~\cite{ppcheck} consistency model is deployed to identify the consistency between apps' behavior, privacy policies and regulatory requirements.
\end{comment}

%

% To satisfy the regulation requirements and make developers' apps 

% PPChecker~\cite{ppcheck} 


% 说一下不足，以及我们可以提供的

%
%Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}.
%
%Thus, {\tpl}s are required to provide privacy policies and disclose data usage in the privacy policies.
%
%To make {\tpl}s satisfy regulation requirements and help developers correctly use {\tpl}s, it is urgent to identify the consistency between {\tpl}s' data usage and privacy policies.



\begin{comment}
% Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa} to specify their privacy policy statements to disclose their data usage or directly require~\cite{zhSDKLaw} {\tpl}s to clarify how they use users personal data.
%
% According to regulation requirements~\cite{zhSDKLaw, gdpr, ccpa}, {\tpl}s should provide privacy policy to clearly disclose their data usage.
%
% Thus, {\tpl}s' functionality should be analyzed to identify the whether their privacy policies disclose all of their data usage
% consistency of their behavior with privacy policy statements.
%




% \kaifa{Rewritten as latest paragraph}
% \revise{Although existing methods provide promising performance, they ignore the regulation requirements for {\tpl}s, and their basic methodology, i.e., dynamic analysis, limits their analysis.}
% %
% Regulations either consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa} to specify their privacy policy statements to disclose their data usage or directly require~\cite{zhSDKLaw} {\tpl}s to clarify how they use users personal data.
% %
% However, existing works neither ignores analyzing {\tpl}s functionalities~\cite{zhang2020does, andow2019policylint} nor only consider specific types of {\tpl}, such as advertising services and analytic service~\cite{ppcheck,nguyen2021share}.
% %
% According to regulation requirements~\cite{zhSDKLaw, gdpr, ccpa}, {\tpl}s should provide privacy policy to clearly disclose their data usage.
% %
% Thus, {\tpl}s' functionality should be analyzed to identify the consistency of their behavior with privacy policy statements.
% %
% Because {\tpl}s are a set of methods or functions, {\tpl}s are generally not executable alone.
% %
% \revise{Therefore, dynamic analysis is limited to analyzing {\tpl}s' functionality.}
% \xiancm{I cannot understand why you say the limitation of dynamic analysis as current research gap used in previous research. I think that is totally incorrect. without any proofs and many new dynamic methods can solve these issues well.}
%
\end{comment}



Although existing methods provide promising performance for identifying the consistency between the app's behavior and privacy policies~\cite{yu2016revisiting,ppcheck,ppchecker}, they ignore analyzing the regulation requirements for {\tpl}s.
%
% \xiancm{recheck this sentence, Did current research consider the pp analysis of TPLs? Did current research considers the laws analysis of TPLs? }
% To regulate the usage of TPLs and help developers better understand the functionality of TPLs they use, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically check the \textit{legality} of {\tpl}s and \textit{correctness} of usage of {\tpl}s.
%
To regulate the usage of TPLs and help developers better understand the functionality of TPLs they use, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically identify the consistency between regulation requirements and TPLs, and whether the host app's usage of TPLs satisfies regulations.
% the consistency between regulation requirements and app's usage of TPL.
%
First, we analyze regulations that are related to privacy and security law~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr}, or normalizing software applications~\cite{zhSDKLaw} (\S\ref{sec:bb_regulation_req}).
%
We concentrate on TPL-related Articles.% that are related to third parties.
%
After summarizing the regulation requirements, {\oursystem} first identifies the consistency between TPL and regulation requirements by analyzing TPL's binary code (\S\ref{sec:tpl_data}) and TPL's privacy policies (\S\ref{sec:tpl_pp}).
%
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
%
Finally, {\oursystem}  checks the consistency between host app's privacy policies and TPL-related regulation requirements.
%
By analyzing the host app's privacy policies and binary code, {\oursystem} identifies whether the host app's privacy policy clearly claims the usage of TPLs, including what kinds of data are shared with TPLs rather than only identifying the existence of used TPLs' privacy links~\cite{ppchecker}.
%
% {\oursystem} implements the following functionalities to achieve such goal and tackles the limitations of existing works accordingly.
%



We address the following challenges in the development of {\oursystem}.
%
First, no dataset is available for research in this area.
%
To counter this issue, we gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{c}) 642 distinct host apps labeled with an integrated TPL list and \textbf{d}) %642 
corresponding host apps' privacy policies.
%
Second, it is non-trivial to track the data usage of TPLs because 1) TPLs are usually provided as compiled code without source code, and 2) it is difficult to construct TPLs' call graph that contains all important edges (invocation relations)~\cite{reif2016call}.
%
To tackle the challenge, {\oursystem} is built on {\soot}~\cite{soot} that is a popular static analysis tool and does not require the source code.
%
To construct a comprehensive callgraph of the TPL to facilitate personal information track, {\oursystem} implements new methods (\S\ref{sec:tpl_data})  to optimize TPLs’ FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Third, privacy policy analysis remains challenging as a natural language processing task, because privacy policies use different patterns (\S\ref{sec:host_app_pp}) to describe the usage,and the usage of TPLs.% and data sharing with TPLs.
%
To counter the challenge, {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
{\oursystem} implements abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).




\begin{comment}



% \xiancm{based on your description the legality analysis is clearly say PI usage in PP in previous paragraph and this paragraph is to say ignore the regulation requirements analysis for TPLs, here, you did not say anything about that. need to detailed description about the functions involving the pp analysis and laws consistency analysis}
% \xiancm{Why \oursystem need to explain here}
%
% For legality identification, {\oursystem} checks whether the {\tpl} contains a privacy policy and uses static analysis to analyze its functionalities to identify the consistency with PP.
% %
% For correctness usage of {\tpl}s, {\oursystem} identifies 1) what {\tpl}s are used by host apps, 2) what kinds data are interacted with {\tpl}s, and 3) whether hosp apps' privacy policy clearly state {\tpl}s' data usage.
%
% \xiancm{I remember your paper need to consider the laws analysis, I cannot find any description about laws analysis in this introduction}
%However, there still exist challenges to be countered when designing {\oursystem}.
% \xian{To achieve such goals, we need to solve the following challenges:}
%



We address the following challenges in the development of {\oursystem}.
%
First, there is no available dataset for research in this area.
%
% To counter this issue and facilitate the research in this area, we 
% gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) 498 TPLs' privacy policies with labeled tokens in two languages (349 in English and 113 in Chinese), \textbf{d}) 855 distinct host apps labeled with an integrated TPL list and \textbf{f}) 1056 host apps' privacy policies (800 in English and 256 in Chinese).
To counter this issue, we gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{d}) 642 distinct host apps labeled with an integrated TPL list and \textbf{f}) %642 
corresponding host apps' privacy policies.
%
% We will release the dataset after the paper gets published.
%
Second, it is non-trivial to track the data usage of TPLs because 1) TPLs are usually provided as compiled code without source code and 2) it is difficult to construct a call graph that contains all important edges (invocation relations)~\cite{reif2016call}.
%
To tackle the challenge, {\oursystem} is built on {\soot}~\cite{soot} that is a popular static analysis tool and does not require the source code.
%
To construct a comprehensive callgraph of the TPL to facilitate personal information track, {\oursystem} implements new methods (\S\ref{sec:tpl_data})  to optimize TPLs’ FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Third, privacy policy analysis remains challenging as a natural language processing task, because privacy policies use different patterns (\S\ref{sec:host_app_pp}) to describe the usage,and the usage of TPLs.% and data sharing with TPLs.
%
To counter the challenge, {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
{\oursystem} designs abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).
%





% \noindent\textbf{Availability of dataset.}


\noindent\textbf{Data leakage analysis in third-party  libraries.}
%
\xiancm{Based on your description, I cannot see any challenges here, challenges should be the point that difficult to solve, where is it}
As TPLs are usually provided as compiled code~\cite{qiu2021libcapsule} without source code, {\oursystem} uses {\soot}~\cite{soot} to analyze TPLs that does not require source code.
%
{\oursystem} applies static analysis to identify the data leakage in third-party libraries.
%
{\oursystem} analyzes the data flow of TPLs to identify the definition and usage chain~\cite{pande1994interprocedural} (\S\ref{sec:tpl_data}) of personal information (PI).
%
As {\oursystem} uses function call graphs (FCG) to better trace the usage of target variables, we propose new methods (\S\ref{sec:tpl_data}) to optimize TPLs' FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Excepting PI name matching with predefined data types, we also construct a mapping knowledge set that builds connections with PI name and Android APIs to improve the variable locating precision.
% 



% \noindent\textbf{Identification of host apps' PI interaction with TPLs.}
%
% \cite{wei2018amandroid}


\end{comment}



\begin{comment}

\noindent\textbf{TPL usage identification in host apps.}
%
Taint analysis is widely used to identify data leakage in software with predefined sources and sinks.
%
However, it is still a challenge to locate the destination of those data leakages while it is necessary to locate them to further identify the correctness of host apps' usage of TPLs. 
%
{\oursystem} first builds a knowledge set to match {\tpl} related invocations in binary code.% (\kaifa{revise it}).
%
Combining the data flow of personal information and {\tpl}s, {\oursystem} determines the destination of PI data (\S\ref{sec:host_app_data})

%
% \xiancm{I am dying if I just read more lines..... I do not know what are you doing...... many things are totally incorrect}
% \xiancm{The figure cannot show any useful information and ugly }
% % 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/tpl_enumeration_in_host_app_pp_new.png}
%     \caption{TPL usage in privacy policy of \textit{jp.ne.ibis.ibis-paintx.app}}
%     \label{fig:pp_tpl_list}
% \end{figure}


\noindent\textbf{TPL related statements extraction in host apps' privacy policies.}
%
\revise{Existing data-related statements extraction methods~\cite{ppcheck, andow2019policylint} are generally constructed on named entity recognition techniques that require a large amount of labeled corpus for model training.
%
Besides, existing methods are usually based on predefined sharing and collecting verbs to locate those data-related sentences. \xiancm{you just say the existing method, where is the challenges of your work}
%
Although those methods achieves desirable performance for analyzing apps' data collection statements in privacy policy, those methods may omit information related to {\tpl}s because host apps may provide {\tpl}s' information in form of table or enumeration.} \xiancm{this is limitation of existing work is not your work's challenges. logic chaos}
%(as is illustrated in 
% Fig.~\ref{fig:pp_table} and 
% Fig.~\ref{fig:pp_tpl_list} separately).  
%
Besides extending the existing sharing and collection words list to locate data usage-related statements in the privacy policy, {\oursystem} also designs \revise{heuristic patterns}\xiancm{when anytime you use heuristic you need to explain the heuristic patterns first} to precisely extract {\tpl} related statements for further flow-to-policy analysis.
\xiancm{I still cannot see any challenges here}



\end{comment}
% write a paragraph to summarize the performance of our tool

Overall, our contributions are summarized as follows:


\begin{itemize}[leftmargin=*]


\item We propose a novel system named {\oursystem} to analyze Android TPL-related regulation complaints.
%
{\oursystem} conducts static analysis to analyze TPLs personal information accessing both individually and inside host apps, and applies NLP techniques to analyze TPLs' and host apps' privacy policies.
%
Then, {\oursystem} identifies the whether the data access behaviors are clearly claimed in the privacy policies.
% {\oursystem} uses static analysis to extract data flow in TPLs and host apps based on soot, and uses natural language process methods to extract personal information statements in privacy policies.
% {\oursystem} builds on {\soot} for static analysis of TPLs and host apps, and uses natural language processing to analyze privacy policies.
%
% \vspace{1em}

\item We construct a privacy data set that includes 187 TPLs and corresponding privacy policies, 642 host apps and corresponding privacy policies.
%
% Specifically, 
Our TPL's privacy policies contain labeled corpus related to TPLs data collection and sharing behavior, host apps are labeled with integrated TPLs, and the host app's privacy policies are labeled with used TPLs and data interaction with TPLs.
%
Our dataset will be released after the paper get published.

% \vspace{1em}

\item {\oursystem} discovers 24\% of TPLs miss providing privacy policies, 37\% of TPL's privacy policies conceal their data usage.
%
{\oursystem} also finds over 65\% of host apps violate the regulation requirements for disclosing data interactions with TPLs.
%

% \item We propose a novel system \oursystem to identify the compliance of\xiancm{what do you mean here? compliance of TPLs, hard to understand. compliance should be laws and regulations instead of TPLs???? logic issue} third-party libraries and apps' interaction with third-party libraries.
% % Android Third party libraries misuse and Privacy policy conflict checker


% \item We develop {\oursystem}, a new tool to automatically analyze TPLs' and apps' data flow and privacy policies.
% %
% \xiancm{rewrite the above two items, it seems like they can combine together}


% \xiancm{one item can say the released dataset but you need to give the link, besides, SE usually need to release the code, the other item can say your performance is good, ok.}
% \item We build a data set including a) labeled privacy policies in two languages, b)TPLs with data leakage behavior, and c) host apps with labels concerning used TPLs and data interaction with TPLs.
% %
% We evaluate the performance of {\oursystem} on created dataset and disclose the harm of TPL data leakage in a large scale.
% %



\end{itemize}









\begin{comment}
%
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.






This is introduction
\subsection{Our target}


\begin{itemize}
    \item We have to identify whether the action of {\tpl} is consistent with {\tpl}'s privacy policy.
     
    \item We need to detect all data usage (at least sensitive data usage) in APP. And specify which groups are used by app and which groups are used by {\tpl}.
    
    \item
\end{itemize}


Tool name: {\oursystem} Android Third party libraries misuse and Privacy policy conflict checker.

\subsection{Challenges}

\textbf{1. {\tpl} information extraction}: Information about the usage of {\tpl}, the data related to {\tpl} are usually formatted as a table or organized as form of explanations (for example, facebook: data1, data2 \kaifa{put a case study in Appendix}).
%
% We apply \texttt{Tablemaster} to extract information from tables and \kaifa{a new NLP technique} to merge information in form of explanations.
\kaifa{not suitable. I analyze 3502 privacy policy. Only 471/3502 privacy policy contains html tag \textit{table}. I manually checked 200/471. Only 6/200 contains table are related to data usage that cannot be analyzed by the method in PolicyLint.}

PolicyLint~\cite{andow2019policylint} deals with the table data by merging the formatted lists into sentences.
%
This preprocessing method fails when only noun phrase on the table because the method in PolicyLint directly merges the items together without considering the characteristics of table, i.e., the data in each item shares same attributes. \kaifa{give an example in appendix}
%


\textbf{2. Data analysis in third party libraries. }
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
For dynamic analysis,  we must find a apk that uses the {\tpl} and leverage the data usage of {\tpl}.
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.
%
\kaifa{details, how to design such a tool}


\textbf{3. Consistency analysis} We focus on two aspect of consistency analysis: a) whether the app's privacy policy covers all {\tpl} usage. 
%
To relax condition, the app's privacy policy should contain all {\tpl}s that collect or share data.
%
b) If the app's privacy policy covers the {\tpl} usage, does the data usage in privacy policy consistent with the {\tpl}'s real data usage.

\end{comment}

==> tmp/intro_old_220829.tex <==
\section{Introduction}

% \input{table/regulation_summary}


% \vspace{0.5em}
\begin{quote}
    \emph{\textbf{``Hedges have eyes and walls have ears.''}}
    \begin{flushright}
    - Trusler, John, 1735-1820.
    \end{flushright}
\end{quote}
% \vspace{1em}




Nowadays, the smartphone is ubiquitous, and mobile apps, as a significant part of mobile ecology, are playing essential roles in our daily life, from living, working, and education to  business~\cite{deepintent2019SIGSAC}. 
Besides, more and more developers tend to use many off-the-shelf toolkits or third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE,libdetect2020ASE}.
% Have you ever thought about the security of these third-party libraries (TPLs) used in your apps? 
% TPLs probably leak your personal privacy. 
%
However, developers may omits the privacy threat in amount of TPLs.
%
For example, Anthony et.al.~\cite{short2014android} identify Android advertisement libraries leak amount of user data, such as IMEI.
 

Some special TPLs (e.g., advertising and analytic libraries) use personal information to provide better service. 
%
However, TPLs may collect user data that is not necessary for providing related services, and those data collection behavior may lead to privacy leakage or even security concerns~\cite{deepintent2019SIGSAC, harty2021logging, tangtse:21a}.
%
% However, behaviors of those TPLs are undesirable or even harmful, including disclosing users' sensitive information such as location and personal profiles without informing users~\cite{deepintent2019SIGSAC,harty2021logging, tangtse:21a, tang:ase19}. 
%
Considering the dominating mobile operation system~\cite{mobile_operating_system}, Android, 
% 
% Android, the privacy leakage from TPLs is more serious.
%
the permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}. 
%
Since the host apps share the same process space and the same permissions with TPLs, the mechanism leads to the over-privileged of TPLs. 
%
Recent research has demonstrated that permissions abuse makes TPLs access users' personal information and causes potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} will also cause serious personal information leakage from host apps. 
%
For example, a recent report~\cite{cybernews_dataleakage} discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties, such as Firebase~\cite{firebase}.
%
Zhang et.al.~\cite{zhang2020does} disclose 120 of 555 apps that share users' personal identifiable information to analytic service TPLs without encryption. 
%
Besides, research~\cite{kiranmayi2018reducing, chen2014information} also demonstrates that linking and mining large amount of unencrypted personal information will lead to serious personal privacy leakage.
%
Thus, it is urgent to identify TPLs' data sharing and collection actions to protect user privacy.
%
% Even the unencrypted personal data are only shared with trusted TPLs that do not abuse the data, linking and mining of a large amount of unencrypted personal information also could lead to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
% }



%%%%%%%%%%%%

\begin{comment}


\kaifa{
Android permission mechanism provides the same permissions to Android applications (apps) and the third-party libraries (TPL) used in the app~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android}.
%
The TPLs can abuse host apps’ permissions~\cite{qiu2021libcapsule, xu2022lie, li2021embedding} to access users' personal information (PI).
%
Recent research has demonstrated that the permissions abuse~\cite{xu2022lie, qiu2021libcapsule, di2021influencing, seneviratne2015measurement,cybernews_dataleakage} makes TPLs access users' personal information without user consent.
%
This will expose users' personal information to easy leakage situations.
%
Besides, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} will also cause serious personal information leakage from host apps.
%
A recent report~\cite{cybernews_dataleakage} also discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties, such as Firebase~\cite{firebase}.
%
PAMDroid~\cite{zhang2020does} discloses 120/555 apps shares users' personal identifiable information to analytic service TPLs without encryption.
%
Even the unencrypted personal data are only shared with trusted TPLs that will not abuse the data, linking and mining of large amount of unencrypted personal information leads to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
}
\end{comment}
%%%%%%

% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{comment}


\begin{table}[t]
\centering
\smaller
\vspace{2ex}
\caption{Personal information protection related regulations}
\scalebox{0.95}{%
\begin{tabular}{@{}p{0.4\textwidth}c@{}}
\toprule
\textbf{Regulations}                                                                             & \textbf{Enact Date} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
California Consumer Privacy Act (CCPA)                                                   & Jun-2018   \\
California Privacy Rights Act of 2020 (CPRA)                                             & Nov-2020   \\
\rowcolor[HTML]{EFEFEF} 
EU General Data Protection Regulation (GDPR)                                             & May-2018   \\
China Cybersecurity Practices Guidelines – Security Guidelines for Using Software Development Kit (SDK) for Mobile Internet Applications & Nov-2020 \\
\rowcolor[HTML]{EFEFEF} 
China Information security technology - Basic requirements for collecting personal information   in mobile internet applications         & Jan-2020 \\
China Information security technology - Personal information (PI) security specification & Oct-2020   \\
\rowcolor[HTML]{EFEFEF} 
New Zealand International Covenant on Civil and Political Rights (ICCPR) Privacy Act     & Jun-2020   \\ \bottomrule
\end{tabular}%
}
\label{tab:regulation}
\end{table}
\end{comment}

\begin{comment}
Personal data protection-related regulations have been promulgated worldwide to protect people's personal information from misuse since 2020 (Table~\ref{tab:regulation}). 
%
However, there still exist popular Android apps with over 142.5 million installations lead to user data leakages that violate regulation requirements~\cite{cybernews_dataleakage}.
%
%
Some of those user data leakages are caused by the mis-configuration of third-party libraries ({\tpl}s)~\cite{zhang2020does, harty2021logging}. This report~\cite{cpr_mis_tpl} disclosed that developers' mis-configuration of third-party services causes over 100 million personal information leakage.
%
\kaifa{For example, apps directly use users' personally identifiable information (e.g., email) as a user ID to submit to TP Ls without configuring any anonymization or encryption~\cite{zhang2020does}}.
%
%\xiancm{still need the misconfiguration's reference. Besides, what dd? you mean the misconfiguration, I think some readers may misunderstand or cannot know the misconfiguration}, %such as Firebase~\cite{firebase}.
% ~\cite{XXXX}\xiancm{still need add the firebase link}
% \xiancm{add the reference of firebase and cite the lili wei's paper about the firebase 'Logging Practices with Mobile Analytics: An Empirical Study on Firebase'}
%
%Besides, another report~\cite{cpr_mis_tpl} also disclosed that developers' mis-configuration of third-party services causes over 100 million personal information leakage.
%
% Although third-party libraries (TPLs) provide abundant functionalities to facilitate developers perfect their applications, the misconfigurations of TPLs will cause serious data leakage and conflicts with legal requirements.
%
% Zhang et al.~\cite{zhang2020does} exposed the misconfiguration of analytic TPLs lead to compromising privacy policies.
%\xiancm{what do you mean misconfiguration? since you have use many pages to introduce the misconf, I think you need to explain the misconfiguration at the begin. As far as I know, I know TPL especially ads can read the Personal information is not due to misconf. meanwhile, I think yutian tang's paper also give some reasons about the TPL can lead to privacy leakage.There are some reasons due to the Android permission mechanism. The TPLs and host apps share the same process, therefore ,they share the privilege that host apps have}



% 介绍 TPL
While third-party libraries ({\tpl}s) provide abundant functionalities to facilitate developers developing their applications, the vulnerabilities of {\tpl}s also threaten the security of users' personal information.
% and lead to violations of regulations.
% of apps' functionality with regulation requirements.
%
\kaifa{
For example, video apps, such as Youtube, integrate sharing functions to share the content with social apps, such as Whatsapp, that provide TPLs to facilitate sharing experience~\cite{xu2022lie}.
%
However, the sharing mechanism provides adversaries opportunities to steal the sharing content and thus lead to users' personal information leakage.
%
}
\end{comment}



To normalize apps' behaviors and prevent privacy leakage, various personal privacy  protection-related regulations (e.g., CCPA, CPRA, GDPR, ICCPR)~\cite{piss, zhSDKLaw, gdpr, ccpa} have been promulgated to protect people's personal information from abuse, which requires developers to clearly understand TPL behaviors and declare these sensitive behaviors in their privacy policy so as not to violate the regulations.
%
Besides, the latest Google Play Developer Program policies (GPDP) ~\cite{google_play_pp_update} also ask developers to ensure the TPLs used in their apps are compliant with GPDP~\cite{gpdp}.
% 
% Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}. 
%
Developers of {\tpl}s are required to provide privacy policies and disclose data usage in the privacy policies. 
%
To make {\tpl}s comply with regulation requirements and help developers correctly use {\tpl}s, it is urgent to identify the consistency between {\tpl}s' data usage and privacy policies.






%\xian{I think you should give up ASE, this paper cannot be accepted}

% 介绍现有的 app pp 分析
Recent research~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding} propose methods to identify the legality of apps, 
i.e., the apps are required to disclose personal information usage in their privacy policies.
%
PoliCheck~\cite{ppcheck} checks the consistency between the apps' data collection and sharing behaviors with the privacy policy.
%
PAMDRroid identifies the TPLs' misconfiguration caused by personally identifiable information (PII) leakage.
%
Specifically, PAMDroid investigates whether the PII is preprocessed, such as anonymization and encryption, before sharing with analytic service libraries.
%
PPChecker~\cite{ppchecker} discovers the trustworthiness of apps' privacy policies.
%
Specifically, PPChecker identifies a) whether apps' privacy policies cover all apps' personal information (PI) usage behaviors (\textbf{completeness}), b) whether apps' privacy policies correctly claim the personal information(PI) that the app uses or does not use (\textbf{correctness}), c) whether privacy policies' description uses vague words (\textbf{preciseness}), d) whether apps' privacy policies consistent other sources, such as TPL and Google Play, (\textbf{consistency}), and e) whether the privacy policies are easy-to-read.
%
However, PPChecker only concentrates on apps' privacy policies and is out-of-dated to satisfy the latest regulation requirements.
%



\begin{comment}

\revise{Recent research~\cite{ppcheck, zhang2020does, nguyen2021share, andow2019policylint} has proposed methods to verify the consistency between apps' functionalities, privacy policies, and regulation requirements to make the apps in the markets satisfy the regulatory requirements, and help developers normalize apps implementation.}
\xian{are these papers verified these relations, I think maybe some paper just verified the relation between pp and functionalities. 
These paragraph can delete since they are repeated with the following paragraph}
\xiancm{write these papers separately}
%
\xian{Current research also has paid attention to the privacy policy analysis. Andow et al.~\cite{andow2019policylint} identified the conflicts XXXXX
}
\xiancm{rewrite}
Those methods either identify the conflicts within apps' privacy policies~\cite{andow2019policylint} or identify the inconsistency between apps' functionalities and their privacy policies, and further identify~\cite{zhang2020does, ppcheck} whether the app violates regulation requirements.
%
PPCheck~\cite{ppcheck} also reports that over 54\% apps disclose their usage of {\tpl}s in vague tones and Nguyen et al.~\cite{nguyen2021share} use dynamic analysis to identify whether the apps' data sharing behavior achieved users' explicit consent that is required by regulations~\cite{gdpr}.
\xiancm{rewrite}
%
These works widely\xiancm{what do you mean widely} analyze whether the apps' privacy policies on the market meet the regulation requirements, and help developers to write legal privacy policy documents more accurately. 
%
\revise{Those\xiancm{those indicate who, these indicate who} studies use dynamic analysis to extract apps' data usage behavior and natural language processing methods to extract data usage statements in privacy policies.}
%
Then flow-to-policy~\cite{ppcheck} consistency model is deployed to identify the consistency between apps' behavior, privacy policies and regulatory requirements.
\end{comment}

%

% To satisfy the regulation requirements and make developers' apps 

% PPChecker~\cite{ppcheck} 


% 说一下不足，以及我们可以提供的

%
%Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}.
%
%Thus, {\tpl}s are required to provide privacy policies and disclose data usage in the privacy policies.
%
%To make {\tpl}s satisfy regulation requirements and help developers correctly use {\tpl}s, it is urgent to identify the consistency between {\tpl}s' data usage and privacy policies.





% Although existing methods identify the consistency between the app's behavior and privacy policies~\cite{yu2016revisiting,ppcheck,ppchecker}, they ignore analyzing the regulation requirements for {\tpl}s. 
%
% To regulate the usage of TPLs and help developers better understand the functionality of TPLs they use, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically check the \textit{legality} of {\tpl}s and \textit{correctness} of usage of {\tpl}s.


Existing methods are limited to identifying the consistency between apps' behavior and privacy policies~\cite{yu2016revisiting,ppcheck,ppchecker} and ignore the regulation requirements for {\tpl}s.
%
To regulate the usage of TPLs and help developers better understand the functionality of TPLs they use, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically identify the consistency between regulation requirements and TPLs, and determine whether the host app's usage of TPLs satisfies regulations or not.
%
First, we analyze regulations of privacy and security related law~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr}, and the regulations that normalizing software applications~\cite{zhSDKLaw} (\S\ref{sec:bb_regulation_req}). 
% 
We concentrate on TPL-related Articles.
%
As privacy policy analysis requires expert knowledge of both legal and software engineering, one expert and  one senior researcher, who has conducted research on software engineering and privacy policy analysis for over seven years and two years, respectively, read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPL usages. 
%
{\oursystem} first identifies the consistency between TPL and regulation requirements by analyzing TPL's binary code (\S\ref{sec:tpl_data}) and TPL's privacy policies (\S\ref{sec:tpl_pp}).
%
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
%
{\oursystem} checks the consistency between host app's privacy policies and TPL-related regulation requirements.
%
By analyzing the host app's privacy policies and binary code, {\oursystem} identifies whether the host app's privacy policy clearly claims  the usage of TPLs, including what kinds of data are shared with TPLs rather than only identifying the existence of used TPLs' privacy links~\cite{ppchecker}. 
%
% {\oursystem} implements the following functionalities to achieve such goal and tackles the limitations of existing works accordingly.
%



We address the following challenges in developing {\oursystem}.
%
First, no normalized data are publicly available for analyzing TPL compliance. 
% no dataset is available for research in this area.
%
To counter this issue, we create a novel data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{c}) 642 distinct host apps labeled with an integrated TPL list and \textbf{d}) 
corresponding host apps' privacy policies.
%
Second, it is non-trivial to get the data usage of TPLs because TPLs are usually provided as compiled code without source code, and it is challenging to trace data usage in close source TPLs. %
To overcome this challenge, {\oursystem} conducts static analysis for TPL data usage analysis.
We do not conduct dynamic analysis since it cannot execute all possible paths in apps~\cite{schindler2022privacy}.
%and it also requires executing the target software and analyzing the data changes during runtime.
%
Moreover, TPL only provides APIs and it relies on the host app to trigger these APIs. 
Thus, dynamic analysis cannot execute the TPL directly.
%
To perform static analysis, {\oursystem} uses {\soot}~\cite{soot}, a popular static analysis tool, 
%and does not require the source code. 
%Then, {\oursystem}  optimizes
to construct the TPL's function call graph and conduct data flow analysis(\S\ref{sec:tpl_data}). %, specifically variable use-define analysis. 
%
Third, analyzing privacy policy is challenging because developers can use different sentences (\S\ref{sec:host_app_pp}) to describe personal information usage and TPL usage.
%
To analyze data and TPL usage related statements of privacy policies, {\oursystem} implements an expert system to extract abstract data usage patterns.
% {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
% {\oursystem} implements abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).




\begin{comment}



% \xiancm{based on your description the legality analysis is clearly say PI usage in PP in previous paragraph and this paragraph is to say ignore the regulation requirements analysis for TPLs, here, you did not say anything about that. need to detailed description about the functions involving the pp analysis and laws consistency analysis}
% \xiancm{Why \oursystem need to explain here}
%
% For legality identification, {\oursystem} checks whether the {\tpl} contains a privacy policy and uses static analysis to analyze its functionalities to identify the consistency with PP.
% %
% For correctness usage of {\tpl}s, {\oursystem} identifies 1) what {\tpl}s are used by host apps, 2) what kinds data are interacted with {\tpl}s, and 3) whether hosp apps' privacy policy clearly state {\tpl}s' data usage.
%
% \xiancm{I remember your paper need to consider the laws analysis, I cannot find any description about laws analysis in this introduction}
%However, there still exist challenges to be countered when designing {\oursystem}.
% \xian{To achieve such goals, we need to solve the following challenges:}
%



We address the following challenges in the development of {\oursystem}.
%
First, there is no available dataset for research in this area.
%
To counter this issue, we gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{d}) 642 distinct host apps labeled with an integrated TPL list and \textbf{f}) %642 
corresponding host apps' privacy policies.
%
% We will release the dataset after the paper gets published.
%
Second, it is non-trivial to track the data usage of TPLs because 1) TPLs are usually provided as compiled code without source code and 2) it is difficult to construct a call graph that contains all important edges (invocation relations)~\cite{reif2016call}.
%
To tackle the challenge, {\oursystem} is built on {\soot}~\cite{soot} that is a popular static analysis tool and does not require the source code.
%
To construct a comprehensive callgraph of the TPL to facilitate personal information track, {\oursystem} implements new methods (\S\ref{sec:tpl_data})  to optimize TPLs’ FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Third, privacy policy analysis remains challenging as a natural language processing task, because privacy policies use different patterns (\S\ref{sec:host_app_pp}) to describe the usage,and the usage of TPLs.% and data sharing with TPLs.
%
To counter the challenge, {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
{\oursystem} designs abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).
%





% \noindent\textbf{Availability of dataset.}


\noindent\textbf{Data leakage analysis in third-party  libraries.}
%
\xiancm{Based on your description, I cannot see any challenges here, challenges should be the point that difficult to solve, where is it}
As TPLs are usually provided as compiled code~\cite{qiu2021libcapsule} without source code, {\oursystem} uses {\soot}~\cite{soot} to analyze TPLs that does not require source code.
%
{\oursystem} applies static analysis to identify the data leakage in third-party libraries.
%
{\oursystem} analyzes the data flow of TPLs to identify the definition and usage chain~\cite{pande1994interprocedural} (\S\ref{sec:tpl_data}) of personal information (PI).
%
As {\oursystem} uses function call graphs (FCG) to better trace the usage of target variables, we propose new methods (\S\ref{sec:tpl_data}) to optimize TPLs' FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Excepting PI name matching with predefined data types, we also construct a mapping knowledge set that builds connections with PI name and Android APIs to improve the variable locating precision.
% 



% \noindent\textbf{Identification of host apps' PI interaction with TPLs.}
%
% \cite{wei2018amandroid}


\end{comment}



\begin{comment}

\noindent\textbf{TPL usage identification in host apps.}
%
Taint analysis is widely used to identify data leakage in software with predefined sources and sinks.
%
However, it is still a challenge to locate the destination of those data leakages while it is necessary to locate them to further identify the correctness of host apps' usage of TPLs. 
%
{\oursystem} first builds a knowledge set to match {\tpl} related invocations in binary code.% (\kaifa{revise it}).
%
Combining the data flow of personal information and {\tpl}s, {\oursystem} determines the destination of PI data (\S\ref{sec:host_app_data})

%
% \xiancm{I am dying if I just read more lines..... I do not know what are you doing...... many things are totally incorrect}
% \xiancm{The figure cannot show any useful information and ugly }
% % 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/tpl_enumeration_in_host_app_pp_new.png}
%     \caption{TPL usage in privacy policy of \textit{jp.ne.ibis.ibis-paintx.app}}
%     \label{fig:pp_tpl_list}
% \end{figure}


\noindent\textbf{TPL related statements extraction in host apps' privacy policies.}
%
\revise{Existing data-related statements extraction methods~\cite{ppcheck, andow2019policylint} are generally constructed on named entity recognition techniques that require a large amount of labeled corpus for model training.
%
Besides, existing methods are usually based on predefined sharing and collecting verbs to locate those data-related sentences. \xiancm{you just say the existing method, where is the challenges of your work}
%
Although those methods achieves desirable performance for analyzing apps' data collection statements in privacy policy, those methods may omit information related to {\tpl}s because host apps may provide {\tpl}s' information in form of table or enumeration.} \xiancm{this is limitation of existing work is not your work's challenges. logic chaos}
%(as is illustrated in 
% Fig.~\ref{fig:pp_table} and 
% Fig.~\ref{fig:pp_tpl_list} separately).  
%
Besides extending the existing sharing and collection words list to locate data usage-related statements in the privacy policy, {\oursystem} also designs \revise{heuristic patterns}\xiancm{when anytime you use heuristic you need to explain the heuristic patterns first} to precisely extract {\tpl} related statements for further flow-to-policy analysis.
\xiancm{I still cannot see any challenges here}



\end{comment}
% write a paragraph to summarize the performance of our tool

Overall, our contributions are summarized as follows:


\begin{itemize}[leftmargin=*]


\item We propose a novel system named {\oursystem} to analyze the compliance of Android TPLs. 
%
{\oursystem} analyzes TPLs' personal information accessing both individually and inside host apps, and applies NLP techniques to analyze TPLs' and host apps' privacy policies.
%
By combining the result of bytecode analysis and privacy policy analysis, {\oursystem} determines whether the TPLs and usage of TPLs in host apps comply with regulation requirements or not.
% {\oursystem} identifies whether data access behaviors are clearly claimed in  privacy policies.

% {\oursystem} uses static analysis to extract data flow in TPLs and host apps based on soot, and uses natural language process methods to extract personal information statements in privacy policies.
% {\oursystem} builds on {\soot} for static analysis of TPLs and host apps, and uses natural language processing to analyze privacy policies.
%
% \vspace{1em}

\item We construct a privacy data set that includes 187 TPLs and corresponding privacy policies, 642 host apps and corresponding privacy policies.
%
TPL's privacy policies in our data set contain labeled corpus related to TPLs' data accessing behavior and the host app's privacy policies are labeled with used TPLs and data interaction with TPLs.
%
Our data set will be released after the publication of this paper.

% \vspace{1em}

\item {\oursystem} discovers over 24\% of TPLs miss providing privacy policies, 37\% of TPL's privacy policies conceal their data usage.
%
{\oursystem} also finds over 65\% of host apps violate the regulation requirements for disclosing data interactions with TPLs.
%

% \item We propose a novel system \oursystem to identify the compliance of\xiancm{what do you mean here? compliance of TPLs, hard to understand. compliance should be laws and regulations instead of TPLs???? logic issue} third-party libraries and apps' interaction with third-party libraries.
% % Android Third party libraries misuse and Privacy policy conflict checker


% \item We develop {\oursystem}, a new tool to automatically analyze TPLs' and apps' data flow and privacy policies.
% %
% \xiancm{rewrite the above two items, it seems like they can combine together}


% \xiancm{one item can say the released dataset but you need to give the link, besides, SE usually need to release the code, the other item can say your performance is good, ok.}
% \item We build a data set including a) labeled privacy policies in two languages, b)TPLs with data leakage behavior, and c) host apps with labels concerning used TPLs and data interaction with TPLs.
% %
% We evaluate the performance of {\oursystem} on created dataset and disclose the harm of TPL data leakage in a large scale.
% %



\end{itemize}









\begin{comment}
%
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.






This is introduction
\subsection{Our target}


\begin{itemize}
    \item We have to identify whether the action of {\tpl} is consistent with {\tpl}'s privacy policy.
     
    \item We need to detect all data usage (at least sensitive data usage) in APP. And specify which groups are used by app and which groups are used by {\tpl}.
    
    \item
\end{itemize}


Tool name: {\oursystem} Android Third party libraries misuse and Privacy policy conflict checker.

\subsection{Challenges}

\textbf{1. {\tpl} information extraction}: Information about the usage of {\tpl}, the data related to {\tpl} are usually formatted as a table or organized as form of explanations (for example, facebook: data1, data2 \kaifa{put a case study in Appendix}).
%
% We apply \texttt{Tablemaster} to extract information from tables and \kaifa{a new NLP technique} to merge information in form of explanations.
\kaifa{not suitable. I analyze 3502 privacy policy. Only 471/3502 privacy policy contains html tag \textit{table}. I manually checked 200/471. Only 6/200 contains table are related to data usage that cannot be analyzed by the method in PolicyLint.}

PolicyLint~\cite{andow2019policylint} deals with the table data by merging the formatted lists into sentences.
%
This preprocessing method fails when only noun phrase on the table because the method in PolicyLint directly merges the items together without considering the characteristics of table, i.e., the data in each item shares same attributes. \kaifa{give an example in appendix}
%


\textbf{2. Data analysis in third party libraries. }
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
For dynamic analysis,  we must find the apk that uses the {\tpl} and leverage the data usage of {\tpl}. 
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.
%
\kaifa{details, how to design such a tool}


\textbf{3. Consistency analysis} We focus on two aspect of consistency analysis: a) whether the app's privacy policy covers all {\tpl} usage. 
%
To relax condition, the app's privacy policy should contain all {\tpl}s that collect or share data.
%
b) If the app's privacy policy covers the {\tpl} usage, does the data usage in privacy policy consistent with the {\tpl}'s real data usage.

\end{comment}

==> tmp/limitation_0105.tex <==
\section{Discussion}


\kaifa{
{\oursystem} our system is designed to identify the compliance between TPLs' behavior and privacy policies, and host apps' TPL usage and privacy policies.
TPLs are mainly used as an additional part of apps to enhance app functionalities and may not be responsible for data access behaviors or work in the role of data controllers as defined in GDPR. 
%
However, we can not assume all TPLs only conduct user data access behavior for assisting apps. 
%
Existing work~\cite{tangtse:21a, meng2016price, liu2016alde} has demonstrated that development tool TPLs, such as firebase~\cite{tangtse:21a}, may leak users’ privacy without developers' consciousness.
%
Besides, regulations, such as GDPR Article 35 and SGSDK Article 5.3, request clearly giving the purpose of data processing. 
%
Even if we could assume TPLs only access user data for specific functionalities and would never share or collect the data, we still recommend TPLs provide privacy policies to clearly state their user data access behavior and related purpose.
%
This can not only help app developers better understand TPL's functionalities but also help TPL developers suffer from legal disputes.
%
Thus, we assume all TPLs should provide privacy policies when evaluating {\oursystem}.
%
Next, we discuss the limitation of {\oursystem}, threats to validity and future work.
}



\subsection{Limitations}
{\oursystem} is designed to identify whether TPLs' personal information usage complies with regulations and whether host apps' TPL usage complies with regulations.
% regulation compliance between TPLs' privacy policies and personal information operations, and host apps' privacy policies and usage of TPLs.
% data leakage in TPLs and host apps and whether their privacy policies satisfy regulation requirements.
%
{\oursystem} is limited to analyzing TPLs and corresponding privacy policies under the version we collect the data and documents.
%
TPLs' functionalities keep changing with the update of the TPL versions.
%
It is still available to trace TPL versions from {\maven}, but not easy to trace the privacy policy of corresponding versions.
%
Besides, {\oursystem} is built upon static analysis (i.e., soot and flowdroid).
%
% Thus, {\oursystem} may miss some dynamic characters of TPLs, such as reflection, and is limited to analyzing large apk files~\cite{arzt2014flowdroid}. 
{\oursystem} cannot handle some dynamic behaviors of TPLs (e.g., reflection, dynamic class loading) and it cannot process large apk~\cite{arzt2014flowdroid} files due to the limited memory space. 
%
Furthermore, {\oursystem} cannot handle host apps in the format of \textit{xapk} which is created by Apkpure~\cite{apkpure}.
%
Besides, TPL non-compliance identification research is still limited to large-scale labeled data sets. 
%
We only crawl the TPL list and the top 10 host apps from {\appbrain} as the role of academic researchers.
%
% Labeling privacy policy documents, TPL data trace, and apps' usage of TPLs are both laborious and challenging to guarantee accuracy.
It is very laborious to label privacy policies and ground truth of data usage in software and privacy policies.
%
\kaifa{
Besides, {\oursystem} are limited to pre-defined patterns and string matching to identify the statements and TPL usage in collected privacy policies.
%
{\oursystem} will fail detection once those adversaries target our detection tool and conduct adversarial attacks~\cite{boucher2022bad, zhao2021structural} using novel patterns to hide their data usage statements.
}



\subsection{Threats to Validity}
(I) The first threat comes from the language used in privacy policies, it is not trivial to identify and switch the language of privacy policy during the collecting phase, which may lead to missing collection of some privacy policies.
%
% As some TPLs or apps are developed by different countries, such as China or Korea, the default language used in the privacy policy website are provided using their native language.
As TPLs or apps are published in different countries, such as China or Korea, the default language used in the privacy policy website is provided using their native language. 
%
(II) Another threat comes from inconsistent  versions of TPLs and their privacy policies.
%
Notice that all our data is collected from Feb-2022 to Apr-2022.
%
There may be cases where the TPL or app functions have been updated, but the privacy policies have not been updated in time. 
%
This can lead our system to misidentify that the behavior of the software is inconsistent with the privacy policy and violates regulation requirements.
We will mine software and privacy policy version issues in future work.



\subsection{Future work}


To further improve {\oursystem}, we will integrate analyzing the data collection purpose into {\oursystem}.
%
When analyzing privacy policies of TPLs or apps, {\oursystem} analyzes data usage-related statements but is limited to analyzing the purpose.
%
During our analysis of privacy policy documents, we believe that purpose descriptions can help researchers 
1) better understand the code or functionalities and 
2) more precisely understand whether apps violate regulation requirements.
%
In future work, we will investigate more information and integrate them into {\oursystem}.
%
Furthermore, writing legal privacy policies remains a challenging and time-consuming work for TPL developers.
%
Automatic privacy policy generation methods are under urgent needs.
% for TPL and apk developers.
%
Although there existing privacy policy generation methods~\cite{le2015ppg, zimmeck2021privacyflash} for APKs, those methods are not suitable for generating privacy policies for TPLs.
%
In future work, we will develop automatic TPL privacy policy generation methods by combing regulations requirements analysis~\cite{zhSDKLaw, gdpr, ccpa}, natural language processing methods~\cite{zhao22ca4p} and TPL analysis techniques.  



==> tmp/method_old_0831.tex <==

% \input{table/abbreviation_table}

% \input{table/data_type_table}

\section{Methodology}
In this section, we will introduce how {\oursystem} identifies data usage in TPLs' code (\S\ref{sec:tpl_data}) and how to identify the consistency of TPLs' data usage with the statements in privacy policies (\S\ref{sec:tpl_pp}).
We will also describe how to determine whether host apps describe TPLs usage correctly in their privacy policy (\S\ref{sec:host_app_pp}) and whether host apps use TPLs correctly(\S\ref{sec:host_app_data}) or not.
%
Figure.~\ref{fig:sys_frame} shows the framework of {\oursystem}.
 

\begin{figure*}[t]
    % \vspace{-2ex}
    \centering
    \includegraphics[width=0.66\textwidth]{figures/framework_win.pdf}
    % \vspace{-0.5ex}
    \caption{Framework of {\oursystem}}
    % \vspace{-1.5ex}
    \label{fig:sys_frame}
\end{figure*}



\subsection{Identify personal information usage in third-party library}
\label{sec:tpl_data}


This section introduces how {\oursystem} identifies personal information (PI) usage in TPL's code.
%
Given the APK files of Android apps, {\oursystem} analyzes TPL's PI usages by performing static analysis with {\soot}~\cite{soot}. % and does not require source code.
%
{\oursystem} analyzes TPLs' data flow analysis, specifically variable use-define analysis~\cite{defuse94}, to locate data of interested (DOI) (Tab.~\ref{tab:data_type}).
%
Our data flow analysis uses function call graphs (FCG) to trace PI flow among methods.
%
However, soot cannot precisely construct FCG to investigate the function invocations~\cite{arzt2014flowdroid}. 
%
Our analysis discovers that the soot cannot effectively discover the TPL's main functions and entry points to construct a valid FCG.
%
Thus, we propose the following methods to optimize the FCG construction process and improve the precision of the data flow analysis.




\begin{comment}

% Intuitively, each method in TPLs can be invoked and further used by the host apps to use the TPL's functionalities.
%
% Thus, when we use static analysis to analyze data flow in TPLs, it is hard to find and determine natural entry points to start the analysis.
%
% To counter the challenges, our solutions are given as follows

 
% There are two challenges in analyzing TPLs.
% %
% \textbf{C1.} TPLs generally can not run independently without host apps that limit the application of dynamic analysis.% for analyzing TPLs.
% % 
% To counter this challenge, {\oursystem} applies static analysis to identify data usage in TPLs.
% %
% \textbf{C2.} No explicitly entry points or main function for TPLs to start analysis.
% %
\end{comment}



% \input{table/PI_related_API_list}


\begin{comment}

% {\oursystem} conducts data flow analysis based on top of {\soot}~\cite{lam2011soot} as {\soot} is widely used for java code analysis and does not require the source code.
% %
% In this way, {\oursystem} is capable of analyzing TPLs in form of \textit{jar} or \textit{aar} files that are publicly available for usage in \textit{mvnrepository}~\cite{mvnrepository}.
% %
% However, when analyzing the data flow in TPLs, we still require entry points to start our analysis.
%
\end{comment}



\begin{table}[]
\centering
\smaller
% \vspace{2ex}
\vspace{3.5ex}
\caption{Tracked data types in static analysis}
\begin{tabular}{p{0.9\columnwidth}}
\toprule
\textbf{Data Type} \\ \midrule
Ad ID, username, password, name, location, contact, phone number, email address, IMEI, Wi-Fi, MAC address,  GSF ID, Android ID, serial number, SIM serial number \\ \bottomrule
\end{tabular}
% \vspace{-1ex}
\label{tab:data_type}
\end{table}



\begin{table}[]
\centering
\smaller
\vspace{1ex}
\caption{Personal information and corresponding APIs}
% \vspace{-1ex}
\scalebox{0.95}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.14\textwidth}@{}}
\toprule
\textbf{PI}                    & \textbf{Class Name}                                      & \textbf{Method Name}                         \\ \midrule
Ad ID                          & AdvertisingIdClient                                      & AdvertisingIdClient                          \\
\rowcolor[HTML]{EFEFEF} 
Bluetooch address              & android.bluetooth.BluetoothAdapter                       & getAddress                                   \\
Camera                         & android.hardware.Camera                                  & setPreviewDisplay                            \\
\rowcolor[HTML]{EFEFEF} 
Cell   Loca-tion                & android.telephony.TelephonyManager                       & getCellLocation                              \\
Contact                        & android.provider.ContactsContract                        & PhoneLookup                                  \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude          \\
                               & android.location.Location                                & getLongitude                                 \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLastKnownLocation \\
                               & android.location.LocationManager                         & requestLocationUpdates                       \\
\multirow{-5}{*}{GPS Location} & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLongitude         \\
Sim Number                     & android.telephony.TElephonyManager                       & getSimSerialNumber                           \\
\rowcolor[HTML]{EFEFEF} 
IMEI                           & android.telephony.TElephonyManager                       & getDeviceId                                  \\
IMSE                           & android.telephony.TElephonyManager                       & getSubscriberId                              \\
\rowcolor[HTML]{EFEFEF} 
Location                       & java.util.Calendar                                       & getTimeZone                                  \\
MAC address                    & android.net.wifi.WifiInfo                                & getMacAddress                                \\
\rowcolor[HTML]{EFEFEF} 
Password                       & android.accounts.AccountManager                          & getPassword                                  \\
Phone   Number                 & android.telephony.TelephonyManager                       & getLine1Number                               \\
\rowcolor[HTML]{EFEFEF} 
SMS                            & android.telephony.SmsManager                             & sendTextMessage                              \\
SSID                           & android.net.wifi.WifiInfo                                & getSSID                                      \\
\rowcolor[HTML]{EFEFEF} 
User Credential                & android.accounts.AccountManager                          & getAccounts                                  \\
UserName                       & android.os.UserManager                                   & getUserName                                  \\ \bottomrule
\end{tabular}
}
\vspace{-2ex}
\label{tab:pi_api}
\end{table}

\noindent\textbf{TPL FCG construction: }
%
{\oursystem} first 
% uses {\soot} to get the intermediate representation (IR) of a TPL and 
iterates over each class and method.
%
{\oursystem} identifies the methods that \textsf{a)} are not concrete~\cite{soot}, \textsf{b)} possess active method bodies and \textsf{c)} are \textit{publicly} accessible.
%
{\oursystem} extends the extracted methods to entry points set to optimize the initialization of FCG construction process.
%


\noindent\textbf{TPL DOI identification: }
%
% {\oursystem} focuses on personal information (PI) listed in Table~\ref{tab:data_type} to locate variables.
% %
% Based on PI names, we extract related Android APIs~\cite{androidDeveloper} (Table~\ref{tab:pi_api}) to improve variable locating precision.
% %
% Because if we only use string matching with data type names, many false-positive statements will be located~\cite{yu2016can}.
%
We first summary personal information (PI) from regulations~\cite{gdpr,ccpa,zhSDKLaw,piss} as listed in Tab.~\ref{tab:data_type}.
%
Then, we manually crawl PI-related APIs~\cite{androidDeveloper}.
%
Based on those APIs, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
{\oursystem} analyzes the data flow inter- and intra-methods to identify all PI-related statements.
%
% For example, if we want to locate data flows that collect \textit{sim} information, we may locate
% the statements as
% \textit{"virtualinvoke \$r1.$\langle$android.os.Bundle: void putSerializable( java.lang.String, java.io.Serializable )$\rangle$( "fractionProgres\underline{sIm}pressions-Sent", \$r2 )"} that is not related to personal information.
%
% Then, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
% Finally, {\oursystem} performs forward analysis and backward analysis~\cite{arzt2014flowdroid, zhou2021finding} to trace the inter-methods and intra-methods data usage.



% 可以加个algorithm
\input{figures/algorithm_data_flow}

The method used for extracting the TPL data usage extraction is shown in Algorithm ~\ref{alg:data_usage}. %methods in {\oursystem}. 
%
% With the intermediate representation (i.e., Jimple in {\soot}), we get the method body, the method's statements and target variables.
%
{\oursystem} iterates over all statements in TPL to locate the target variables ($var$) saving the personal information listed in Table~\ref{tab:data_type}).
%
Then, {\oursystem} conducts both inter-procedure and intra-procedure analysis to get the data flow.
%
For inter-procedure analysis, {\oursystem} starts backward analyzing from the statement $s_t$ in method $m_t$ with the DOI $v_t$ (Alg.~\ref{alg:data_usage} line 1).
%
% construct the control flow graph (CFG) of current methods ($m_{src}$) using soot.
% Specifically, for backward analysis, {\oursystem}
The backward analysis first locates the definition statements ($defs$) in $m_t$ that relates to DOI $v_t$ (Alg.~\ref{alg:data_usage} line 11).
%
For statements in $defs$, {\oursystem} iterates $defs$ and locates the variable signature of $v_t$ in $d$ (Alg.~\ref{alg:data_usage} line 12-13).
%
Then, {\oursystem} iterates the function call graph of TPL and finds the methods ($caller_{list}$) that invoke $m$ (Alg.~\ref{alg:data_usage} line 14).
%
For each caller $m$, {\oursystem} locates the statements ($src_{stmt}$) in $m$ that invoke $m_t$.
%
Then, {\oursystem} finds the variable ($src_v$) in $src_{stmt}$ that corresponds to DOI $v_t$ (Alg.~\ref{alg:data_usage} line 17).
%
If $src_{v}$ is a variable, {\oursystem} continues backward analysis, starts with $src_{stmt}$ in $src_m$ and focuses analysis on variable $src_v$ (Alg.~\ref{alg:data_usage} line 18-19); 
% otherwise, 
if $src_{v}$ is a constant, {\oursystem} determines one piece of code that describes the data usage of $var$ (Alg.~\ref{alg:data_usage} line 21).


To locate the $v_t$'s data usage in the method $m_t$, {\oursystem} performs \textit{intra-methods variable analysis}.
%
Specifically, {\oursystem} locates all statements ($uses$) that uses $var$ in method $m$. (Alg.~\ref{alg:data_usage} line 5).
%
For each statement $u$ in $uses$, {\oursystem} stores the usage of variable $var$ (Alg.\ref{alg:data_usage} line 7) because the target variable have been used in the statement $u$.
%
Then, {\oursystem} use forward analysis (line 8) to identify whether the variable $var$ is used further.
%
% Specifically, {\oursystem} locates the statements ($tar_{stmt}$) that contain $stmt$ because the $stmt$ maybe invoked in some \textit{specialinvoke} statements accordingly to the prosperity of {\soot}.
%
Then, for each statement $s$ in $tar_{stmt}$, {\oursystem} stores the the data flow describing the data usage. 
% data usage.
%
If $s$ contains invoke statements, {\oursystem} locates the method $tar_m$ that calls $stmt$ (Alg.\ref{alg:data_usage} line 28), builds the variable $tar_v$ corresponds to target variable $v_t$ and continue the forward analysis (Alg.\ref{alg:data_usage} line 30).
%


% \kaifa{todo: add the obfuscation detection； 1）用了mamadroid 的检测string encryption的方法；2）XFinder 检测 reflection 的方法，但未发现 TPL -- jar,aar-- 有此类现象}



% %
% Then, we get the statements that defines $var$ in $m_{src}$ through analyzing the CFG using \textit{soot}.% API.
% % We get the definition sites for $var$ at a certain point (statement) that defines $var$ in the method.
% %
% Next, we traverse the call stack in reverse to find the the statement that initially defines target variable.
% %
% Then, we get the data flow of target variable.
% %
% For intra-procedure analysis, we iterate the statements in current method ($m_{src}$) to trace the data flow.
% %
% It worth noticing that when we find recursive invocation, we terminate the current traverse to avoid redundant analysis.



%update:25-Jan-2022:
%
%Figure out the problem that flowdroid cannot be directly used to analyze \textit{dex/jar} files.
%
%To deal with it, we write methods based on soot and soot-infoflow.
%
%Currently, we can analyze the data flow of specific methods.
%
%Demo: 
%
%\textbf{APK}: E133-3A32B-15F79-A6AA6-6CB57-FA7FC-648AC-68351-6ECDE-7399B-89999-14012-474F2.apk
%
%\textbf{Target}: location
%r
%\textbf{dataflow:}



% How to define \textbf{\textit{callback}} methods?

%%%\textbf{Questions:} When analyzing \textit{.jar} file, the \textit{infoflow} can find the target trace, e.g. the \textit{location} in aforementioned case. 
%However, when analyzing \textit{.dex}, the trace missed.
%
%Another interesting thing is: when analyzing the demo using \textit{soot} only, the results of \textit{.dex} returns more invocation results than results of \textit{.jar}.
%There could be some problems in \textit{dex2jar}.



\vspace{-1ex}
\subsection{Identify data usage statements in TPL's privacy policy}
\label{sec:tpl_pp}

% Privacy policy analysis 
% Data usage identification is a kind of named entity recognition (NER) task in natural language processing.
%
TPLs' privacy policy analysis aims at identifying the data usage statements in the documents.
%
{\oursystem} analyzes TPLs' privacy policy to extract used data.
%
The pipeline of our privacy policy analysis consists of three steps: 
1) preprocessing of privacy policy,
2) named entity extraction, 
and 3) data usage action construction.
%
Finally, each privacy policy is abstracted into a set of abstract data usage patterns (ADUP) that describe \textit{who} will (\textit{not}) \textit{access} \textit{what kinds of data} with \textit{whom}. 
%
Each ADUP is in form of $\{data\_entity, action, \{data\_type\}, \{data\_recipient\}, \{neg\}\}$.
%
For example, the sentence ~\textit{"We may share your private personal information with our service providers," (in Adad's privacy policy)} is abstracted as \textit{\{app, share, \{personal information\}, \{service provider\}, false\}}.
%The extraction methods for each component of ADUP is detailed as follows.


% 1) fined-turning a state-of-the-art NER model to adapt our application scenario, 2) identifying data entities in privacy policy using pretrained model, and 3) applying expert system to identify the data usage in privacy policy.

\subsubsection{Preprocessing privacy policy}
\label{sec:pre_pp}
To download the apps' privacy policies from Google Play~\cite{googleplay},
we use the \textit{Selenium Webdriver}~\cite{gojare2015analysis} to open web pages of privacy policies with the Chrome browser.
%
Then, we use \textit{html2text}~\cite{html2text} to transform the download privacy policies into plain text.
%
However, the transformed plain text contains many special characters, e.g. $*$, $|$, that may lead to unnatural segmentation of sentences.
%
{\oursystem} first uses patterns~\cite{stack_pre_nlp} to eliminate noisy characters.
%
% Besides, enumeration items are in privacy policies to detail the related data items.
%
Besides, privacy policies use enumeration items~\cite{andow2019policylint} to detail related data items, which may lead to a whole sentence being segmented by item index and further cause information lose.
%
{\oursystem} merges the items by searching for sentences ending in a colon, and the next sentence starts with list items, such as bullets, roman numerals, and formatted numbers.
%
% Then, we use the dependency parse tree to get the constellation between words.
%


\subsubsection{Data access extraction}
%
With preprocessed privacy policy sentences, {\oursystem} analyzes each sentence to identify data access descriptions.
%
Since the interrogative sentence are commonly used in privacy policies but they do not describe the types of accessed personal information, we omit them by checking the interrogative words (i.e., who, where, when, why, whether, and what, how). 
%this sentence as it would be an \textit{Introduction}, 
For example, the sentence \textit{\underline{What} personal information do we collect} is omitted. %  (appid: wp.wattpad).
%
Then, we construct the part-of-speech (POS) tagging, and dependency parsing tree (DPS) for each sentence.
%
We will omit sentences without verb words because those sentences will not claim data access behaviors.
%
For example, ``\textit{Do-Not-Track Signals and Similar Mechanisms}" in \textit{Facebook Open Source Privacy Policy} only claims the title of the paragraph.
%
Then, for the remaining sentences, we follow the following steps to extract data action, data entity, and data actor.
% data action, data objects, data operator, and data recipient (if applicable).


\begin{table}[]
\centering
\smaller
\vspace{3.5ex}
\caption{Data sharing and collecting words}
%p{0.9\columnwidth}
\begin{tabular}{p{0.23\columnwidth}p{0.67\columnwidth}}
\toprule
\textbf{Action Type} & \textbf{Keywords} \\ \midrule
Collect     &  access, check, collect, gather, know, obtain, receive, save, store, use \\ \hline
Sharing     &  accumulate, afford, aggregate, associate,  cache,  combine, convert, connect,  deliver, disclose, distribute, disseminate, exchange,  gather, get, give, keep, lease, obtain, offer, post, possess, proxy,  provide, protect against, receive,  rent, report, request, save, seek, sell, share, send, track,  trade, transport, transfer, transmit\\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:actionwords}
\end{table}


%
\noindent\textbf{Identification of data action words}. 
%
We first identify whether the verb words are in the data usage word list (Table~\ref{tab:actionwords}).
%
It is worth noting that, we stem the word using \textit{nltk} library~\cite{loper2002nltk} %before identification 
since English verbs have tenses.%, singular or plural forms.
%
% Besides, we will identify the verb as some statements that claim the data sharing and collection action in one sentence, for example: \textit{we \underline{collect} the information you have authorized the platform to \underline{share} with us, such as your name, email address, gender, date of birth, friend list, profile picture and playlists}(us.current.android).
%
We also identify the modifier of target verb, because the privacy policies also claim the data that they will not use or collect.
%
To achieve this, we analyze the dependency parsing tree and recognize the words whose relation with the target verb are '\textit{advmod}' (adverbial modifier) or '\textit{mmod}' (modal verb modifier).
%
Then, if the words are negation words (e.g., 'not', 'no')  or its tag is negative (i.e., 'neg'), we regard the data usage action as a negative one.
%
To this end, {\oursystem} determines the data-related sentences, and data sharing or collection operations.


%\vspace{1.5ex}
\noindent\textbf{Identification of data entity}.
%
We identify objects of identified collecting and sharing words (target verb) according to DPS.
%
{\oursystem} first merges the noun phrase (NP) tag into one noun tag according to POS tagging to simplify sentence structure because many compound noun exists in sentence to describe the related data.
For example, consider the following sentence in the privacy policy of the app \textit{video.reface.app} \textit{With the use of Google Analytics, we collect such data as IP-Address, your \underline{device model}, \underline{screen resolution} and \underline{operation system}, \underline{session duration}, your location}.
%
Then, {\oursystem} identifies the objects of the target verb.
%
As only one noun or noun phrase will be identified as the object of the target verb~\cite{hanlp21}, {\oursystem} locates all coordinating nouns for the object.
%
Specifically, {\oursystem} iterates the constituency parsing tree, that are calculated by two stage conditional random field (CRF) model~\cite{zhang2021fast}, to find the sub-trees whose \textit{a) root label are common noun ('NN' tag) or Noun Phrase ('NP)} or \textit{b) coordinating conjunction ('CC' tag) or punctuation exist in the sub-tree}.
% 
The condition \textit{a)} denotes that the leaves in the tree can be merged into one noun, and  \textit{b)} indicates there may exist enumeration items or coordinating nouns.
%
If we omit the relations, {\oursystem} cannot fully extract all data entities, i.e., false-positive occurs.
%
To this end, we obtain all candidate data objects in each sentence.
%


%\vspace{1.5ex}
\noindent\textbf{Identification of data actor.}
%
To identify the data actor, {\oursystem} analyzes DPT and finds the words whose relation with sharing and collection verbs is nominal subject ("\textit{nsubj}") or direct object ("\textit{dobj}").
%
% Besides, if the sentence or the object is prepositional complement or clausal complement of a preposition, we will iterate the DPT to find the coordinating verb and then locate the nominal subject of coordinating verb.
Besides, suppose the sentence or the object is a prepositional complement or clausal complement of a preposition (ccomp). In that case, we will iterate the DPT to find the coordinating verb and then locate the nominal subject of the target verb.
%
Then, the nominal subject and the verb will be added to the actor list and the sharing/collection verb list, respectively.
%
% \kaifa{add an example here.}
%
We also consider the data actor as users separately, under which situation the real data actor is the user rather than the supplier.
%
For example, '\textit{we will not collect the personal information you shared with us}'.
%
The data actor should be 'you' (users) while the data recipient is 'we' (privacy policy owner).

% Besides, for the object complementary cases, (i.e., \textit{"we will ask you to provide personal information that is necessary to provide those services to you"})

% \noindent\textbf{Data recipient identification.}
%

%\vspace{1.5ex}
\noindent\textbf{Post-process}
%
To eliminate false detection, e.g. conditional clauses, we design the following rule to avoid false data usage extractions.
%
For sentences start with condition or assumption hints, such as \textit{'if'} (\textit{"if you do not provide your personal information"}), we will not identify the data usage pattern inside (i.e., \textit{\{you, not provide, personal information\}}).


\begin{figure}[t]
    \centering
    \vspace{0.5ex}
    \includegraphics[width=0.45\textwidth]{figures/demo_tpl_parameter.pdf}
    % \vspace{1ex}

    \caption{Demo: TPL as parameters in statements (app:\textit{"br.com.tapps.chicago.bruger.truck"})}
    \vspace{-1ex}
    \label{fig:demo_tpl_para}
\end{figure}

\subsection{Extract host apps' interaction with TPLs}
\label{sec:host_app_data}

% \subsection{Data Sharing with Enumeration}
% \label{app:demo:tpl_enumeration}

{\oursystem} performs static analysis to identify the host apps' interaction with TPLs.
%
{\oursystem} aims at identifying what kinds of PI data (listed in Table~\ref{tab:data_type}) are shared with TPLs.
%
{\oursystem} uses Flowdroid~\cite{arzt2014flowdroid} to construct the function call graph (FCG) of apps.
%
{\oursystem} does not use the methods in \S\ref{sec:tpl_data} to construct the entry points of apps because Flowdroid prepossesses apps' Manifest and resources files to identify the entry points and create the dummy main function~\cite{arzt2014flowdroid}. % that are proven to be more comprehensive and effective~\cite{arzt2014flowdroid}.
%
Then, {\oursystem} iterates each statement to locate the variables related to TPLs or PI.
%
{\oursystem} performs the data flow analysis (\S\ref{sec:tpl_data}) to find the PI related data flow.
%
To identify TPLs, {\oursystem} identifies whether the statement contains the TPLs' name or package name or not.
%
After obtaining the data flows of TPLs and PI data, we identify whether the sinks exists in the data flows.
This is done by using FlowDroid~\cite{arzt2014flowdroid}.
%
Besides, we optimize the signature of sink invocation (\textit{SSI}) as the invoke statement.
% signature of the method that invokes the sink concreting the signature of the sink methods.
%
For example, if the sink method ~\textit{$\langle$android.content.Intent: android.content.Intent setAction(java.lang.String)$\rangle$} is invoked in statement: (\textit{JimpleLocalBox(\$r1) in virtualinvoke \$r1.$\langle$ android.content.Intent: android.con-tent.Intent setAction( java.lang.String ) $\rangle$  
( "com.google.android.gms.-fitness.app\_disconnected" )} 
% (\textsf{st1} )
, we use the the whole invocation statement as the stored signature.
%
Then, {\oursystem} matches the SSI in both PIs' data flow and TPLs' data flow.
%
Once the SSI matched between $TPL_i$ and $PI_j$, {\oursystem} regards the host app shares the $PI_j$ with the $TPL_i$.
%
If the SSI only exits in $PI_j$'s data flow, {\oursystem} will identify the host app collects $PI_j$  without sharing it with TPLs.




\subsection{Identify TPLs usage statements in host apps' privacy policy}
\label{sec:host_app_pp}

To identify the TPL usage statements in host {\app}s, we extract two descriptions from the privacy policy: 
%
a) the \textit{data sharing} related statements, and 
b) TPL related  descriptions.
%
The \textit{data sharing} related statements claim how the {\app} discloses users' personal information under what kinds of situations.
%
For example, the {\app} (\textit{flipboard.boxer.app}) claims that "\textit{We share personal information with vendors and service providers that help us offer and improve our service}" in their privacy policy.
%
The statement denotes that \textit{flipboard.boxer.app} will share users' \textit{personal information} with vendors and service providers.
%
If {\oursystem} also identifies the {\app}'s data flow sharing users' data with TPLs tagged as vendors or service providers, {\oursystem} regards the app's privacy policy consistent with its behavior.
%
Besides, some {\app}'s privacy policy will enumerate the TPLs they used and the data they shared with TPLs. % (see demo in~\ref{app:demo:tpl_enumeration}). 
%
% The patterns are extracted from our manually labeled 400 privacy policies (200 for Chinese and English separately).
%
% The patterns are extracted from our manually labeled 200 privacy policies.


First, we use methods in \S\ref{sec:pre_pp} to preprocess TPLs' privacy policy.
%
Then, we use NLP tool (i.e., \textit{hanlp}) to get the the tokenization, POS tagging and DPS for each sentence.
%
For sentences with verbs, we check whether the verb is in SHARING word list (Table~\ref{tab:actionwords}).
%
After obtaining the data sharing verb, we need to identify the data recipient to determine which TPLs the data are shared with.
%
Specifically, we iterate the words in the sentence.
%
If the word is object of a preposition (\textit{pobj}) or an indirect object (\textit{iobj}) of the verb, we will identify the words as candidate data recipient, i.e., TPLs.
%
For enumeration patterns, once we identify the sentence that a) starts with a noun or noun phrase (denoted as $tar_{TPL}$) that involved in our TPL list, v) the noun ends with colon following only noun or noun phrases, we will regards the noun (phrases) following colon as the shared data with $tar_{TPL}$.

%There are two types of action:
%1) "We may collect \textbf{data} from third parities."
%2) "We share \textbf{data} with third parties."

\subsection{TPL vulnerability investigation}


{\oursystem} investigates TPL vulnerabilities by performing
 normativeness analysis, % 规范性分析
 privacy policies legality analysis, % 合法性分析
and  vulnerability transmissibility analysis. % 传播性分析


\noindent\textbf{Normativeness analysis} identifies whether TPL provides privacy policies.
%
According to GDPR Article 12 (1)  and  Article 13 (1), TPLs, who act as the data controller or third party of personal data, should infer users about data access behaviors in a concise, transparent, intelligible and easily accessible form.
%


\noindent\textbf{Legality analysis} identifies conflicts between TPLs' behavior and privacy policy statements.
%
Specifically, {\oursystem} identifies whether TPLs' data access action are clearly claimed in their privacy policies by combining the data flow results (\S\ref{sec:tpl_data}) and PP ADUP (\S\ref{sec:tpl_pp}).
%
If {\oursystem} identifies data usage in TPL data flow results are not mentioned in \textit{$data\_type$}s of ADUP set, the TPL will be regarded as violate legal requirements.



\noindent\textbf{Vulnerability transmissibility analysis} checks what extend the TPLs with vulnerabilities will affect other TPLs or host apps.
%
To achieve this, {\oursystem} counts the number of  artifacts that use vulnerable TPLs from {\textit{Maven Repository}}.
%



\subsection{Regulation conflict analysis}

Regulation conflict analysis discovers whether the usage of TPLs in host apps comply regulation requirements.
Two kinds of conflict will be identified:

\begin{itemize}
    \item {\oursystem} identifies whether usage of TPLs from data flow analysis (\S\ref{sec:host_app_data} are clearly claimed in their privacy policy statements(\S\ref{sec:host_app_pp}. To achieve this, {\oursystem} investigate whether the TPL package names in data flow analysis matches the \textit{$data\_entity$} or \textit{$data\_recipient$} in ADUP set of host app privacy policy results.
    
    \item For host apps that disclose their interaction with TPLs, {\oursystem} also identifies whether the data usage of TPLs, that is achieved from data flow analysis of TPLs (\S\ref{sec:tpl_data}), are clearly and comprehensively disclosed in host apps privacy policies.
\end{itemize}



% \subsection{Extract data usage in host {app}'s privacy policy}

% In this subsection, I wil; introduce how to analyze the data usage of TPL through analyze the TPL bytecode.

% We should target specific sensitive data, in this way we can identify the DataFlow of TPL:

% Email, userid, username, password, contact, gps, location, device ID, identifier, advertising ID, account/imei address, PHOTOGRAPHY


% To identify the TPL usage in our 




\begin{comment}


\subsubsection{Demo}

package name = \textbf{"com.facebook.ads"}

    

    

%\begin{itemize}
%    \item \textbf{email}  
    % SPECIAL edge: specialinvoke \$r15.$\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$( \kaifa{"EMAIL"}, 15, "email" ) in $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$() $\rangle$ ==$\rangle$ $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$
    
%    \item \textbf{userid} 
    % VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\kaifa{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$
    
%    \item \textbf{deviceid} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$("Stub!") in $\langle$android.view.InputDevice: int[] \kaifa{getDeviceIds()} $\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$

 %   \item \textbf{identifier} 
    % VIRTUAL edge: \$r3 = virtualinvoke r1.$\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$() in $\langle$com.facebook.ads.internal.bridge.gms.AdvertisingId: com.facebook.ads.internal.bridge.gms.AdvertisingId getAdvertisingIdInfoDirectly(android.content.Context)$\rangle$ ==$\rangle$ $\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$
    
%    \item \textbf{account} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$("Stub!") in $\langle$android.content.ContentResolver: boolean isSyncPending(android.accounts.Account,java.lang.String)$\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$


    
%    \item \textbf{photo}: 
    % SPECIAL edge: specialinvoke \$r38.$\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$(\kaifa{"PHOTOGRAPHY"}, 38, "photography") in $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$()$\rangle$ ==$\rangle$ $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$
    
%\end{itemize}



% For data that android system provides API to collect, such as location, we identify the invocation of those methods. \kaifa{to list the related API in appendix}
% %
% For other data, such as gender or username, we identify the parameters passed to target server.
% %
%such as:  \textit{VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\textbf{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$}

\end{comment}











\begin{comment}

In this subsection, I will introduce how to analyze data usage in app and whether the data is used by host app or TPL.
%
\kaifa{PoliCheck had done this through dynamic analysis. However, dynamic analysis can not cover all data flow. \textbf{we need a case study to demonstrate that.}
For example, PoliCheck only identifies whether the collected data flows are mentioned in Privacy Policy but not identifies whether the data in privacy policy are really in app's code (that's also a limitation of dynamic analysis);
%
PoliCheck only identifies TPL of popular advertisers and analytic providers.
} 
\end{comment} 


==> tmp/methodolody_0105.tex <==

% \input{table/abbreviation_table}

% \input{table/data_type_table}

\section{Methodology}
% In this section, we will 
This section introduces how {\oursystem} identifies data usage in TPLs' bytecode (\S\ref{sec:tpl_data}) and how to identify the consistency of TPLs' data usage with the statements in privacy policies (\S\ref{sec:tpl_pp}).
We will also describe how to determine whether host apps describe TPLs usage correctly in their privacy policy (\S\ref{sec:host_app_pp}) and whether host apps use TPLs correctly(\S\ref{sec:host_app_data}) or not.
%
Fig.~\ref{fig:sys_frame} shows the framework of {\oursystem}.
 

\begin{figure*}[ht]
   % \vspace{-2ex}
    \centering
    \includegraphics[width=0.66\textwidth]{figures/framework.pdf}
    \vspace{0.5ex}
    \caption{Framework of {\oursystem}.} 
    % \vspace{0.5ex}
    \label{fig:sys_frame}
\end{figure*}


\begin{table}[hb]
\centering
\smaller 
\vspace{1em}
% \vspace{3.5ex}
\caption{Tracked data types in static analysis.}
\vspace{-1ex}
\begin{tabular}{p{0.9\columnwidth}}
\toprule
\textbf{Data Type} \\ \midrule
Ad ID, username, password, name, location, contact, phone number, email address, IMEI, Wi-Fi, MAC address,  GSF ID, Android ID, serial number, SIM serial number \\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:data_type}
\end{table}


\subsection{Identify personal information usage in third-party libraries}
\label{sec:tpl_data}


% This section introduces how {\oursystem} identifies personal information (PI) usage in TPL's code.
%
Given the TPL binary files, {\oursystem} analyzes TPL's  personal information  (PI) usages by performing static analysis based on {\soot}~\cite{soot}. % and does not require source code.
%
{\oursystem} conducts data flow analysis, specifically variable use-define analysis~\cite{defuse94}, to locate data of interest (DOI) (Tab.~\ref{tab:data_type}). 
%
{\oursystem} uses function call graphs (FCG) to trace PI flow among methods. 
%
% However, soot cannot precisely construct FCG to investigate the function invocations~\cite{arzt2014flowdroid}. 
%
However, our analysis discovers that the soot cannot effectively discover the TPL's main functions and entry points to construct a valid FCG~\cite{arzt2014flowdroid}.
%
Thus, we propose the following methods to optimize the FCG construction process and improve the precision of the data flow analysis.






\noindent\textbf{TPL FCG construction: }
%
{\oursystem} first 
% uses {\soot} to get the intermediate representation (IR) of a TPL and 
iterates over each class and method.
%
% {\oursystem} identifies the methods that a) are not concrete~\cite{soot}, b) possess active method bodies and c) are \textit{publicly} accessible.
%
Since apks mainly use TPLs by invoking their \textit{public} methods, {\oursystem} extends TPLs \textit{public} methods to entry points set to optimize FCG construction.
% TPL's FCG construction.
% the identified methods to entry points set to optimize  
% the initialization of 
% FCG construction.
% process.
%


\noindent\textbf{TPL DOI identification: }
%
% {\oursystem} focuses on personal information (PI) listed in Tab.~\ref{tab:data_type} to locate variables.
% %
% Based on PI names, we extract related Android APIs~\cite{androidDeveloper} (Tab.~\ref{tab:pi_api}) to improve variable locating precision.
% %
% Because if we only use string matching with data type names, many false-positive statements will be located~\cite{yu2016can}.
%
We summarize 
% personal information 
(PI) from regulations~\cite{gdpr,ccpa,zhSDKLaw,piss} as listed in Tab.~\ref{tab:data_type}.
%
Then, we manually crawl PI-related APIs~\cite{androidDeveloper}.
%
Based on those APIs, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
{\oursystem} performs inter and intra-procedural data flow analysis to identify all PI-related statements. 
% {\oursystem} analyzes the data flow inter- and intra-methods to identify all PI-related statements.
%
% For example, if we want to locate data flows that collect \textit{sim} information, we may locate
% the statements as
% \textit{``virtualinvoke \$r1.$\langle$android.os.Bundle: void putSerializable( java.lang.String, java.io.Serializable )$\rangle$( "fractionProgres\underline{sIm}pressions-Sent", \$r2 )"} that is not related to personal information.
%
% Then, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
% Finally, {\oursystem} performs forward analysis and backward analysis~\cite{arzt2014flowdroid, zhou2021finding} to trace the inter-methods and intra-method data usage.

\begin{algorithm}[t]
% \vspace{-2ex}
\caption{Data usage analysis}\label{alg:data_flow}
\label{alg:data_usage}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  
  \KwInput{method $m_t$, statement $s_t$, variable $v_t$}
  \KwOutput{data usage $FD$ of variable $v_t$}
  
 

% Set Function Names
    \SetKwFunction{FInterMVA}{InterMethodVarAnalysis}
    \SetKwFunction{FIntraMVA}{IntraMethodVarAnalysis}
    \SetKwFunction{FForwar}{ForwardAnalysis}
    \SetKwFunction{FBackwar}{BackwardAnalysis}
  
    % BackwardAnalysis($src_{var}$, $src_{stmt}$, $src_{m}$)\;
    BackwardAnalysis($m_t$, $s_t$, $v_t$)\;

    IntraMethodVarAnalysis($m_t$, $s_t$, $v_t$) \;
    % \vspace{-1.1ex}\;\vspace{-1.1ex}
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FIntraMVA{$m$, $stmt$, $var$}}{
        $uses$ = find statements that use $var$ in method $m$ \;
        \For{$u$ in $uses$}{
            store($var$, u) in $DF$ \;
            ForwardAnalysis($m$, $u$, $var$)
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    \SetKwProg{Fn}{Def}{:}{\KwRet}
    \Fn{\FBackwar{$m_t$, $s_t$, $v_t$}}{
        % InterProcedureVariableAnalysis($m$, $stmt$, $var$)  \;
        % $cfg$ = construct\_cfg($m$)\;
        $defs$ = getDefsOfAt($v_t$, $s_t$, $cfg$)  \;
        \For{$d$ in $defs$}{
            $src_{var}$ = get the signature of $v_t$ in $d$\;
            $caller_{list}$ = find methods that invoke $m_t$ \;
            \For{$m$ in $caller_{list}$}{
                $src_{stmt}$ = statements that invoke $m_t$ in $m$\;
                $src_{v}$ = variables in $src_{stmt}$ that correspond to $v_t$\;
                \If{$src_{v}$  is \textit{Variable}}{
                    BackwardAnalysis($src_{v}$, $src_{stmt}$, $src_{m}$)
                } \ElseIf{$src_{v}$ is \textit{Constant}}{
                    store ($v_t$, $src_{stmt}$) in $DF$
                }
            }
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FForwar{$m$, $stmt$, $var$}}{
        $tar_{stmt}$ = find all statements that contain $stmt$ \;
        \For{$s$ in $tar_{stmt}$}{
            store ($var$, $s$) in $DF$ \;
            \If{$s$ contain invoke statements}{
                $tar_{m}$ = method that invokes $stmt$ in $s$ \;
                $tar_{v}$ = variable in $tar_{m}$ that correspond to $var$\;
                ForwardAnalysis($tar_{method}$, $s$, $tar_{v}$)
            }
        }
    }

% \vspace{-1ex}
\end{algorithm}




% 可以加个algorithm
% \input{figures/algorithm_data_flow}

% The method used for extracting the TPL data usage extraction is shown in Algorithm ~\ref{alg:data_usage}.
%methods in {\oursystem}. 
%
% With the intermediate representation (i.e., Jimple in {\soot}), we get the method body, the method's statements and target variables.
Algorithm~\ref{alg:data_usage} sketches the TPL data usage analysis method.
% 
{\oursystem} iterates over all statements in TPL to locate the target variables ({\small{$var$}}) that represent personal information listed in Tab.\ref{tab:data_type}.
%
Then, {\oursystem} conducts both inter-procedure and intra-procedure analysis to get the data flow.
%
For inter-procedures analysis, {\oursystem} backward analyzes statement {\small{$s_t$}} in method {\small{$m_t$}} with the DOI {\small{$v_t$}} (line 1).
%
The backward analysis locates the definition statements ({\small{$defs$}}) in {\small{$m_t$}} that relates to DOI {\small{$v_t$}} (line 11).
%
For statements in {\small{$defs$}}, {\oursystem} iterates {\small{$defs$}} and locates the variable signature of {\small{$v_t$}} in {\small{$d$}} (line 12-13).
%
{\oursystem} iterates FCG 
% the function call graph 
of target TPL and finds the methods ({\small{$caller_{list}$}}) that invoke {\small{$m$}} (line 14).
%
For each caller {\small{$m$}}, {\oursystem} locates the statements ({\small{$src_{stmt}$}}) in {\small{$m$}} that invoke {\small{$m_t$}}.
%
{\oursystem} finds the variable {\small{($src_v$)}} in {\small{$src_{stmt}$}} that corresponds to DOI {\small{$v_t$}} (line 17).
%
If {\small{$src_{v}$}} is a variable, {\oursystem} continues backward analysis, starts with {\small{$src_{stmt}$}} in {\small{$src_m$}} and focuses analysis on variable {\small{$src_v$}} (line 18-19); 
% otherwise, 
if {\small{$src_{v}$}} is a constant, {\oursystem} finds one piece of code that describes the data usage of {\small{$var$}} (line 21).



To locate the {\small{$v_t$}}'s data usage in {\small{$m_t$}}, {\oursystem} performs \textit{intra-method analysis}.
%
Specifically, {\oursystem} locates all statements ({\small{$uses$}}) that uses {\small{$var$}} in method {\small{$m$}} (line 5).
%
For each statement {\small{$u$}} in {\small{$uses$}}, {\oursystem} stores the usage of variable {\small{$var$}} (line 7) because the target variable have been used in the statement {\small{$u$}}.
%
Then, {\oursystem} use forward analysis (line 8) to identify whether {\small{$var$}} is used further.
%
% Specifically, {\oursystem} locates the statements ($tar_{stmt}$) that contain $stmt$ because the $stmt$ maybe invoked in some \textit{specialinvoke} statements accordingly to the prosperity of {\soot}.
%
For each statement {\small{$s$}} in {\small{$tar_{stmt}$}}, {\oursystem} stores the the data flow describing the data usage. 
% data usage.
%
If {\small{$s$}} contains invoke statements, {\oursystem} locates the method {\small{$tar_m$}} that calls {\small{$stmt$}} (line 28), builds the variable {\small{$tar_v$}} corresponding to target variable {\small{$v_t$}} and continues the forward analysis (line 30).
%





% %
% Then, we get the statements that defines $var$ in $m_{src}$ through analyzing the CFG using \textit{soot}.% API.
% % We get the definition sites for $var$ at a certain point (statement) that defines $var$ in the method.
% %
% Next, we traverse the call stack in reverse to find the the statement that initially defines target variable.
% %
% Then, we get the data flow of target variable.
% %
% For intra-procedure analysis, we iterate the statements in current method ($m_{src}$) to trace the data flow.
% %
% It worth noticing that when we find recursive invocation, we terminate the current traverse to avoid redundant analysis.



%update:25-Jan-2022:
%
%Figure out the problem that flowdroid cannot be directly used to analyze \textit{dex/jar} files.
%
%To deal with it, we write methods based on soot and soot-infoflow.
%
%Currently, we can analyze the data flow of specific methods.
%
%Demo: 
%
%\textbf{APK}: E133-3A32B-15F79-A6AA6-6CB57-FA7FC-648AC-68351-6ECDE-7399B-89999-14012-474F2.apk
%
%\textbf{Target}: location
%r
%\textbf{dataflow:}



% How to define \textbf{\textit{callback}} methods?

%%%\textbf{Questions:} When analyzing \textit{.jar} file, the \textit{infoflow} can find the target trace, e.g. the \textit{location} in aforementioned case. 
%However, when analyzing \textit{.dex}, the trace missed.
%
%Another interesting thing is: when analyzing the demo using \textit{soot} only, the results of \textit{.dex} returns more invocation results than results of \textit{.jar}.
%There could be some problems in \textit{dex2jar}.



\subsection{Identify data usage statements in TPL's privacy policy}
\label{sec:tpl_pp}

% Privacy policy analysis 
% Data usage identification is a kind of named entity recognition (NER) task in natural language processing.
%
TPL privacy policy analysis aims to identify the data usage statements.
%
% {\oursystem} analyzes TPLs' privacy policy to extract used data.
%
The pipeline of our privacy policy analysis consists of three steps: 
1) preprocessing of privacy policy,
2) named entity extraction, 
and 3) data usage action construction.
%
Finally, each privacy policy is abstracted into a set of \textbf{a}bstract \textbf{d}ata \textbf{u}sage \textbf{p}atterns (ADUP) that describes \textit{who} will (\textit{not}) \textit{access} \textit{what kinds of data} with \textit{whom}. 
%
Each ADUP is in form of {\small{\{data\_entity, action, \{data\_type\}, \{data\_recipient\}, \{neg\}\}}}.
% \{$\small{data\_entity,action,\{data\_type\},\{data\_recipient\},\{neg\}}$\}.
%
For example, \textit{``We share your personal information with our service providers," (in Adad's privacy policy)} is abstracted as {\small{\textit{\{app, share, \{personal information\}, \{service provider\}, false\}}}}.
%The extraction methods for each component of ADUP is detailed as follows.


% 1) fined-turning a state-of-the-art NER model to adapt our application scenario, 2) identifying data entities in privacy policy using pretrained model, and 3) applying expert system to identify the data usage in privacy policy.

\subsubsection{Preprocessing privacy policy}
\label{sec:pre_pp}
To download the apps' privacy policies from Google Play~\cite{googleplay},
we use the \textit{Selenium Webdriver}~\cite{gojare2015analysis} to open web pages of privacy policies.
%
Then, we use \textit{html2text}~\cite{html2text} to transform downloaded privacy policies into plain text. 
%
However, the transformed plain text contains many special characters, e.g. $*$ and $|$, which will lead to unnatural segmentation of sentences. 
%
{\oursystem} first uses patterns~\cite{stack_pre_nlp} to eliminate special characters. 
%
% Besides, enumeration items are in privacy policies to detail the related data items.
%
Besides, privacy policies use enumeration items~\cite{andow2019policylint} to detail related data items, which may lead to a whole sentence being segmented by item index and further cause losing information.
%
{\oursystem} merges the items by searching for sentences ending in a colon, and the next sentence starts with list items, such as bullets, roman numerals, and formatted numbers.
%
% Then, we use the dependency parse tree to get the constellation between words.
%


\subsubsection{Data access extraction}
%
With preprocessed privacy policy sentences, {\oursystem} analyzes each sentence to identify data access descriptions.
%
Since the interrogative sentences are commonly used in privacy policies but do not describe the types of accessed personal information, we omit them by checking the interrogative words (i.e., who, where, when, why, whether, what, and how). 
%this sentence as it would be an \textit{Introduction}, 
For example, the sentence \textit{\underline{What} personal information do we collect} is omitted. %  (appid: wp.wattpad).
%
Then, we construct the part-of-speech (POS) tagging, and dependency parsing tree (DPS) for each sentence.
%
We will omit sentences without verb words because those sentences will not claim data access behaviors.
%
For example, ``\textit{Do-Not-Track Signals and Similar Mechanisms}" in \textit{Facebook Open Source Privacy Policy} only claims the title of the paragraph.
%
For the remaining sentences, we follow the following steps to extract data action, data entity, and data actor.
% data action, data objects, data operator, and data recipient (if applicable).




%
\noindent\textbf{Identification of data action words}. 
%
We first identify whether the verb words are in the data usage word list (Tab.~\ref{tab:actionwords}).
%
We stem the word using \textit{nltk}~\cite{loper2002nltk} to deal with English verb tenses. 
%before identification 
% since English verbs have tenses. %, singular or plural forms.
%
% Besides, we will identify the verb as some statements that claim the data sharing and collection action in one sentence, for example: \textit{we \underline{collect} the information you have authorized the platform to \underline{share} with us, such as your name, email address, gender, date of birth, friend list, profile picture and playlists}(us.current.android).
%
We also identify the modifier of target verb because the privacy policies also claim the data they will not use or collect.
%
To achieve this, we analyze the dependency parsing tree and recognize the words whose relation with the target verb is `\textit{advmod}' (adverbial modifier) or `\textit{mmod}' (modal verb modifier).
%
If the words or their tags are negative (i.e., `neg'), we regard the data usage action as negative one.
%
To this end, {\oursystem} identifies
% data-related sentences and 
data sharing or collection operations.



\begin{table}[]
\centering
\smaller
\vspace{2ex}
\caption{Personal information and corresponding APIs.}
%\vspace{-1ex}
\scalebox{0.95}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.14\textwidth}@{}}
\toprule
\textbf{PI}                    & \textbf{Class Name}                                      & \textbf{Method Name}                         \\ \midrule
Ad ID                          & AdvertisingIdClient                                      & AdvertisingIdClient                          \\
\rowcolor[HTML]{EFEFEF} 
Bluetooch address              & android.bluetooth.BluetoothAdapter                       & getAddress                                   \\
Camera                         & android.hardware.Camera                                  & setPreviewDisplay                            \\
\rowcolor[HTML]{EFEFEF} 
Cell   Loca-tion                & android.telephony.TelephonyManager                       & getCellLocation                              \\
Contact                        & android.provider.ContactsContract                        & PhoneLookup                                  \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude          \\
                               & android.location.Location                                & getLongitude                                 \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLastKnownLocation \\
                               & android.location.LocationManager                         & requestLocationUpdates                       \\
\multirow{-5}{*}{GPS Location} & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLongitude         \\
Sim Number                     & android.telephony.TElephonyManager                       & getSimSerialNumber                           \\
\rowcolor[HTML]{EFEFEF} 
IMEI                           & android.telephony.TElephonyManager                       & getDeviceId                                  \\
IMSE                           & android.telephony.TElephonyManager                       & getSubscriberId                              \\
\rowcolor[HTML]{EFEFEF} 
TimeZone                       & java.util.Calendar                                       & getTimeZone                                  \\
MAC address                    & android.net.wifi.WifiInfo                                & getMacAddress                                \\
\rowcolor[HTML]{EFEFEF} 
Password                       & android.accounts.AccountManager                          & getPassword                                  \\
Phone   Number                 & android.telephony.TelephonyManager                       & getLine1Number                               \\
\rowcolor[HTML]{EFEFEF} 
SMS                            & android.telephony.SmsManager                             & sendTextMessage                              \\
SSID                           & android.net.wifi.WifiInfo                                & getSSID                                      \\
\rowcolor[HTML]{EFEFEF} 
User Credential                & android.accounts.AccountManager                          & getAccounts                                  \\
UserName                       & android.os.UserManager                                   & getUserName                                  \\ \bottomrule
\end{tabular}
}
% \vspace{-2ex}
\label{tab:pi_api}
\end{table}



% \vspace{1.5ex}
\noindent\textbf{Identification of data entity}.
%
We identify objects of identified collecting and sharing words (target verb) according to DPS.
%
{\oursystem} first merges the noun phrase (NP) tag into one noun tag according to POS tagging to simplify sentence structure. 
% because many nouns exist in sentences to describe the related data.
%
For example, consider the following sentence in the privacy policy of the app \textit{video.reface.app} ``\textit{\small{With the use of Google Analytics, we collect such data as IP-Address, your \underline{device model}, \underline{screen resolution} and \underline{operation system}, \underline{session duration}, your location}}''.
%
% {\oursystem} identifies the objects of the target verb.
%
As only one noun or noun phrase will be identified as the object of the target verb~\cite{hanlp21}, {\oursystem} locates all coordinating nouns for the object. 
%
Specifically, {\oursystem} iterates the constituency parsing tree, which is calculated by two stages conditional random field (CRF) model~\cite{zhang2021fast}, to find the sub-trees whose \textit{a) root label are common noun (NN tag) or Noun Phrase (NP)} or \textit{b) coordinating conjunction (CC tag) or punctuation exist in the sub-tree}.
% 
The condition \textit{a)} denotes that the leaves in the tree can be merged into one noun, and  \textit{b)} indicates there may exist enumeration items or coordinating nouns.
%
If we omit the relations, {\oursystem} cannot fully extract all data entities, i.e., false-positive occurs.
%
To this end, we obtain all candidate data objects in each sentence.
%


%\vspace{1.5ex}
\noindent\textbf{Identification of data actor.}
%
To identify the data actor, {\oursystem} analyzes DPT and locates the words whose relation with sharing and collection verbs is nominal subject (``\textit{nsubj}") or direct object (``\textit{dobj}").
%
% Besides, if the sentence or the object is prepositional complement or clausal complement of a preposition, we will iterate the DPT to find the coordinating verb and then locate the nominal subject of coordinating verb.
Suppose the sentence or the object is a prepositional complement or clausal complement of a preposition (``\textit{ccomp}").
%
% In that case, we will iterate 
We iterate the DPT to find the coordinating verb and then locate the nominal subject of the target verb.
%
The nominal subject and the verb will be added to the actor list and the sharing/collection verb list, respectively.
%
We also consider the data actor as users separately, under which situation the real data actor is the user rather than the supplier.
%
For example, ``\textit{we will not collect the personal information you shared with us}''.
%
The data actor should be ``you"  while the data recipient is ``us".

% Besides, for the object complementary cases, (i.e., \textit{"we will ask you to provide personal information that is necessary to provide those services to you"})

% \noindent\textbf{Data recipient identification.}
%






%\vspace{1.5ex}
\noindent\textbf{Post-process}
%
To eliminate false detection, e.g., conditional clauses, we design rules to avoid false data usage extractions.
%
For sentences that start with condition or assumption hints, such as \textit{`if'} (\textit{``if you do not provide your personal information"}), we will not identify the data usage pattern inside.
% (i.e., \textit{\{you, not provide, personal information\}}).


\begin{table}[b]
\centering
\smaller
\caption{Data sharing and collecting words.}
% \vspace{3.5ex}
%p{0.9\columnwidth}
\begin{tabular}{p{0.23\columnwidth}p{0.67\columnwidth}}
\toprule
\textbf{Action Type} & \textbf{Keywords} \\ \midrule
Collect &  access, check, collect, gather, know, obtain, receive, save, store, use \\ \hline
Sharing &  accumulate, afford, aggregate, associate,  cache,  combine, convert, connect,  deliver, disclose, distribute, disseminate, exchange,  gather, get, give, keep, lease, obtain, offer, post, possess, proxy,  provide, protect against, receive,  rent, report, request, save, seek, sell, share, send, track,  trade, transport, transfer, transmit\\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:actionwords}
\end{table}


\subsection{Extract host apps' interaction with TPLs}
\label{sec:host_app_data}

% \subsection{Data Sharing with Enumeration}
% \label{app:demo:tpl_enumeration}

To identify whether host apps' privacy policies are consistent with their TPL usage
%  with their interaction behavior with TPLs, 
{\oursystem} conducts static analysis to identify the host apps' interaction with TPLs.
%
{\oursystem} discloses what kinds of PI data (Tab.~\ref{tab:data_type}) are shared with TPLs.
%
{\oursystem} uses Flowdroid~\cite{arzt2014flowdroid} to construct FCG of apps.
%
Since Flowdroid optimizes Android app analysis process~\cite{arzt2014flowdroid}, {\oursystem} directly uses the FCG constructed from Flowdroid.
% , and performs data usage analysis(\S\ref{sec:host_app_data}) to locate 
% then iterates each statement to locate the variables related to TPLs or PI.   
% {\oursystem} does not use the methods in \S\ref{sec:tpl_data} to construct the entry points of apps because Flowdroid prepossesses apps' Manifest and resources files to identify the entry points and create the dummy main function~\cite{arzt2014flowdroid}. % that are proven to be more comprehensive and effective~\cite{arzt2014flowdroid}.
%
% Then, {\oursystem} 
%
{\oursystem} performs the data flow analysis (\S\ref{sec:tpl_data}) to find the PI related data flow.
%
To identify TPLs, {\oursystem} identifies whether the statement contains the TPLs' name or package name or not.
% 
After obtaining TPLs and PI data, we identify whether the method exists in the data flows.
%
% This is done by using FlowDroid~\cite{arzt2014flowdroid}.
%
Besides, we optimize the signature of method invocation (\textit{SMI}) using the invoking statement.
%
% For example, if the sink method ~\textit{$\langle$android.content.Intent: android.content.Intent setAction(java.lang.String)$\rangle$} is invoked in statement: (\textit{JimpleLocalBox(\$r1) in virtualinvoke \$r1.$\langle$ android.content.Intent: android.con-tent.Intent setAction( java.lang.String ) $\rangle$  
% ( "com.google.android.gms.-fitness.app\_disconnected" )} 
% % (\textsf{st1} )
% , we use the the whole invocation statement as the stored signature.
%
{\oursystem} matches the \textit{SMI} in both PIs' data flow and TPLs' data flow.
%
Once the \textit{SMI} is matched between $TPL_i$ and $PI_j$, {\oursystem} regards the host app sharing the $PI_j$ with the $TPL_i$.
%
If the \textit{SMI} only exits in $PI_j$'s data flow, {\oursystem} identify that the host app collects $PI_j$  without sharing it with TPLs.




\subsection{Identify TPLs usage statements in host apps' privacy policy}
\label{sec:host_app_pp}

To identify the TPL usage statements in host {\app}s, we extract two descriptions from the privacy policy: 
%
a) the \textit{data sharing} related statements and 
b) TPL related  descriptions.
%
The \textit{data sharing} related statements claim how the {\app} discloses users' personal information under which situations.
%
For example, the {\app} (\textit{flipboard.boxer.app}) claims that "\textit{We share personal information with vendors and service providers that help us offer and improve our service}".
% in their privacy policy.
%
The statement indicates that \textit{flipboard.boxer.app} will share users' \textit{personal information} with vendors and service providers.
%
If {\oursystem} also identifies the {\app}'s data flow sharing users' data with TPLs tagged as vendors or service providers, {\oursystem} regards the app's privacy policy as consistent with its behavior.
%
% Besides, some {\app}'s privacy policies will enumerate the TPLs they used and the data they shared with TPLs.
% (see demo in~\ref{app:demo:tpl_enumeration}). 
%
% The patterns are extracted from our manually labeled 400 privacy policies (200 for Chinese and English separately).
%
% The patterns are extracted from our manually labeled 200 privacy policies.


% First, we use methods in \S\ref{sec:pre_pp} to preprocess TPLs' privacy policy.
%
% Then, 
After preprocessing TPLs' privacy policies (\S\ref{sec:pre_pp}), we use NLP methods~\cite{hanlp21} to get the tokenization, POS tagging and DPS for each sentence.
%
For sentences with verbs, we check whether the verb is in \textit{sharing} word list (Tab.~\ref{tab:actionwords}).
%
After obtaining the data sharing verb, we identify the data recipient to determine which TPL the data are shared with.
%
Specifically, we iterate the words in the sentence.
%
If the word is the object of a preposition (\textit{pobj}) or an indirect object (\textit{iobj}) of the verb, we identify the words as candidate data recipients, i.e., TPLs.
%
For enumeration patterns, once we identify the sentence that a) starts with a noun or noun phrase (denoted as $tar_{TPL}$) that is involved in our TPL list, v) the noun ends with colon following only noun or noun phrases, we regard the noun (phrases) following colon as the shared data with $tar_{TPL}$.

%There are two types of action:
%1) "We may collect \textbf{data} from third parities."
%2) "We share \textbf{data} with third parties."


\subsection{TPL privacy compliance investigation}


{\oursystem} investigates TPL privacy compliance by performing 
\textit{normativeness analysis}, 
\textit{privacy policies legality analysis}, 
and \textit{privacy non-compliance transmissibility analysis}. 


\noindent\textbf{Normativeness analysis} identifies whether TPL provides privacy policies.
%
According to GDPR Article 12 (1)  and  Article 13 (1), TPLs, who act as the data controller or third party of personal data, should infer users about data access behaviors in a concise, transparent, intelligible and easily accessible form.
%


\noindent\textbf{Legality analysis} identifies conflicts between TPLs' behavior and privacy policy statements.
%
Specifically, {\oursystem} identifies whether TPLs' data access actions are clearly claimed in their privacy policies by combining the data flow results (\S\ref{sec:tpl_data}) and PP ADUP (\S\ref{sec:tpl_pp}).
%
If {\oursystem} identifies data usage in TPL data flow results are not mentioned in \textit{$data\_type$}s of ADUP set, the TPL will be regarded as violating legal requirements.




\noindent\textbf{Privacy non-compliance transmissibility analysis} 
\kaifa{checks to what extent the TPLs (TPL$_v$), whose privacy policies violate the regulation requirements, affect other TPLs or apps.
%
{\oursystem} summarizes artifacts that use TPL$_v$ from {\textit{Maven Repository}} to investigate the impact of TPL's privacy non-compliance.
%
Specifically, {\oursystem} crawls \textit{Usages} information in {\textit{Maven Repository}} to count the number of artifacts that use TPL$_v$.
%
}

\subsection{Regulation issue analysis}
% \subsection{Regulation conflict analysis}

Regulation conflict analysis discovers whether the usage of TPLs in host apps comply regulation requirements.
Two kinds of conflict will be identified:

% \begin{itemize}[leftmargin=*]
    % \item 
    
\noindent{$\bullet$} {\oursystem} identifies whether usage of TPLs from data flow analysis (\S\ref{sec:host_app_data}) is clearly claimed in their privacy policy statements(\S\ref{sec:host_app_pp}). 
    % To achieve this, 
    {\oursystem} investigates whether the TPL package names in data flow analysis match the \textit{$data\_entity$} or \textit{$data\_recipient$} in ADUP of host app privacy policy results.
    
    % \item 
\noindent{$\bullet$}    {\oursystem} discloses whether the host apps clearly state their data interaction with TPLs. 
    %
    % To achieve this, 
    {\oursystem} identifies whether the apps' TPL interaction behavior (\S\ref{sec:host_app_data}) is clearly stated in host apps' privacy policies (\S\ref{sec:host_app_pp}.









==> tmp/methodology_1206.tex <==

% \input{table/abbreviation_table}

% \input{table/data_type_table}

\section{Methodology}
% In this section, we will 
This section introduces how {\oursystem} identifies data usage in TPLs' code (\S\ref{sec:tpl_data}) and how to identify the consistency of TPLs' data usage with the statements in privacy policies (\S\ref{sec:tpl_pp}).
We will also describe how to determine whether host apps describe TPLs usage correctly in their privacy policy (\S\ref{sec:host_app_pp}) and whether host apps use TPLs correctly(\S\ref{sec:host_app_data}) or not.
%
Fig.~\ref{fig:sys_frame} shows the framework of {\oursystem}.
 

\begin{figure*}[ht]
   % \vspace{-2ex}
    \centering
    \includegraphics[width=0.66\textwidth]{figures/framework_win.pdf}
    % \vspace{-0.5ex}
    \caption{Framework of {\oursystem}.} 
  %  \vspace{-1.5ex}
    \label{fig:sys_frame}
\end{figure*}


\begin{table}[hb]
\centering
\smaller
\vspace{1em}
% \vspace{3.5ex}
\caption{Tracked data types in static analysis.}
\vspace{-1ex}
\begin{tabular}{p{0.9\columnwidth}}
\toprule
\textbf{Data Type} \\ \midrule
Ad ID, username, password, name, location, contact, phone number, email address, IMEI, Wi-Fi, MAC address,  GSF ID, Android ID, serial number, SIM serial number \\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:data_type}
\end{table}


\subsection{Identify personal information usage in third-party libraries}
\label{sec:tpl_data}


% This section introduces how {\oursystem} identifies personal information (PI) usage in TPL's code.
%
Given the APK files, {\oursystem} analyzes TPL's PI usages by performing static analysis based on {\soot}~\cite{soot}. % and does not require source code.
%
{\oursystem} conducts data flow analysis, specifically variable use-define analysis~\cite{defuse94}, to locate data of interest (DOI) (Tab.~\ref{tab:data_type}). 
%
{\oursystem} uses function call graphs (FCG) to trace PI flow among methods. 
%
% However, soot cannot precisely construct FCG to investigate the function invocations~\cite{arzt2014flowdroid}. 
%
However, our analysis discovers that the soot cannot effectively discover the TPL's main functions and entry points to construct a valid FCG~\cite{arzt2014flowdroid}.
%
Thus, we propose the following methods to optimize the FCG construction process and improve the precision of the data flow analysis.


\begin{table}[]
\centering
\smaller
% \vspace{1ex}
\caption{Personal information and corresponding APIs.}
%\vspace{-1ex}
\scalebox{0.95}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.14\textwidth}@{}}
\toprule
\textbf{PI}                    & \textbf{Class Name}                                      & \textbf{Method Name}                         \\ \midrule
Ad ID                          & AdvertisingIdClient                                      & AdvertisingIdClient                          \\
\rowcolor[HTML]{EFEFEF} 
Bluetooch address              & android.bluetooth.BluetoothAdapter                       & getAddress                                   \\
Camera                         & android.hardware.Camera                                  & setPreviewDisplay                            \\
\rowcolor[HTML]{EFEFEF} 
Cell   Loca-tion                & android.telephony.TelephonyManager                       & getCellLocation                              \\
Contact                        & android.provider.ContactsContract                        & PhoneLookup                                  \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude          \\
                               & android.location.Location                                & getLongitude                                 \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLastKnownLocation \\
                               & android.location.LocationManager                         & requestLocationUpdates                       \\
\multirow{-5}{*}{GPS Location} & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLongitude         \\
Sim Number                     & android.telephony.TElephonyManager                       & getSimSerialNumber                           \\
\rowcolor[HTML]{EFEFEF} 
IMEI                           & android.telephony.TElephonyManager                       & getDeviceId                                  \\
IMSE                           & android.telephony.TElephonyManager                       & getSubscriberId                              \\
\rowcolor[HTML]{EFEFEF} 
TimeZone                       & java.util.Calendar                                       & getTimeZone                                  \\
MAC address                    & android.net.wifi.WifiInfo                                & getMacAddress                                \\
\rowcolor[HTML]{EFEFEF} 
Password                       & android.accounts.AccountManager                          & getPassword                                  \\
Phone   Number                 & android.telephony.TelephonyManager                       & getLine1Number                               \\
\rowcolor[HTML]{EFEFEF} 
SMS                            & android.telephony.SmsManager                             & sendTextMessage                              \\
SSID                           & android.net.wifi.WifiInfo                                & getSSID                                      \\
\rowcolor[HTML]{EFEFEF} 
User Credential                & android.accounts.AccountManager                          & getAccounts                                  \\
UserName                       & android.os.UserManager                                   & getUserName                                  \\ \bottomrule
\end{tabular}
}
\vspace{-2ex}
\label{tab:pi_api}
\end{table}



\begin{comment}

% Intuitively, each method in TPLs can be invoked and further used by the host apps to use the TPL's functionalities.
%
% Thus, when we use static analysis to analyze data flow in TPLs, it is hard to find and determine natural entry points to start the analysis.
%
% To counter the challenges, our solutions are given as follows

 
% There are two challenges in analyzing TPLs.
% %
% \textbf{C1.} TPLs generally can not run independently without host apps that limit the application of dynamic analysis.% for analyzing TPLs.
% % 
% To counter this challenge, {\oursystem} applies static analysis to identify data usage in TPLs.
% %
% \textbf{C2.} No explicitly entry points or main function for TPLs to start analysis.
% %
\end{comment}



% \input{table/PI_related_API_list}


\begin{comment}

% {\oursystem} conducts data flow analysis based on top of {\soot}~\cite{lam2011soot} as {\soot} is widely used for java code analysis and does not require the source code.
% %
% In this way, {\oursystem} is capable of analyzing TPLs in form of \textit{jar} or \textit{aar} files that are publicly available for usage in \textit{mvnrepository}~\cite{mvnrepository}.
% %
% However, when analyzing the data flow in TPLs, we still require entry points to start our analysis.
%
\end{comment}








\noindent\textbf{TPL FCG construction: }
%
{\oursystem} first 
% uses {\soot} to get the intermediate representation (IR) of a TPL and 
iterates over each class and method.
%
{\oursystem} identifies the methods that a) are not concrete~\cite{soot}, b) possess active method bodies and c) are \textit{publicly} accessible.
%
{\oursystem} extends the identified methods to entry points set to optimize  
% the initialization of 
FCG construction.
% process.
%


\noindent\textbf{TPL DOI identification: }
%
% {\oursystem} focuses on personal information (PI) listed in Tab.~\ref{tab:data_type} to locate variables.
% %
% Based on PI names, we extract related Android APIs~\cite{androidDeveloper} (Tab.~\ref{tab:pi_api}) to improve variable locating precision.
% %
% Because if we only use string matching with data type names, many false-positive statements will be located~\cite{yu2016can}.
%
We first summarize personal information (PI) from regulations~\cite{gdpr,ccpa,zhSDKLaw,piss} as listed in Tab.~\ref{tab:data_type}.
%
Then, we manually crawl PI-related APIs~\cite{androidDeveloper}.
%
Based on those APIs, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
{\oursystem} analyzes the data flow inter- and intra-methods to identify all PI-related statements.
%
% For example, if we want to locate data flows that collect \textit{sim} information, we may locate
% the statements as
% \textit{``virtualinvoke \$r1.$\langle$android.os.Bundle: void putSerializable( java.lang.String, java.io.Serializable )$\rangle$( "fractionProgres\underline{sIm}pressions-Sent", \$r2 )"} that is not related to personal information.
%
% Then, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
% Finally, {\oursystem} performs forward analysis and backward analysis~\cite{arzt2014flowdroid, zhou2021finding} to trace the inter-methods and intra-methods data usage.

\begin{algorithm}[t]
% \vspace{-2ex}
\caption{Data usage analysis}\label{alg:data_flow}
\label{alg:data_usage}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  
  \KwInput{method $m_t$, statement $s_t$, variable $v_t$}
  \KwOutput{data usage $FD$ of variable $v_t$}
  
 

% Set Function Names
    \SetKwFunction{FInterMVA}{InterMethodVarAnalysis}
    \SetKwFunction{FIntraMVA}{IntraMethodVarAnalysis}
    \SetKwFunction{FForwar}{ForwardAnalysis}
    \SetKwFunction{FBackwar}{BackwardAnalysis}
  
    % BackwardAnalysis($src_{var}$, $src_{stmt}$, $src_{m}$)\;
    BackwardAnalysis($m_t$, $s_t$, $v_t$)\;

    IntraMethodVarAnalysis($m_t$, $s_t$, $v_t$) \;
    % \vspace{-1.1ex}\;\vspace{-1.1ex}
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FIntraMVA{$m$, $stmt$, $var$}}{
        $uses$ = find statements that use $var$ in method $m$ \;
        \For{$u$ in $uses$}{
            store($var$, u) in $DF$ \;
            ForwardAnalysis($m$, $u$, $var$)
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    \SetKwProg{Fn}{Def}{:}{\KwRet}
    \Fn{\FBackwar{$m_t$, $s_t$, $v_t$}}{
        % InterProcedureVariableAnalysis($m$, $stmt$, $var$)  \;
        % $cfg$ = construct\_cfg($m$)\;
        $defs$ = getDefsOfAt($v_t$, $s_t$, $cfg$)  \;
        \For{$d$ in $defs$}{
            $src_{var}$ = get the signature of $v_t$ in $d$\;
            $caller_{list}$ = find methods that invoke $m_t$ \;
            \For{$m$ in $caller_{list}$}{
                $src_{stmt}$ = statements that invoke $m_t$ in $m$\;
                $src_{v}$ = variables in $src_{stmt}$ that correspond to $v_t$\;
                \If{$src_{v}$  is \textit{Variable}}{
                    BackwardAnalysis($src_{v}$, $src_{stmt}$, $src_{m}$)
                } \ElseIf{$src_{v}$ is \textit{Constant}}{
                    store ($v_t$, $src_{stmt}$) in $DF$
                }
            }
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FForwar{$m$, $stmt$, $var$}}{
        $tar_{stmt}$ = find all statements that contain $stmt$ \;
        \For{$s$ in $tar_{stmt}$}{
            store ($var$, $s$) in $DF$ \;
            \If{$s$ contain invoke statements}{
                $tar_{m}$ = method that invokes $stmt$ in $s$ \;
                $tar_{v}$ = variable in $tar_{m}$ that correspond to $var$\;
                ForwardAnalysis($tar_{method}$, $s$, $tar_{v}$)
            }
        }
    }

% \vspace{-1ex}
\end{algorithm}




% 可以加个algorithm
% \input{figures/algorithm_data_flow}

% The method used for extracting the TPL data usage extraction is shown in Algorithm ~\ref{alg:data_usage}.
%methods in {\oursystem}. 
%
% With the intermediate representation (i.e., Jimple in {\soot}), we get the method body, the method's statements and target variables.
Algorithm~\ref{alg:data_usage} sketches the TPL data usage analysis method.
% 
{\oursystem} iterates over all statements in TPL to locate the target variables ({\small{$var$}}) that represent personal information listed in Tab.~\ref{tab:data_type}.
%
Then, {\oursystem} conducts both inter-methods and intra-methods analyses to get the data flow.
%
For inter-methods analysis, {\oursystem} backward analyzes statement {\small{$s_t$}} in method {\small{$m_t$}} with the DOI {\small{$v_t$}} (line 1).
%
% construct the control flow graph (CFG) of current methods ($m_{src}$) using soot.
% Specifically, for backward analysis, {\oursystem}
The backward analysis locates the definition statements ({\small{$defs$}}) in {\small{$m_t$}} that relates to DOI {\small{$v_t$}} (line 11).
%
For statements in {\small{$defs$}}, {\oursystem} iterates {\small{$defs$}} and locates the variable signature of {\small{$v_t$}} in {\small{$d$}} (line 12-13).
%
{\oursystem} iterates the function call graph of TPL and finds the methods ({\small{$caller_{list}$}}) that invoke {\small{$m$}} (line 14).
%
For each caller {\small{$m$}}, {\oursystem} locates the statements ({\small{$src_{stmt}$}}) in {\small{$m$}} that invoke {\small{$m_t$}}.
%
{\oursystem} finds the variable {\small{($src_v$)}} in {\small{$src_{stmt}$}} that corresponds to DOI {\small{$v_t$}} (line 17).
%
If {\small{$src_{v}$}} is a variable, {\oursystem} continues backward analysis, starts with {\small{$src_{stmt}$}} in {\small{$src_m$}} and focuses analysis on variable {\small{$src_v$}} (line 18-19); 
% otherwise, 
if {\small{$src_{v}$}} is a constant, {\oursystem} finds one piece of code that describes the data usage of {\small{$var$}} (line 21).



To locate the {\small{$v_t$}}'s data usage in {\small{$m_t$}}, {\oursystem} performs \textit{intra-methods variable analysis}.
%
Specifically, {\oursystem} locates all statements ({\small{$uses$}}) that uses {\small{$var$}} in method {\small{$m$}} (line 5).
%
For each statement {\small{$u$}} in {\small{$uses$}}, {\oursystem} stores the usage of variable {\small{$var$}} (line 7) because the target variable have been used in the statement {\small{$u$}}.
%
Then, {\oursystem} use forward analysis (line 8) to identify whether {\small{$var$}} is used further.
%
% Specifically, {\oursystem} locates the statements ($tar_{stmt}$) that contain $stmt$ because the $stmt$ maybe invoked in some \textit{specialinvoke} statements accordingly to the prosperity of {\soot}.
%
For each statement {\small{$s$}} in {\small{$tar_{stmt}$}}, {\oursystem} stores the the data flow describing the data usage. 
% data usage.
%
If {\small{$s$}} contains invoke statements, {\oursystem} locates the method {\small{$tar_m$}} that calls {\small{$stmt$}} (line 28), builds the variable {\small{$tar_v$}} corresponding to target variable {\small{$v_t$}} and continues the forward analysis (line 30).
%





% %
% Then, we get the statements that defines $var$ in $m_{src}$ through analyzing the CFG using \textit{soot}.% API.
% % We get the definition sites for $var$ at a certain point (statement) that defines $var$ in the method.
% %
% Next, we traverse the call stack in reverse to find the the statement that initially defines target variable.
% %
% Then, we get the data flow of target variable.
% %
% For intra-procedure analysis, we iterate the statements in current method ($m_{src}$) to trace the data flow.
% %
% It worth noticing that when we find recursive invocation, we terminate the current traverse to avoid redundant analysis.



%update:25-Jan-2022:
%
%Figure out the problem that flowdroid cannot be directly used to analyze \textit{dex/jar} files.
%
%To deal with it, we write methods based on soot and soot-infoflow.
%
%Currently, we can analyze the data flow of specific methods.
%
%Demo: 
%
%\textbf{APK}: E133-3A32B-15F79-A6AA6-6CB57-FA7FC-648AC-68351-6ECDE-7399B-89999-14012-474F2.apk
%
%\textbf{Target}: location
%r
%\textbf{dataflow:}



% How to define \textbf{\textit{callback}} methods?

%%%\textbf{Questions:} When analyzing \textit{.jar} file, the \textit{infoflow} can find the target trace, e.g. the \textit{location} in aforementioned case. 
%However, when analyzing \textit{.dex}, the trace missed.
%
%Another interesting thing is: when analyzing the demo using \textit{soot} only, the results of \textit{.dex} returns more invocation results than results of \textit{.jar}.
%There could be some problems in \textit{dex2jar}.



\vspace{-1ex}
\subsection{Identify data usage statements in TPL's privacy policy}
\label{sec:tpl_pp}
\vspace{-1ex}
% Privacy policy analysis 
% Data usage identification is a kind of named entity recognition (NER) task in natural language processing.
%
TPL privacy policy analysis aims aims to identify the documents' data usage statements.
%
% {\oursystem} analyzes TPLs' privacy policy to extract used data.
%
The pipeline of our privacy policy analysis consists of three steps: 
1) preprocessing of privacy policy,
2) named entity extraction, 
and 3) data usage action construction.
%
Finally, each privacy policy is abstracted into a set of abstract data usage patterns (ADUP) that describe \textit{who} will (\textit{not}) \textit{access} \textit{what kinds of data} with \textit{whom}. 
%
Each ADUP is in form of {\small{\{data\_entity, action, \{data\_type\}, \{data\_recipient\}, \{neg\}\}}}.
% \{$\small{data\_entity,action,\{data\_type\},\{data\_recipient\},\{neg\}}$\}.
%
For example, \textit{``We share your personal information with our service providers," (in Adad's privacy policy)} is abstracted as {\small{\textit{\{app, share, \{personal information\}, \{service provider\}, false\}}}}.
%The extraction methods for each component of ADUP is detailed as follows.


% 1) fined-turning a state-of-the-art NER model to adapt our application scenario, 2) identifying data entities in privacy policy using pretrained model, and 3) applying expert system to identify the data usage in privacy policy.

\subsubsection{Preprocessing privacy policy}
\label{sec:pre_pp}
To download the apps' privacy policies from Google Play~\cite{googleplay},
we use the \textit{Selenium Webdriver}~\cite{gojare2015analysis} to open web pages of privacy policies.
%
Then, we use \textit{html2text}~\cite{html2text} to transform downloaded privacy policies into plain text. 
%
However, the transformed plain text contains many special characters, e.g. $*$ and $|$, which will lead to unnatural segmentation of sentences. 
%
{\oursystem} first uses patterns~\cite{stack_pre_nlp} to eliminate special characters. 
%
% Besides, enumeration items are in privacy policies to detail the related data items.
%
Besides, privacy policies use enumeration items~\cite{andow2019policylint} to detail related data items, which may lead to a whole sentence being segmented by item index and further cause losing information.
%
{\oursystem} merges the items by searching for sentences ending in a colon, and the next sentence starts with list items, such as bullets, roman numerals, and formatted numbers.
%
% Then, we use the dependency parse tree to get the constellation between words.
%


\subsubsection{Data access extraction}
%
With preprocessed privacy policy sentences, {\oursystem} analyzes each sentence to identify data access descriptions.
%
Since the interrogative sentences are commonly used in privacy policies but do not describe the types of accessed personal information, we omit them by checking the interrogative words (i.e., who, where, when, why, whether, what, and how). 
%this sentence as it would be an \textit{Introduction}, 
For example, the sentence \textit{\underline{What} personal information do we collect} is omitted. %  (appid: wp.wattpad).
%
Then, we construct the part-of-speech (POS) tagging, and dependency parsing tree (DPS) for each sentence.
%
We will omit sentences without verb words because those sentences will not claim data access behaviors.
%
For example, ``\textit{Do-Not-Track Signals and Similar Mechanisms}" in \textit{Facebook Open Source Privacy Policy} only claims the title of the paragraph.
%
For the remaining sentences, we follow the following steps to extract data action, data entity, and data actor.
% data action, data objects, data operator, and data recipient (if applicable).




%
\noindent\textbf{Identification of data action words}. 
%
We first identify whether the verb words are in the data usage word list (Tab.~\ref{tab:actionwords}).
%
We stem the word using \textit{nltk}~\cite{loper2002nltk} to deal with English verb tenses. 
%before identification 
% since English verbs have tenses. %, singular or plural forms.
%
% Besides, we will identify the verb as some statements that claim the data sharing and collection action in one sentence, for example: \textit{we \underline{collect} the information you have authorized the platform to \underline{share} with us, such as your name, email address, gender, date of birth, friend list, profile picture and playlists}(us.current.android).
%
We also identify the modifier of target verb because the privacy policies also claim the data they will not use or collect.
%
To achieve this, we analyze the dependency parsing tree and recognize the words whose relation with the target verb is `\textit{advmod}' (adverbial modifier) or `\textit{mmod}' (modal verb modifier).
%
If the words or their tags are negative (i.e., `neg'), we regard the data usage action as negative one.
%
To this end, {\oursystem} identifies
% data-related sentences and 
data sharing or collection operations.


% \vspace{1.5ex}
\noindent\textbf{Identification of data entity}.
%
We identify objects of identified collecting and sharing words (target verb) according to DPS.
%
{\oursystem} first merges the noun phrase (NP) tag into one noun tag according to POS tagging to simplify sentence structure. 
% because many nouns exist in sentences to describe the related data.
%
For example, consider the following sentence in the privacy policy of the app \textit{video.reface.app} ``\textit{\small{With the use of Google Analytics, we collect such data as IP-Address, your \underline{device model}, \underline{screen resolution} and \underline{operation system}, \underline{session duration}, your location}}''.
%
% {\oursystem} identifies the objects of the target verb.
%
As only one noun or noun phrase will be identified as the object of the target verb~\cite{hanlp21}, {\oursystem} locates all coordinating nouns for the object. 
%
Specifically, {\oursystem} iterates the constituency parsing tree, which is calculated by two stages conditional random field (CRF) model~\cite{zhang2021fast}, to find the sub-trees whose \textit{a) root label are common noun (NN tag) or Noun Phrase (NP)} or \textit{b) coordinating conjunction (CC tag) or punctuation exist in the sub-tree}.
% 
The condition \textit{a)} denotes that the leaves in the tree can be merged into one noun, and  \textit{b)} indicates there may exist enumeration items or coordinating nouns.
%
If we omit the relations, {\oursystem} cannot fully extract all data entities, i.e., false-positive occurs.
%
To this end, we obtain all candidate data objects in each sentence.
%


%\vspace{1.5ex}
\noindent\textbf{Identification of data actor.}
%
To identify the data actor, {\oursystem} analyzes DPT and locates the words whose relation with sharing and collection verbs is nominal subject (``\textit{nsubj}") or direct object (``\textit{dobj}").
%
% Besides, if the sentence or the object is prepositional complement or clausal complement of a preposition, we will iterate the DPT to find the coordinating verb and then locate the nominal subject of coordinating verb.
Suppose the sentence or the object is a prepositional complement or clausal complement of a preposition (``\textit{ccomp}").
%
% In that case, we will iterate 
We iterate the DPT to find the coordinating verb and then locate the nominal subject of the target verb.
%
The nominal subject and the verb will be added to the actor list and the sharing/collection verb list, respectively.
%
We also consider the data actor as users separately, under which situation the real data actor is the user rather than the supplier.
%
For example, ``\textit{we will not collect the personal information you shared with us}''.
%
The data actor should be ``you"  while the data recipient is ``us".

% Besides, for the object complementary cases, (i.e., \textit{"we will ask you to provide personal information that is necessary to provide those services to you"})

% \noindent\textbf{Data recipient identification.}
%






%\vspace{1.5ex}
\noindent\textbf{Post-process}
%
To eliminate false detection, e.g., conditional clauses, we design rules to avoid false data usage extractions.
%
For sentences that start with condition or assumption hints, such as \textit{`if'} (\textit{``if you do not provide your personal information"}), we will not identify the data usage pattern inside.
% (i.e., \textit{\{you, not provide, personal information\}}).


\begin{table}[]
\centering

\vspace{2ex}

\smaller
\caption{Data sharing and collecting words.}
% \vspace{3.5ex}
%p{0.9\columnwidth}
\begin{tabular}{p{0.23\columnwidth}p{0.67\columnwidth}}
\toprule
\textbf{Action Type} & \textbf{Keywords} \\ \midrule
Collect &  access, check, collect, gather, know, obtain, receive, save, store, use \\ \hline
Sharing &  accumulate, afford, aggregate, associate,  cache,  combine, convert, connect,  deliver, disclose, distribute, disseminate, exchange,  gather, get, give, keep, lease, obtain, offer, post, possess, proxy,  provide, protect against, receive,  rent, report, request, save, seek, sell, share, send, track,  trade, transport, transfer, transmit\\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:actionwords}
\end{table}


\subsection{Extract host apps' interaction with TPLs}
\label{sec:host_app_data}

% \subsection{Data Sharing with Enumeration}
% \label{app:demo:tpl_enumeration}

To identify whether host apps' privacy policies are consistent with their TPL usage
%  with their interaction behavior with TPLs, 
{\oursystem} conducts static analysis to identify the host apps' interaction with TPLs.
%
{\oursystem} discloses what kinds of PI data (Tab.~\ref{tab:data_type}) are shared with TPLs.
%
{\oursystem} uses Flowdroid~\cite{arzt2014flowdroid} to construct FCG of apps.
%
Since Flowdroid optimizes Android app analysis process~\cite{arzt2014flowdroid}, {\oursystem} directly uses the FCG constructed from Flowdroid, and then iterates each statement to locate the variables related to TPLs or PI.   
% {\oursystem} does not use the methods in \S\ref{sec:tpl_data} to construct the entry points of apps because Flowdroid prepossesses apps' Manifest and resources files to identify the entry points and create the dummy main function~\cite{arzt2014flowdroid}. % that are proven to be more comprehensive and effective~\cite{arzt2014flowdroid}.
%
% Then, {\oursystem} 
%
{\oursystem} performs the data flow analysis (\S\ref{sec:tpl_data}) to find the PI related data flow.
%
To identify TPLs, {\oursystem} identifies whether the statement contains the TPLs' name or package name or not.
%
After obtaining TPLs and PI data, we identify whether the sinks exist in the data flows.
%
% This is done by using FlowDroid~\cite{arzt2014flowdroid}.
%
Besides, we optimize the signature of sink invocation (\textit{SSI}) using the invoke statement.
%
% For example, if the sink method ~\textit{$\langle$android.content.Intent: android.content.Intent setAction(java.lang.String)$\rangle$} is invoked in statement: (\textit{JimpleLocalBox(\$r1) in virtualinvoke \$r1.$\langle$ android.content.Intent: android.con-tent.Intent setAction( java.lang.String ) $\rangle$  
% ( "com.google.android.gms.-fitness.app\_disconnected" )} 
% % (\textsf{st1} )
% , we use the the whole invocation statement as the stored signature.
%
{\oursystem} matches the \textit{SSI} in both PIs' data flow and TPLs' data flow.
%
Once the \textit{SSI} is matched between $TPL_i$ and $PI_j$, {\oursystem} regards the host app sharing the $PI_j$ with the $TPL_i$.
%
If the \textit{SSI} only exits in $PI_j$'s data flow, {\oursystem} identify that the host app collects $PI_j$  without sharing it with TPLs.




\subsection{Identify TPLs usage statements in host apps' privacy policy}
\label{sec:host_app_pp}

To identify the TPL usage statements in host {\app}s, we extract two descriptions from the privacy policy: 
%
a) the \textit{data sharing} related statements and 
b) TPL related  descriptions.
%
The \textit{data sharing} related statements claim how the {\app} discloses users' personal information under which situations.
%
For example, the {\app} (\textit{flipboard.boxer.app}) claims that "\textit{We share personal information with vendors and service providers that help us offer and improve our service}".
% in their privacy policy.
%
The statement indicates that \textit{flipboard.boxer.app} will share users' \textit{personal information} with vendors and service providers.
%
If {\oursystem} also identifies the {\app}'s data flow sharing users' data with TPLs tagged as vendors or service providers, {\oursystem} regards the app's privacy policy as consistent with its behavior.
%
% Besides, some {\app}'s privacy policies will enumerate the TPLs they used and the data they shared with TPLs.
% (see demo in~\ref{app:demo:tpl_enumeration}). 
%
% The patterns are extracted from our manually labeled 400 privacy policies (200 for Chinese and English separately).
%
% The patterns are extracted from our manually labeled 200 privacy policies.


% First, we use methods in \S\ref{sec:pre_pp} to preprocess TPLs' privacy policy.
%
% Then, 
After preprocessing TPLs' privacy policies (\S\ref{sec:pre_pp}), we use NLP methods~\cite{hanlp21} to get the tokenization, POS tagging and DPS for each sentence.
%
For sentences with verbs, we check whether the verb is in \textit{sharing} word list (Tab.~\ref{tab:actionwords}).
%
After obtaining the data sharing verb, we identify the data recipient to determine which TPL the data are shared with.
%
Specifically, we iterate the words in the sentence.
%
If the word is the object of a preposition (\textit{pobj}) or an indirect object (\textit{iobj}) of the verb, we identify the words as candidate data recipients, i.e., TPLs.
%
For enumeration patterns, once we identify the sentence that a) starts with a noun or noun phrase (denoted as $tar_{TPL}$) that is involved in our TPL list, v) the noun ends with colon following only noun or noun phrases, we regard the noun (phrases) following colon as the shared data with $tar_{TPL}$.

%There are two types of action:
%1) "We may collect \textbf{data} from third parities."
%2) "We share \textbf{data} with third parties."


\subsection{TPL vulnerability investigation}


{\oursystem} investigates TPL vulnerabilities by performing
 normativeness analysis, 
 privacy policies legality analysis, 
and vulnerability transmissibility analysis. 


\noindent\textbf{Normativeness analysis} identifies whether TPL provides privacy policies.
%
According to GDPR Article 12 (1)  and  Article 13 (1), TPLs, who act as the data controller or third party of personal data, should infer users about data access behaviors in a concise, transparent, intelligible and easily accessible form.
%


\noindent\textbf{Legality analysis} identifies conflicts between TPLs' behavior and privacy policy statements.
%
Specifically, {\oursystem} identifies whether TPLs' data access actions are clearly claimed in their privacy policies by combining the data flow results (\S\ref{sec:tpl_data}) and PP ADUP (\S\ref{sec:tpl_pp}).
%
If {\oursystem} identifies data usage in TPL data flow results are not mentioned in \textit{$data\_type$}s of ADUP set, the TPL will be regarded as violating legal requirements.


% \xiancm{how do you conduct this step, this step is very difficult, super challenging, how denote the vulnerable version, and which version is used by other apps or TPLs, which means you have conduct an Android SCA tool? did you}


\noindent\textbf{Privacy leakage transmissibility analysis} 
\kaifa{checks to what extent the vulnerable TPLs, which potentially leak user privacy, will affect other TPLs or apps.
%
{\oursystem} summarizes artifacts that use vulnerable TPLs from {\textit{Maven Repository}} to investigate the impact of TPL's privacy leakage.
%
Specifically, {\oursystem} crawls \textit{Usages} information in {\textit{Maven Repository}} to count the number of artifacts that use vulnerable TPLs.
%
% The more artifacts using vulnerable TPLs, the more effect of TPLs' vulnerability. 
}

\begin{comment}

\noindent\textbf{Vulnerability transmissibility analysis} checks to what extent the TPLs with vulnerabilities will affect other TPLs or apps.
%
{\oursystem} adds up artifacts that use vulnerable TPLs from {\textit{Maven Repository}}.
%
The more artifacts using vulnerable TPLs, the more effect of TPLs' vulnerability. 
% \xiancm{incorrect.... not accurate}

\end{comment}

\subsection{Regulation conflict analysis}

Regulation conflict analysis discovers whether the usage of TPLs in host apps comply regulation requirements.
Two kinds of conflict will be identified:

% \begin{itemize}[leftmargin=*]
    % \item 
    
\noindent{$\bullet$} {\oursystem} identifies whether usage of TPLs from data flow analysis (\S\ref{sec:host_app_data}) is clearly claimed in their privacy policy statements(\S\ref{sec:host_app_pp}. 
    % To achieve this, 
    {\oursystem} investigates whether the TPL package names in data flow analysis match the \textit{$data\_entity$} or \textit{$data\_recipient$} in ADUP of host app privacy policy results.
    
    % \item 
\noindent{$\bullet$}    {\oursystem} discloses whether the host apps clearly state their data interaction with TPLs. 
    %
    % To achieve this, 
    {\oursystem} matches whether the apps' TPL interaction behavior (\S\ref{sec:host_app_data}) is clearly stated in host apps' privacy policies (\S\ref{sec:host_app_pp}.
    % {\oursystem} matches the host apps interaction behaviors results (\S\ref{sec:host_app_data} and host apps' privacy policies analysis results (\S\ref{sec:host_app_pp}).
    % For host apps that disclose their interaction with TPLs, {\oursystem} also identifies whether the data usage of TPLs, that is achieved from data flow analysis of TPLs (\S\ref{sec:tpl_data}), are clearly and comprehensively disclosed in host apps privacy policies.
% \end{itemize}



% \subsection{Extract data usage in host {app}'s privacy policy}

% In this subsection, I wil; introduce how to analyze the data usage of TPL through analyze the TPL bytecode.

% We should target specific sensitive data, in this way we can identify the DataFlow of TPL:

% Email, userid, username, password, contact, gps, location, device ID, identifier, advertising ID, account/imei address, PHOTOGRAPHY


% To identify the TPL usage in our 




\begin{comment}


\subsubsection{Demo}

package name = \textbf{``com.facebook.ads"}

    

    

%\begin{itemize}
%    \item \textbf{email}  
    % SPECIAL edge: specialinvoke \$r15.$\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$( \kaifa{"EMAIL"}, 15, "email" ) in $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$() $\rangle$ ==$\rangle$ $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$
    
%    \item \textbf{userid} 
    % VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\kaifa{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$
    
%    \item \textbf{deviceid} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$(``Stub!") in $\langle$android.view.InputDevice: int[] \kaifa{getDeviceIds()} $\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$

 %   \item \textbf{identifier} 
    % VIRTUAL edge: \$r3 = virtualinvoke r1.$\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$() in $\langle$com.facebook.ads.internal.bridge.gms.AdvertisingId: com.facebook.ads.internal.bridge.gms.AdvertisingId getAdvertisingIdInfoDirectly(android.content.Context)$\rangle$ ==$\rangle$ $\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$
    
%    \item \textbf{account} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$(``Stub!") in $\langle$android.content.ContentResolver: boolean isSyncPending(android.accounts.Account,java.lang.String)$\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$


    
%    \item \textbf{photo}: 
    % SPECIAL edge: specialinvoke \$r38.$\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$(\kaifa{"PHOTOGRAPHY"}, 38, "photography") in $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$()$\rangle$ ==$\rangle$ $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$
    
%\end{itemize}



% For data that android system provides API to collect, such as location, we identify the invocation of those methods. \kaifa{to list the related API in appendix}
% %
% For other data, such as gender or username, we identify the parameters passed to target server.
% %
%such as:  \textit{VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\textbf{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$}

\end{comment}











==> tmp/methodology_221206.tex <==

% \input{table/abbreviation_table}

% \input{table/data_type_table}

\section{Methodology}
% In this section, we will 
This section introduces how {\oursystem} identifies data usage in TPLs' code (\S\ref{sec:tpl_data}) and how to identify the consistency of TPLs' data usage with the statements in privacy policies (\S\ref{sec:tpl_pp}).
We will also describe how to determine whether host apps describe TPLs usage correctly in their privacy policy (\S\ref{sec:host_app_pp}) and whether host apps use TPLs correctly(\S\ref{sec:host_app_data}) or not.
%
Fig.~\ref{fig:sys_frame} shows the framework of {\oursystem}.
 

\begin{figure*}[ht]
   % \vspace{-2ex}
    \centering
    \includegraphics[width=0.66\textwidth]{figures/framework_win.pdf}
    % \vspace{-0.5ex}
    \caption{Framework of {\oursystem}.} 
  %  \vspace{-1.5ex}
    \label{fig:sys_frame}
\end{figure*}


\begin{table}[hb]
\centering
\smaller
\vspace{1em}
% \vspace{3.5ex}
\caption{Tracked data types in static analysis.}
\vspace{-1ex}
\begin{tabular}{p{0.9\columnwidth}}
\toprule
\textbf{Data Type} \\ \midrule
Ad ID, username, password, name, location, contact, phone number, email address, IMEI, Wi-Fi, MAC address,  GSF ID, Android ID, serial number, SIM serial number \\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:data_type}
\end{table}


\subsection{Identify personal information usage in third-party libraries}
\label{sec:tpl_data}


% This section introduces how {\oursystem} identifies personal information (PI) usage in TPL's code.
%
Given the APK files, {\oursystem} analyzes TPL's PI usages by performing static analysis based on {\soot}~\cite{soot}. % and does not require source code.
%
{\oursystem} conducts data flow analysis, specifically variable use-define analysis~\cite{defuse94}, to locate data of interest (DOI) (Tab.~\ref{tab:data_type}). 
%
{\oursystem} uses function call graphs (FCG) to trace PI flow among methods. 
%
% However, soot cannot precisely construct FCG to investigate the function invocations~\cite{arzt2014flowdroid}. 
%
However, our analysis discovers that the soot cannot effectively discover the TPL's main functions and entry points to construct a valid FCG~\cite{arzt2014flowdroid}.
%
Thus, we propose the following methods to optimize the FCG construction process and improve the precision of the data flow analysis.






\noindent\textbf{TPL FCG construction: }
%
{\oursystem} first 
% uses {\soot} to get the intermediate representation (IR) of a TPL and 
iterates over each class and method.
%
{\oursystem} identifies the methods that a) are not concrete~\cite{soot}, b) possess active method bodies and c) are \textit{publicly} accessible.
%
{\oursystem} extends the identified methods to entry points set to optimize  
% the initialization of 
FCG construction.
% process.
%


\noindent\textbf{TPL DOI identification: }
%
% {\oursystem} focuses on personal information (PI) listed in Tab.~\ref{tab:data_type} to locate variables.
% %
% Based on PI names, we extract related Android APIs~\cite{androidDeveloper} (Tab.~\ref{tab:pi_api}) to improve variable locating precision.
% %
% Because if we only use string matching with data type names, many false-positive statements will be located~\cite{yu2016can}.
%
We first summarize personal information (PI) from regulations~\cite{gdpr,ccpa,zhSDKLaw,piss} as listed in Tab.~\ref{tab:data_type}.
%
Then, we manually crawl PI-related APIs~\cite{androidDeveloper}.
%
Based on those APIs, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
{\oursystem} analyzes the data flow inter- and intra-methods to identify all PI-related statements.
%
% For example, if we want to locate data flows that collect \textit{sim} information, we may locate
% the statements as
% \textit{``virtualinvoke \$r1.$\langle$android.os.Bundle: void putSerializable( java.lang.String, java.io.Serializable )$\rangle$( "fractionProgres\underline{sIm}pressions-Sent", \$r2 )"} that is not related to personal information.
%
% Then, {\oursystem} iterates over all statements and locates DOI with target variables. 
%
% Finally, {\oursystem} performs forward analysis and backward analysis~\cite{arzt2014flowdroid, zhou2021finding} to trace the inter-methods and intra-methods data usage.

\begin{algorithm}[t]
% \vspace{-2ex}
\caption{Data usage analysis}\label{alg:data_flow}
\label{alg:data_usage}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  
  \KwInput{method $m_t$, statement $s_t$, variable $v_t$}
  \KwOutput{data usage $FD$ of variable $v_t$}
  
 

% Set Function Names
    \SetKwFunction{FInterMVA}{InterMethodVarAnalysis}
    \SetKwFunction{FIntraMVA}{IntraMethodVarAnalysis}
    \SetKwFunction{FForwar}{ForwardAnalysis}
    \SetKwFunction{FBackwar}{BackwardAnalysis}
  
    % BackwardAnalysis($src_{var}$, $src_{stmt}$, $src_{m}$)\;
    BackwardAnalysis($m_t$, $s_t$, $v_t$)\;

    IntraMethodVarAnalysis($m_t$, $s_t$, $v_t$) \;
    % \vspace{-1.1ex}\;\vspace{-1.1ex}
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FIntraMVA{$m$, $stmt$, $var$}}{
        $uses$ = find statements that use $var$ in method $m$ \;
        \For{$u$ in $uses$}{
            store($var$, u) in $DF$ \;
            ForwardAnalysis($m$, $u$, $var$)
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    \SetKwProg{Fn}{Def}{:}{\KwRet}
    \Fn{\FBackwar{$m_t$, $s_t$, $v_t$}}{
        % InterProcedureVariableAnalysis($m$, $stmt$, $var$)  \;
        % $cfg$ = construct\_cfg($m$)\;
        $defs$ = getDefsOfAt($v_t$, $s_t$, $cfg$)  \;
        \For{$d$ in $defs$}{
            $src_{var}$ = get the signature of $v_t$ in $d$\;
            $caller_{list}$ = find methods that invoke $m_t$ \;
            \For{$m$ in $caller_{list}$}{
                $src_{stmt}$ = statements that invoke $m_t$ in $m$\;
                $src_{v}$ = variables in $src_{stmt}$ that correspond to $v_t$\;
                \If{$src_{v}$  is \textit{Variable}}{
                    BackwardAnalysis($src_{v}$, $src_{stmt}$, $src_{m}$)
                } \ElseIf{$src_{v}$ is \textit{Constant}}{
                    store ($v_t$, $src_{stmt}$) in $DF$
                }
            }
        }
    }
    % \vspace{-1.1ex}
    \;
    % \vspace{-1.1ex}
    
    \SetKwProg{Fn}{Def}{:}{}
    \Fn{\FForwar{$m$, $stmt$, $var$}}{
        $tar_{stmt}$ = find all statements that contain $stmt$ \;
        \For{$s$ in $tar_{stmt}$}{
            store ($var$, $s$) in $DF$ \;
            \If{$s$ contain invoke statements}{
                $tar_{m}$ = method that invokes $stmt$ in $s$ \;
                $tar_{v}$ = variable in $tar_{m}$ that correspond to $var$\;
                ForwardAnalysis($tar_{method}$, $s$, $tar_{v}$)
            }
        }
    }

% \vspace{-1ex}
\end{algorithm}




% 可以加个algorithm
% \input{figures/algorithm_data_flow}

% The method used for extracting the TPL data usage extraction is shown in Algorithm ~\ref{alg:data_usage}.
%methods in {\oursystem}. 
%
% With the intermediate representation (i.e., Jimple in {\soot}), we get the method body, the method's statements and target variables.
Algorithm~\ref{alg:data_usage} sketches the TPL data usage analysis method.
% 
{\oursystem} iterates over all statements in TPL to locate the target variables ({\small{$var$}}) that represent personal information listed in Tab.~\ref{tab:data_type}.
%
Then, {\oursystem} conducts both inter-methods and intra-methods analyses to get the data flow.
%
For inter-methods analysis, {\oursystem} backward analyzes statement {\small{$s_t$}} in method {\small{$m_t$}} with the DOI {\small{$v_t$}} (line 1).
%
% construct the control flow graph (CFG) of current methods ($m_{src}$) using soot.
% Specifically, for backward analysis, {\oursystem}
The backward analysis locates the definition statements ({\small{$defs$}}) in {\small{$m_t$}} that relates to DOI {\small{$v_t$}} (line 11).
%
For statements in {\small{$defs$}}, {\oursystem} iterates {\small{$defs$}} and locates the variable signature of {\small{$v_t$}} in {\small{$d$}} (line 12-13).
%
{\oursystem} iterates the function call graph of TPL and finds the methods ({\small{$caller_{list}$}}) that invoke {\small{$m$}} (line 14).
%
For each caller {\small{$m$}}, {\oursystem} locates the statements ({\small{$src_{stmt}$}}) in {\small{$m$}} that invoke {\small{$m_t$}}.
%
{\oursystem} finds the variable {\small{($src_v$)}} in {\small{$src_{stmt}$}} that corresponds to DOI {\small{$v_t$}} (line 17).
%
If {\small{$src_{v}$}} is a variable, {\oursystem} continues backward analysis, starts with {\small{$src_{stmt}$}} in {\small{$src_m$}} and focuses analysis on variable {\small{$src_v$}} (line 18-19); 
% otherwise, 
if {\small{$src_{v}$}} is a constant, {\oursystem} finds one piece of code that describes the data usage of {\small{$var$}} (line 21).



To locate the {\small{$v_t$}}'s data usage in {\small{$m_t$}}, {\oursystem} performs \textit{intra-methods variable analysis}.
%
Specifically, {\oursystem} locates all statements ({\small{$uses$}}) that uses {\small{$var$}} in method {\small{$m$}} (line 5).
%
For each statement {\small{$u$}} in {\small{$uses$}}, {\oursystem} stores the usage of variable {\small{$var$}} (line 7) because the target variable have been used in the statement {\small{$u$}}.
%
Then, {\oursystem} use forward analysis (line 8) to identify whether {\small{$var$}} is used further.
%
% Specifically, {\oursystem} locates the statements ($tar_{stmt}$) that contain $stmt$ because the $stmt$ maybe invoked in some \textit{specialinvoke} statements accordingly to the prosperity of {\soot}.
%
For each statement {\small{$s$}} in {\small{$tar_{stmt}$}}, {\oursystem} stores the the data flow describing the data usage. 
% data usage.
%
If {\small{$s$}} contains invoke statements, {\oursystem} locates the method {\small{$tar_m$}} that calls {\small{$stmt$}} (line 28), builds the variable {\small{$tar_v$}} corresponding to target variable {\small{$v_t$}} and continues the forward analysis (line 30).
%





% %
% Then, we get the statements that defines $var$ in $m_{src}$ through analyzing the CFG using \textit{soot}.% API.
% % We get the definition sites for $var$ at a certain point (statement) that defines $var$ in the method.
% %
% Next, we traverse the call stack in reverse to find the the statement that initially defines target variable.
% %
% Then, we get the data flow of target variable.
% %
% For intra-procedure analysis, we iterate the statements in current method ($m_{src}$) to trace the data flow.
% %
% It worth noticing that when we find recursive invocation, we terminate the current traverse to avoid redundant analysis.



%update:25-Jan-2022:
%
%Figure out the problem that flowdroid cannot be directly used to analyze \textit{dex/jar} files.
%
%To deal with it, we write methods based on soot and soot-infoflow.
%
%Currently, we can analyze the data flow of specific methods.
%
%Demo: 
%
%\textbf{APK}: E133-3A32B-15F79-A6AA6-6CB57-FA7FC-648AC-68351-6ECDE-7399B-89999-14012-474F2.apk
%
%\textbf{Target}: location
%r
%\textbf{dataflow:}



% How to define \textbf{\textit{callback}} methods?

%%%\textbf{Questions:} When analyzing \textit{.jar} file, the \textit{infoflow} can find the target trace, e.g. the \textit{location} in aforementioned case. 
%However, when analyzing \textit{.dex}, the trace missed.
%
%Another interesting thing is: when analyzing the demo using \textit{soot} only, the results of \textit{.dex} returns more invocation results than results of \textit{.jar}.
%There could be some problems in \textit{dex2jar}.



\vspace{-1ex}
\subsection{Identify data usage statements in TPL's privacy policy}
\label{sec:tpl_pp}
\vspace{-1ex}
% Privacy policy analysis 
% Data usage identification is a kind of named entity recognition (NER) task in natural language processing.
%
TPL privacy policy analysis aims aims to identify the documents' data usage statements.
%
% {\oursystem} analyzes TPLs' privacy policy to extract used data.
%
The pipeline of our privacy policy analysis consists of three steps: 
1) preprocessing of privacy policy,
2) named entity extraction, 
and 3) data usage action construction.
%
Finally, each privacy policy is abstracted into a set of abstract data usage patterns (ADUP) that describe \textit{who} will (\textit{not}) \textit{access} \textit{what kinds of data} with \textit{whom}. 
%
Each ADUP is in form of {\small{\{data\_entity, action, \{data\_type\}, \{data\_recipient\}, \{neg\}\}}}.
% \{$\small{data\_entity,action,\{data\_type\},\{data\_recipient\},\{neg\}}$\}.
%
For example, \textit{``We share your personal information with our service providers," (in Adad's privacy policy)} is abstracted as {\small{\textit{\{app, share, \{personal information\}, \{service provider\}, false\}}}}.
%The extraction methods for each component of ADUP is detailed as follows.


% 1) fined-turning a state-of-the-art NER model to adapt our application scenario, 2) identifying data entities in privacy policy using pretrained model, and 3) applying expert system to identify the data usage in privacy policy.

\subsubsection{Preprocessing privacy policy}
\label{sec:pre_pp}
To download the apps' privacy policies from Google Play~\cite{googleplay},
we use the \textit{Selenium Webdriver}~\cite{gojare2015analysis} to open web pages of privacy policies.
%
Then, we use \textit{html2text}~\cite{html2text} to transform downloaded privacy policies into plain text. 
%
However, the transformed plain text contains many special characters, e.g. $*$ and $|$, which will lead to unnatural segmentation of sentences. 
%
{\oursystem} first uses patterns~\cite{stack_pre_nlp} to eliminate special characters. 
%
% Besides, enumeration items are in privacy policies to detail the related data items.
%
Besides, privacy policies use enumeration items~\cite{andow2019policylint} to detail related data items, which may lead to a whole sentence being segmented by item index and further cause losing information.
%
{\oursystem} merges the items by searching for sentences ending in a colon, and the next sentence starts with list items, such as bullets, roman numerals, and formatted numbers.
%
% Then, we use the dependency parse tree to get the constellation between words.
%


\subsubsection{Data access extraction}
%
With preprocessed privacy policy sentences, {\oursystem} analyzes each sentence to identify data access descriptions.
%
Since the interrogative sentences are commonly used in privacy policies but do not describe the types of accessed personal information, we omit them by checking the interrogative words (i.e., who, where, when, why, whether, what, and how). 
%this sentence as it would be an \textit{Introduction}, 
For example, the sentence \textit{\underline{What} personal information do we collect} is omitted. %  (appid: wp.wattpad).
%
Then, we construct the part-of-speech (POS) tagging, and dependency parsing tree (DPS) for each sentence.
%
We will omit sentences without verb words because those sentences will not claim data access behaviors.
%
For example, ``\textit{Do-Not-Track Signals and Similar Mechanisms}" in \textit{Facebook Open Source Privacy Policy} only claims the title of the paragraph.
%
For the remaining sentences, we follow the following steps to extract data action, data entity, and data actor.
% data action, data objects, data operator, and data recipient (if applicable).




%
\noindent\textbf{Identification of data action words}. 
%
We first identify whether the verb words are in the data usage word list (Tab.~\ref{tab:actionwords}).
%
We stem the word using \textit{nltk}~\cite{loper2002nltk} to deal with English verb tenses. 
%before identification 
% since English verbs have tenses. %, singular or plural forms.
%
% Besides, we will identify the verb as some statements that claim the data sharing and collection action in one sentence, for example: \textit{we \underline{collect} the information you have authorized the platform to \underline{share} with us, such as your name, email address, gender, date of birth, friend list, profile picture and playlists}(us.current.android).
%
We also identify the modifier of target verb because the privacy policies also claim the data they will not use or collect.
%
To achieve this, we analyze the dependency parsing tree and recognize the words whose relation with the target verb is `\textit{advmod}' (adverbial modifier) or `\textit{mmod}' (modal verb modifier).
%
If the words or their tags are negative (i.e., `neg'), we regard the data usage action as negative one.
%
To this end, {\oursystem} identifies
% data-related sentences and 
data sharing or collection operations.



\begin{table}[]
\centering
\smaller
% \vspace{1ex}
\caption{Personal information and corresponding APIs.}
%\vspace{-1ex}
\scalebox{0.95}{
\begin{tabular}{@{}p{0.07\textwidth}p{0.23\textwidth}p{0.14\textwidth}@{}}
\toprule
\textbf{PI}                    & \textbf{Class Name}                                      & \textbf{Method Name}                         \\ \midrule
Ad ID                          & AdvertisingIdClient                                      & AdvertisingIdClient                          \\
\rowcolor[HTML]{EFEFEF} 
Bluetooch address              & android.bluetooth.BluetoothAdapter                       & getAddress                                   \\
Camera                         & android.hardware.Camera                                  & setPreviewDisplay                            \\
\rowcolor[HTML]{EFEFEF} 
Cell   Loca-tion                & android.telephony.TelephonyManager                       & getCellLocation                              \\
Contact                        & android.provider.ContactsContract                        & PhoneLookup                                  \\
                               & \cellcolor[HTML]{EFEFEF}android.location.Location        & \cellcolor[HTML]{EFEFEF}getLatitude          \\
                               & android.location.Location                                & getLongitude                                 \\
                               & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLastKnownLocation \\
                               & android.location.LocationManager                         & requestLocationUpdates                       \\
\multirow{-5}{*}{GPS Location} & \cellcolor[HTML]{EFEFEF}android.location.LocationManager & \cellcolor[HTML]{EFEFEF}getLongitude         \\
Sim Number                     & android.telephony.TElephonyManager                       & getSimSerialNumber                           \\
\rowcolor[HTML]{EFEFEF} 
IMEI                           & android.telephony.TElephonyManager                       & getDeviceId                                  \\
IMSE                           & android.telephony.TElephonyManager                       & getSubscriberId                              \\
\rowcolor[HTML]{EFEFEF} 
TimeZone                       & java.util.Calendar                                       & getTimeZone                                  \\
MAC address                    & android.net.wifi.WifiInfo                                & getMacAddress                                \\
\rowcolor[HTML]{EFEFEF} 
Password                       & android.accounts.AccountManager                          & getPassword                                  \\
Phone   Number                 & android.telephony.TelephonyManager                       & getLine1Number                               \\
\rowcolor[HTML]{EFEFEF} 
SMS                            & android.telephony.SmsManager                             & sendTextMessage                              \\
SSID                           & android.net.wifi.WifiInfo                                & getSSID                                      \\
\rowcolor[HTML]{EFEFEF} 
User Credential                & android.accounts.AccountManager                          & getAccounts                                  \\
UserName                       & android.os.UserManager                                   & getUserName                                  \\ \bottomrule
\end{tabular}
}
\vspace{-2ex}
\label{tab:pi_api}
\end{table}



% \vspace{1.5ex}
\noindent\textbf{Identification of data entity}.
%
We identify objects of identified collecting and sharing words (target verb) according to DPS.
%
{\oursystem} first merges the noun phrase (NP) tag into one noun tag according to POS tagging to simplify sentence structure. 
% because many nouns exist in sentences to describe the related data.
%
For example, consider the following sentence in the privacy policy of the app \textit{video.reface.app} ``\textit{\small{With the use of Google Analytics, we collect such data as IP-Address, your \underline{device model}, \underline{screen resolution} and \underline{operation system}, \underline{session duration}, your location}}''.
%
% {\oursystem} identifies the objects of the target verb.
%
As only one noun or noun phrase will be identified as the object of the target verb~\cite{hanlp21}, {\oursystem} locates all coordinating nouns for the object. 
%
Specifically, {\oursystem} iterates the constituency parsing tree, which is calculated by two stages conditional random field (CRF) model~\cite{zhang2021fast}, to find the sub-trees whose \textit{a) root label are common noun (NN tag) or Noun Phrase (NP)} or \textit{b) coordinating conjunction (CC tag) or punctuation exist in the sub-tree}.
% 
The condition \textit{a)} denotes that the leaves in the tree can be merged into one noun, and  \textit{b)} indicates there may exist enumeration items or coordinating nouns.
%
If we omit the relations, {\oursystem} cannot fully extract all data entities, i.e., false-positive occurs.
%
To this end, we obtain all candidate data objects in each sentence.
%


%\vspace{1.5ex}
\noindent\textbf{Identification of data actor.}
%
To identify the data actor, {\oursystem} analyzes DPT and locates the words whose relation with sharing and collection verbs is nominal subject (``\textit{nsubj}") or direct object (``\textit{dobj}").
%
% Besides, if the sentence or the object is prepositional complement or clausal complement of a preposition, we will iterate the DPT to find the coordinating verb and then locate the nominal subject of coordinating verb.
Suppose the sentence or the object is a prepositional complement or clausal complement of a preposition (``\textit{ccomp}").
%
% In that case, we will iterate 
We iterate the DPT to find the coordinating verb and then locate the nominal subject of the target verb.
%
The nominal subject and the verb will be added to the actor list and the sharing/collection verb list, respectively.
%
We also consider the data actor as users separately, under which situation the real data actor is the user rather than the supplier.
%
For example, ``\textit{we will not collect the personal information you shared with us}''.
%
The data actor should be ``you"  while the data recipient is ``us".

% Besides, for the object complementary cases, (i.e., \textit{"we will ask you to provide personal information that is necessary to provide those services to you"})

% \noindent\textbf{Data recipient identification.}
%






%\vspace{1.5ex}
\noindent\textbf{Post-process}
%
To eliminate false detection, e.g., conditional clauses, we design rules to avoid false data usage extractions.
%
For sentences that start with condition or assumption hints, such as \textit{`if'} (\textit{``if you do not provide your personal information"}), we will not identify the data usage pattern inside.
% (i.e., \textit{\{you, not provide, personal information\}}).


\begin{table}[]
\centering
\smaller
\caption{Data sharing and collecting words.}
% \vspace{3.5ex}
%p{0.9\columnwidth}
\begin{tabular}{p{0.23\columnwidth}p{0.67\columnwidth}}
\toprule
\textbf{Action Type} & \textbf{Keywords} \\ \midrule
Collect &  access, check, collect, gather, know, obtain, receive, save, store, use \\ \hline
Sharing &  accumulate, afford, aggregate, associate,  cache,  combine, convert, connect,  deliver, disclose, distribute, disseminate, exchange,  gather, get, give, keep, lease, obtain, offer, post, possess, proxy,  provide, protect against, receive,  rent, report, request, save, seek, sell, share, send, track,  trade, transport, transfer, transmit\\ \bottomrule
\end{tabular}
\vspace{-2ex}
\label{tab:actionwords}
\end{table}


\subsection{Extract host apps' interaction with TPLs}
\label{sec:host_app_data}

% \subsection{Data Sharing with Enumeration}
% \label{app:demo:tpl_enumeration}

To identify whether host apps' privacy policies are consistent with their TPL usage
%  with their interaction behavior with TPLs, 
{\oursystem} conducts static analysis to identify the host apps' interaction with TPLs.
%
{\oursystem} discloses what kinds of PI data (Tab.~\ref{tab:data_type}) are shared with TPLs.
%
{\oursystem} uses Flowdroid~\cite{arzt2014flowdroid} to construct FCG of apps.
%
Since Flowdroid optimizes Android app analysis process~\cite{arzt2014flowdroid}, {\oursystem} directly uses the FCG constructed from Flowdroid, and then iterates each statement to locate the variables related to TPLs or PI.   
% {\oursystem} does not use the methods in \S\ref{sec:tpl_data} to construct the entry points of apps because Flowdroid prepossesses apps' Manifest and resources files to identify the entry points and create the dummy main function~\cite{arzt2014flowdroid}. % that are proven to be more comprehensive and effective~\cite{arzt2014flowdroid}.
%
% Then, {\oursystem} 
%
{\oursystem} performs the data flow analysis (\S\ref{sec:tpl_data}) to find the PI related data flow.
%
To identify TPLs, {\oursystem} identifies whether the statement contains the TPLs' name or package name or not.
%
After obtaining TPLs and PI data, we identify whether the sinks exist in the data flows.
%
% This is done by using FlowDroid~\cite{arzt2014flowdroid}.
%
Besides, we optimize the signature of sink invocation (\textit{SSI}) using the invoke statement.
%
% For example, if the sink method ~\textit{$\langle$android.content.Intent: android.content.Intent setAction(java.lang.String)$\rangle$} is invoked in statement: (\textit{JimpleLocalBox(\$r1) in virtualinvoke \$r1.$\langle$ android.content.Intent: android.con-tent.Intent setAction( java.lang.String ) $\rangle$  
% ( "com.google.android.gms.-fitness.app\_disconnected" )} 
% % (\textsf{st1} )
% , we use the the whole invocation statement as the stored signature.
%
{\oursystem} matches the \textit{SSI} in both PIs' data flow and TPLs' data flow.
%
Once the \textit{SSI} is matched between $TPL_i$ and $PI_j$, {\oursystem} regards the host app sharing the $PI_j$ with the $TPL_i$.
%
If the \textit{SSI} only exits in $PI_j$'s data flow, {\oursystem} identify that the host app collects $PI_j$  without sharing it with TPLs.




\subsection{Identify TPLs usage statements in host apps' privacy policy}
\label{sec:host_app_pp}

To identify the TPL usage statements in host {\app}s, we extract two descriptions from the privacy policy: 
%
a) the \textit{data sharing} related statements and 
b) TPL related  descriptions.
%
The \textit{data sharing} related statements claim how the {\app} discloses users' personal information under which situations.
%
For example, the {\app} (\textit{flipboard.boxer.app}) claims that "\textit{We share personal information with vendors and service providers that help us offer and improve our service}".
% in their privacy policy.
%
The statement indicates that \textit{flipboard.boxer.app} will share users' \textit{personal information} with vendors and service providers.
%
If {\oursystem} also identifies the {\app}'s data flow sharing users' data with TPLs tagged as vendors or service providers, {\oursystem} regards the app's privacy policy as consistent with its behavior.
%
% Besides, some {\app}'s privacy policies will enumerate the TPLs they used and the data they shared with TPLs.
% (see demo in~\ref{app:demo:tpl_enumeration}). 
%
% The patterns are extracted from our manually labeled 400 privacy policies (200 for Chinese and English separately).
%
% The patterns are extracted from our manually labeled 200 privacy policies.


% First, we use methods in \S\ref{sec:pre_pp} to preprocess TPLs' privacy policy.
%
% Then, 
After preprocessing TPLs' privacy policies (\S\ref{sec:pre_pp}), we use NLP methods~\cite{hanlp21} to get the tokenization, POS tagging and DPS for each sentence.
%
For sentences with verbs, we check whether the verb is in \textit{sharing} word list (Tab.~\ref{tab:actionwords}).
%
After obtaining the data sharing verb, we identify the data recipient to determine which TPL the data are shared with.
%
Specifically, we iterate the words in the sentence.
%
If the word is the object of a preposition (\textit{pobj}) or an indirect object (\textit{iobj}) of the verb, we identify the words as candidate data recipients, i.e., TPLs.
%
For enumeration patterns, once we identify the sentence that a) starts with a noun or noun phrase (denoted as $tar_{TPL}$) that is involved in our TPL list, v) the noun ends with colon following only noun or noun phrases, we regard the noun (phrases) following colon as the shared data with $tar_{TPL}$.

%There are two types of action:
%1) "We may collect \textbf{data} from third parities."
%2) "We share \textbf{data} with third parties."


\subsection{TPL privacy leakage investigation}


{\oursystem} investigates TPL privacy leakage by performing 
\textit{normativeness analysis}, 
\textit{privacy policies legality analysis}, 
and \textit{privacy leakage transmissibility analysis}. 


\noindent\textbf{Normativeness analysis} identifies whether TPL provides privacy policies.
%
According to GDPR Article 12 (1)  and  Article 13 (1), TPLs, who act as the data controller or third party of personal data, should infer users about data access behaviors in a concise, transparent, intelligible and easily accessible form.
%


\noindent\textbf{Legality analysis} identifies conflicts between TPLs' behavior and privacy policy statements.
%
Specifically, {\oursystem} identifies whether TPLs' data access actions are clearly claimed in their privacy policies by combining the data flow results (\S\ref{sec:tpl_data}) and PP ADUP (\S\ref{sec:tpl_pp}).
%
If {\oursystem} identifies data usage in TPL data flow results are not mentioned in \textit{$data\_type$}s of ADUP set, the TPL will be regarded as violating legal requirements.




\noindent\textbf{Privacy leakage transmissibility analysis} 
\kaifa{checks to what extent the vulnerable TPLs, which potentially leak user privacy, will affect other TPLs or apps.
%
{\oursystem} summarizes artifacts that use vulnerable TPLs from {\textit{Maven Repository}} to investigate the impact of TPL's privacy leakage.
%
Specifically, {\oursystem} crawls \textit{Usages} information in {\textit{Maven Repository}} to count the number of artifacts that use vulnerable TPLs.
%
% The more artifacts using vulnerable TPLs, the more effect of TPLs' vulnerability. 
}

\begin{comment}

\noindent\textbf{Vulnerability transmissibility analysis} checks to what extent the TPLs with vulnerabilities will affect other TPLs or apps.
%
{\oursystem} adds up artifacts that use vulnerable TPLs from {\textit{Maven Repository}}.
%
The more artifacts using vulnerable TPLs, the more effect of TPLs' vulnerability. 
% \xiancm{incorrect.... not accurate}

\end{comment}

\subsection{Regulation conflict analysis}

Regulation conflict analysis discovers whether the usage of TPLs in host apps comply regulation requirements.
Two kinds of conflict will be identified:

% \begin{itemize}[leftmargin=*]
    % \item 
    
\noindent{$\bullet$} {\oursystem} identifies whether usage of TPLs from data flow analysis (\S\ref{sec:host_app_data}) is clearly claimed in their privacy policy statements(\S\ref{sec:host_app_pp}. 
    % To achieve this, 
    {\oursystem} investigates whether the TPL package names in data flow analysis match the \textit{$data\_entity$} or \textit{$data\_recipient$} in ADUP of host app privacy policy results.
    
    % \item 
\noindent{$\bullet$}    {\oursystem} discloses whether the host apps clearly state their data interaction with TPLs. 
    %
    % To achieve this, 
    {\oursystem} identifies whether the apps' TPL interaction behavior (\S\ref{sec:host_app_data}) is clearly stated in host apps' privacy policies (\S\ref{sec:host_app_pp}.
    % {\oursystem} matches the host apps interaction behaviors results (\S\ref{sec:host_app_data} and host apps' privacy policies analysis results (\S\ref{sec:host_app_pp}).
    % For host apps that disclose their interaction with TPLs, {\oursystem} also identifies whether the data usage of TPLs, that is achieved from data flow analysis of TPLs (\S\ref{sec:tpl_data}), are clearly and comprehensively disclosed in host apps privacy policies.
% \end{itemize}



% \subsection{Extract data usage in host {app}'s privacy policy}

% In this subsection, I wil; introduce how to analyze the data usage of TPL through analyze the TPL bytecode.

% We should target specific sensitive data, in this way we can identify the DataFlow of TPL:

% Email, userid, username, password, contact, gps, location, device ID, identifier, advertising ID, account/imei address, PHOTOGRAPHY


% To identify the TPL usage in our 




\begin{comment}


\subsubsection{Demo}

package name = \textbf{``com.facebook.ads"}

    

    

%\begin{itemize}
%    \item \textbf{email}  
    % SPECIAL edge: specialinvoke \$r15.$\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$( \kaifa{"EMAIL"}, 15, "email" ) in $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$() $\rangle$ ==$\rangle$ $\langle$ com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$( java.lang.String, int, java.lang.String ) $\rangle$
    
%    \item \textbf{userid} 
    % VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\kaifa{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$
    
%    \item \textbf{deviceid} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$(``Stub!") in $\langle$android.view.InputDevice: int[] \kaifa{getDeviceIds()} $\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$

 %   \item \textbf{identifier} 
    % VIRTUAL edge: \$r3 = virtualinvoke r1.$\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$() in $\langle$com.facebook.ads.internal.bridge.gms.AdvertisingId: com.facebook.ads.internal.bridge.gms.AdvertisingId getAdvertisingIdInfoDirectly(android.content.Context)$\rangle$ ==$\rangle$ $\langle$com.google.android.gms.ads.identifier.AdvertisingIdClient\$Info: java.lang.String getId()$\rangle$
    
%    \item \textbf{account} 
    % SPECIAL edge: specialinvoke \$r0.$\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$(``Stub!") in $\langle$android.content.ContentResolver: boolean isSyncPending(android.accounts.Account,java.lang.String)$\rangle$ ==$\rangle$ $\langle$java.lang.RuntimeException: void $\langle$init$\rangle$(java.lang.String)$\rangle$


    
%    \item \textbf{photo}: 
    % SPECIAL edge: specialinvoke \$r38.$\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$(\kaifa{"PHOTOGRAPHY"}, 38, "photography") in $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$clinit$\rangle$()$\rangle$ ==$\rangle$ $\langle$com.facebook.ads.ExtraHints\$Keyword: void $\langle$init$\rangle$(java.lang.String,int,java.lang.String)$\rangle$
    
%\end{itemize}



% For data that android system provides API to collect, such as location, we identify the invocation of those methods. \kaifa{to list the related API in appendix}
% %
% For other data, such as gender or username, we identify the parameters passed to target server.
% %
%such as:  \textit{VIRTUAL edge: r6 = virtualinvoke \$r4.$\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$(\textbf{"getUserId"}, \$r5) in $\langle$com.facebook.ads.internal.bridge.fbsdk.FBLoginASID: java.lang.String getFBLoginASID()$\rangle$ ==$\rangle$ $\langle$java.lang.Class: java.lang.reflect.Method getDeclaredMethod(java.lang.String,java.lang.Class[])$\rangle$}

\end{comment}











==> tmp/xzintro.tex <==
\section{Introduction}

% \input{table/regulation_summary}


% \vspace{0.5em}
% \begin{quote}
%     \emph{\textbf{``Hedges have eyes and walls have ears.''}}
%     \begin{flushright}
%     - Trusler, John, 1735-1820.
%     \end{flushright}
% \end{quote}
% \vspace{1em}




% Nowadays, the smartphone is ubiquitous, and mobile apps, as a significant part of mobile ecology, are playing essential roles in our daily life, from living, working, and education to business~\cite{deepintent2019SIGSAC}. 
Nowadays, the smartphone and mobile apps are playing essential roles in our daily life~\cite{deepintent2019SIGSAC}. \xiancm{suggest use daily lives}
Besides, more and more developers tend to use many off-the-shelf \revise{toolkits or}\xiancm{can delete this part, we just say TPLs is ok , let everything close to your topic} third-party libraries (TPLs) to facilitate the development process, to avoid reinventing the wheel~\cite{atvhunter2021ICSE,libdetect2020ASE}.
% Have you ever thought about the security of these third-party libraries (TPLs) used in your apps? 
% TPLs probably leak your personal privacy. 
%
However, developers may omit the privacy threat in TPLs. 
%
For example, the advertisement libraries may leak users' personal information (e.g., IMEI)~\cite{short2014android}.
%
\xian{Some} TPLs (e.g., advertising and analytic libraries) rely on the personal information to provide better service.\xiancm{add reference here} 
%
However, some TPLs may collect user data that is not necessary for providing related services. 
Such behaviors may lead to privacy leakage or even security concerns~\cite{deepintent2019SIGSAC, harty2021logging, tangtse:21a}.
%
% However, behaviors of those TPLs are undesirable or even harmful, including disclosing users' sensitive information such as location and personal profiles without informing users~\cite{deepintent2019SIGSAC,harty2021logging, tangtse:21a, tang:ase19}. 
%
For the dominant mobile operating system Android~\cite{mobile_operating_system}, \xiancm{rewrite this sentence but should delete this sentence}\xian{Nowadays, Android, as the dominate mobile operating system~\cite{mobile_operating_system}}\xiancm{even that, IMHO, I still cannot find the connection between the two sentences, Android as the dominant mobile operation system so? why this can lead to the permission mechanism issues??}
% Android, the privacy leakage from TPLs is more serious.
the permission mechanism also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}. \xian{Besides, the permission mechanism of Android also increases the possibility of leaking user privacy by TPLs~\cite{lin2012expectation, kawabata2013sanadbox, zhang2013aframe, liu2015efficient, shekhar2012adsplit, pearce2012addroid,he2018investigation, salza2018developers, zhan2017splitting, wang2014compac, sun2014nativeguard}.}
%
Since the host apps share the same process space and permissions with TPLs, \revise{this mechanism will\xiancm{delete will} lead to over-privileged TPLs. }\xian{the mechanism violates the principle of least privilege, which leads to TPLs is over-privileged.}
%
Recent papers find that the permissions abuse makes TPLs access users' personal information and causes potential privacy leakage~\cite{qiu2021libcapsule, grace2012unsafe, birendra2016android,xu2022lie,li2021embedding,di2021influencing,seneviratne2015measurement,cybernews_dataleakage}. 
%
In addition, the incorrect use of TPLs~\cite{zhang2020does, chen2014information, cybernews_dataleakage} may cause serious personal information leakage. 
% from host apps. 
%
For example, a recent report~\cite{cybernews_dataleakage} discloses that popular Android apps with over 142.5 million installations leak user data to unauthorized third parties. 
%
Zhang et al.~\cite{zhang2020does} disclose 120 of 555 apps that share users' personal information to analytic service TPLs without encryption.
%
Besides, linking and mining large amounts of unencrypted personal information will \\xiancm{pay attention to the accurate expression, do that may cause but not necessary}\revise{lead to}\xian{probably pose threats to} serious personal privacy leakage~\cite{kiranmayi2018reducing, chen2014information}.
%
% Thus, it is urgent to identify TPLs' data sharing and collection actions to protect user privacy.
Thus, it is urgent to design a system to check the data access behavior and privacy policies of TPLs so that we can determine if TPLs are compliant with the privacy regulations or not.

%analyze the compliance of TPLs data access behavior and privacy policies with regulations to protect user privacy.
%
% Even the unencrypted personal data are only shared with trusted TPLs that do not abuse the data, linking and mining of a large amount of unencrypted personal information also could lead to serious personal information leakage~\cite{kiranmayi2018reducing, chen2014information}.
% }




% To normalize apps' behaviors and prevent privacy leakage, various personal privacy  protection-related regulations (e.g., CCPA, CPRA, GDPR, ICCPR)~\cite{piss, zhSDKLaw, gdpr, ccpa} have been promulgated to protect people's personal information from abuse, which requires developers to clearly understand TPL behaviors and declare these sensitive behaviors in their privacy policy so as not to violate the regulations.
%
To normalize apps' privacy related behaviors and prevent privacy leakage, various privacy related regulations 
% (e.g., CCPA, CPRA, GDPR, ICCPR, CFR)~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr}
(e.g., {\textsc{\small{California Consumer Privacy Act (CCPA), General Data Protection Regulation (GDPR)}}})~\cite{piss, zhSDKLaw, gdpr, ccpa, cfr})
have been promulgated to protect people's personal information from being abused.
%
\revise{However, app developers may unconsciously violate regulations since they cannot understand all TPLs' functionalities and do not have privacy-related background knowledge.}\xiancm{rewrite} \xian{However, app developers may unconsciously violate regulations of used TPLs because they do not need to understand the execution logic of these TPLs, they just need to follow they user guidelines to invoke these TPLs. Due to lack of the security consciousness, some developers may never check whether these used TPLs in their apps have a privacy policy and whether these TPLs may have security risk with respect to privacy leakage.  }
%
The latest \textit{\small{Google Play Developer Program policies (GPDP)}}~\cite{google_play_pp_update} ask developers to ensure the TPLs used in their apps are compliant with GPDP~\cite{gpdp}.
% 
% Regulations consider {\tpl}s as data controllers~\cite{gdpr,piss,ccpa}. 
%
Developers of {\tpl}s are required to provide privacy policies and disclose data usage.
%
Otherwise, the apps violate regulation or market's requirements and they may be removed from the app market~\cite{googleplay_requirements, appgallery_requirements}.
% are queried to withdraw the apps. 
%
\revise{To make {\tpl}s comply with regulations and help developers correctly use {\tpl}s, it is necessary to analyze the consistency between {\tpl}s' data usage and privacy policies.}\xiancm{the logic is not ok, you cannot make the TPL comply with the regulations, you are not the authors, or developers of TPLs, you just want to conduct the analysis, how do you make the TPLs comply with the regulations}





% 介绍现有的 app pp 分析
% Recent research~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding} propose methods to identify the legality of apps, i.e., the apps are required to disclose personal information usage in their privacy policies. 
%
\revise{Some methods have been proposed to identify the privacy issues\xiancm{privacy issues are not equal to privacy policy analysis, which one you want to say ,use accurate expression} of mobile apps~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding}.}\xiancm{based on your comments, I can see you want to say the pp analysis of app based on previous research. however, the key issues is that the privacy issues are not equal to pp analysis, your English still need to improve}
%
However, they cannot identify the conflict between TPLs and regulations because they either failed to identify TPLs functionalities or analyze TPL privacy policies.   \xiancm{the logic of this sentence is totally incorrect, current work cannot identify the conflict between TPLs and regulations, we need to analysis the conflicts between TPLs' behaviors and regulations, this is one solution. but failed to analyze policies cannot solve your issues. there are several conflicts, the behaviors between the TPLs' behaviors and pp, the tpls' behaviors and regulations, the pp and regulations. so we need to give a clear target at the beginning, and then we just can organize our paper}
% 
% However, those systems can not identify TPL-related privacy leakage issues because the systems miss analyzing TPL functionalities and privacy policies, and analyzing the consistency between TPLs' code and privacy policy statements.
%
PoliCheck~\cite{ppcheck} performs dynamic analysis to get traffic flow for analyzing the apps' data usage.
Then, it applies data and entity dependency tree analysis to extract data usage statements from the privacy policy, and designs rules to identify the conflicts. \xiancm{this part is about the app pp analysis}
% checks the consistency between the apps' data collection and sharing behaviors with the privacy policy.
%
PAMDRroid~\cite{zhang2020does} identifies the TPLs' misconfiguration caused by personally identifiable information (PII) leakage.
%
PAMDroid investigates whether the PII is preprocessed, such as anonymization and encryption, before sharing with analytic service libraries.\xiancm{this one is about the TPL misconfiguration analysis}
%
PPChecker~\cite{ppchecker} discovers the trustworthiness of apps' privacy policies, and identifies consistency of app's behavior and privacy policy statements and the consistency of privacy policies from different sources.
% Specifically, PPChecker identifies a) whether apps' privacy policies cover all apps' personal information (PI) usage behaviors (\textbf{completeness}), b) whether apps' privacy policies correctly claim the personal information(PI) that the app uses or does not use (\textbf{correctness}), c) whether privacy policies' description uses vague words (\textbf{preciseness}), d) whether apps' privacy policies consistent other sources, such as TPL and Google Play, (\textbf{consistency}), and e) whether the privacy policies are easy-to-read.
%
PPChecker concentrates on apps' privacy policies and is out-of-dated to satisfy the latest regulations.\xiancm{and this one is about tht app pp analysis agin}
% Existing methods can not identify TPL-related regulation violations since they 

\xiancm{have you found your writing issues, the logic is not fluent and coherent, the TPL and app pp analysis are across each other, the logic is not ok. If I were you, I will write the app pp analysis first and then give the status quo of tpl pp analysis and the present the research gap so that we can introduce our tool}

\xiancm{I rewrite this part but also need to your help to summarize two papers which also talk about the pp analysis on tpls}

\xianw{The most earlier research usually focus on the privacy policy analysis of mobile apps~\cite{ppcheck,ppchecker,andow2019policylint,yu2016can,nguyen2021share,zhang2020does,wang2021understanding}. In sum, previous studies mainly can divided into four directions: 1) inconsistent analysis between privacy policy and apps' behaviors, 2) inconsistent analysis between regulations and apps' behaviors, 3) inconsistent analysis between privacy policy and regulations, 4) automatic generate privacy policy for apps. Recently, more and more researchers started to focus on privacy policy analysis of TPLs as well. PAMDRroid~\cite{zhang2020does} mainly focuses on the personally identifiable information (PII) leakage due to misconfiguration from analytic service libraries.
\xiancm{Besides, please summary the two papers}
\xian{X. Liu, J. Liu, S. Zhu, W. Wang and X. Zhang, "Privacy Risk Analysis and Mitigation of Analytics Libraries in the Android Ecosystem," in IEEE Transactions on Mobile Computing, vol. 19, no. 5, pp. 1184-1199, 1 May 2020, doi: 10.1109/TMC.2019.2903186.
%%%
%%
C. Schindler, M. Atas, T. Strametz, J. Feiner and R. Hofer, "Privacy Leak Identification in Third-Party Android Libraries," 2022 Seventh International Conference On Mobile And Secure Services (MobiSecServ), February 2022, pp. 1-6, doi: 10.1109/MobiSecServ50855.2022.9727217.}
}


% Existing methods are limited to identifying the consistency between apps' behavior and privacy policies~\cite{yu2016revisiting,ppcheck,ppchecker} and ignore the regulation requirements for {\tpl}s.
% Existing methods can not identify TPL-related regulation violations 
%

To regulate TPL usage and help developers better understand TPLs' functionalities\xiancm{we cannot regulate TPL usage, because this work's purpose is to detect the conflicts, how we regulate the TPL usgae, they have many setup readme files can help users to use them}, we develop an \underline{A}utomated \underline{T}hird-party library \underline{P}rivacy leakage \underline{Checker}, namely {\oursystem}, to automatically check the consistency\xiancm{inconsistency} between regulation requirements and TPLs, and they determine whether the host app's usage of TPLs complies with regulations.\xiancm{two sentences is the same meaning, should combine and optimize it}
%
We analyze privacy and security-related laws~\cite{gdpr, ccpa, cpra,  piss,petitcolas1883cryptographie,iccpr}. 
% (\S\ref{sec:bb_regulation_req}).  
% 
%, and the regulations that normalizing software applications~\cite{zhSDKLaw} (\S\ref{sec:bb_regulation_req}). 
% 
We concentrate on TPL-related regulations, e.g., the scope of TPL (\textsc{\small{GDPR Article I.(47), COPPA 312.2}}), and requirements for TPL-related privacy policy statements (\textsc{\small{CFR 332.6}}).
%
\revise{As regulation analysis requires expert knowledge of both legal and software engineering, one expert and one senior researcher, who has conducted research on software engineering and privacy policy analysis for over seven years and two years, respectively, \xian{were invited to} read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. }\xiancm{delete the clause, the sentence is not coherent,}
%
{\oursystem} identifies the inconsistency between TPL and regulation by analyzing TPL's bytecode (\S\ref{sec:tpl_data}) and privacy policies (\S\ref{sec:tpl_pp}).
%
For example, {\oursystem} discovers whether TPLs correctly provide privacy policies.
%
{\oursystem} discloses whether host app's TPL usage comply with regulations(\S\ref{sec:host_app_data}, \S\ref{sec:host_app_pp}). 
% checks the consistency between host app's privacy policies and TPL-related regulation requirements.
%
% By analyzing the host app's privacy policies and binary code, {\oursystem} identifies whether the host app's privacy policy clearly claims TPL usage.
% , e.g., what kinds of data are shared with TPLs rather than only identifying the existence of used TPLs' privacy links~\cite{ppchecker}. 
%
% {\oursystem} implements the following functionalities to achieve such goal and tackles the limitations of existing works accordingly.

\xiancm{I rewrote the above paragraph }

\xianw{Based on our study, we find there is still a research gap with respect to discrepancy analysis between the privacy related behaviors of TPLs and regulations. To this end, we propose a tool, named \oursystem ~(\underline{\textbf{A}}utomated \underline{\textbf{T}}hird-party library \underline{\textbf{P}}rivacy leakage \underline{\textbf{Checker}}) to automatically  check whether the usages of in-app TPLs complies with privacy-related regulations (e.g., {GDPR Article I.(47), COPPA 312.2, CFR 332.6}).
%
As regulation analysis requires expert knowledge of both legal and software engineering, we invited 
one expert and one senior researcher to help us read through related regulations~\cite{gdpr, ccpa, cpra, piss,petitcolas1883cryptographie,iccpr,zhSDKLaw} and summarize requirements for TPLs. Both of them have conducted research on software engineering and privacy policy analysis with experience for over seven years and two years, respectively.
}

It is challenging to develop {\oursystem} due to multiple reasons.
%
First, no standardized data are publicly available for analyzing TPL compliance.
% no dataset is available for research in this area.
%
To counter this issue, we create a novel data set containing 187 TPLs and 642 distinct host apps.\xiancm{why this data is not match the abstract, one is 458 TPLs}
All TPLs' privacy policies are collected and annotated with labeled tokens. \xiancm{but you just collect 23\% of 458, why here you can say all?}
%\textbf{c}) 642 distinct host apps labeled with an integrated TPL list, and 
All host apps' privacy policies are also included.
% \textbf{b}) corresponding privacy policies with labeled tokens,
% \textbf{c}) 642 distinct host apps labeled with an integrated TPL list, and 
% \textbf{d}) corresponding host apps' privacy policies.
%
\revise{Second, it is non-trivial to get TPL data usage because TPLs are usually closed source. }
\xiancm{do you have any reference? or proofs? based on my knowledge, most TPLs are oss. most TPLs in an Android app are open-source as well}
\xiancm{why your challenges here cannot match the abstract you said. there are four challenges, but I think we can use two in abs, but why here you give two new}
% usually provided as compiled code without source code. 
% and it is challenging to trace data usage in close source TPLs. 
{\oursystem} performs static analysis~\cite{soot} to construct the TPL's function call graph and uses data flow analysis to trace TPLs personal information usage without source code (\S\ref{sec:tpl_data}).
% 
We do not conduct dynamic analysis since it cannot execute all possible paths in software~\cite{schindler2022privacy}.
%and it also requires executing the target software and analyzing the data changes during runtime.
%
Moreover, TPLs provide APIs that relies on the host app to trigger them. 
%
Dynamic analysis cannot execute the TPL directly.\xiancm{incorrect}
%
% {\oursystem} uses static analysis~\cite{soot} to construct the TPL's function call graph, and uses data flow analysis to trace TPLs personal information usage (\S\ref{sec:tpl_data}).
% conducts data flow analysis(\S\ref{sec:tpl_data}).
%
Third, analyzing privacy policy is difficult because developers use various natural language to describe the usage of personal information and TPL.
\xiancm{why these challenges cannot match the abstract}
%
To analyze data and TPL usage related statements of privacy policies, {\oursystem} implements an expert system to extract abstract data usage patterns (\S\ref{sec:host_app_pp}) and analyzes the compliance of TPL usage.
\xiancm{there are several issues that make this paper choas. 1. do this paper should consider the single TPL, the independent TPL analysis, or we just consider the in-app TPLs, there are two different things, I do not understand the key targets that the paper want to handle. 
should we consider the pp analysis, but this paper say we just analyze the inconsistencies between TPLs and regulations? what do you means the TPLs here, the behaviors of TPLs, the TPLs consider as the independent software or a part of host app? I still not understand.
}
% {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
% {\oursystem} implements abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).




\begin{comment}



% \xiancm{based on your description the legality analysis is clearly say PI usage in PP in previous paragraph and this paragraph is to say ignore the regulation requirements analysis for TPLs, here, you did not say anything about that. need to detailed description about the functions involving the pp analysis and laws consistency analysis}
% \xiancm{Why \oursystem need to explain here}
%
% For legality identification, {\oursystem} checks whether the {\tpl} contains a privacy policy and uses static analysis to analyze its functionalities to identify the consistency with PP.
% %
% For correctness usage of {\tpl}s, {\oursystem} identifies 1) what {\tpl}s are used by host apps, 2) what kinds data are interacted with {\tpl}s, and 3) whether hosp apps' privacy policy clearly state {\tpl}s' data usage.
%
% \xiancm{I remember your paper need to consider the laws analysis, I cannot find any description about laws analysis in this introduction}
%However, there still exist challenges to be countered when designing {\oursystem}.
% \xian{To achieve such goals, we need to solve the following challenges:}
%



We address the following challenges in the development of {\oursystem}.
%
First, there is no available dataset for research in this area.
%
To counter this issue, we gather a data set containing \textbf{a}) 187 TPLs, \textbf{b}) corresponding privacy policies with labeled tokens, \textbf{d}) 642 distinct host apps labeled with an integrated TPL list and \textbf{f}) %642 
corresponding host apps' privacy policies.
%
% We will release the dataset after the paper gets published.
%
Second, it is non-trivial to track the data usage of TPLs because 1) TPLs are usually provided as compiled code without source code and 2) it is difficult to construct a call graph that contains all important edges (invocation relations)~\cite{reif2016call}.
%
To tackle the challenge, {\oursystem} is built on {\soot}~\cite{soot} that is a popular static analysis tool and does not require the source code.
%
To construct a comprehensive callgraph of the TPL to facilitate personal information track, {\oursystem} implements new methods (\S\ref{sec:tpl_data})  to optimize TPLs’ FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Third, privacy policy analysis remains challenging as a natural language processing task, because privacy policies use different patterns (\S\ref{sec:host_app_pp}) to describe the usage,and the usage of TPLs.% and data sharing with TPLs.
%
To counter the challenge, {\oursystem} applies hanlp~\cite{hanlp21} is natural language processing tool with multi-task learning with transformer encoders.
% that is capable of dealing with both English version and Chines version natural language corpus to deal with  privacy policies (\S\ref{sec:tpl_pp})
%
{\oursystem} designs abundant patterns matching methods to extract TPL related statements in host app's privacy policy (\S\ref{sec:host_app_pp}).
%





% \noindent\textbf{Availability of dataset.}


\noindent\textbf{Data leakage analysis in third-party  libraries.}
%
\xiancm{Based on your description, I cannot see any challenges here, challenges should be the point that difficult to solve, where is it}
As TPLs are usually provided as compiled code~\cite{qiu2021libcapsule} without source code, {\oursystem} uses {\soot}~\cite{soot} to analyze TPLs that does not require source code.
%
{\oursystem} applies static analysis to identify the data leakage in third-party libraries.
%
{\oursystem} analyzes the data flow of TPLs to identify the definition and usage chain~\cite{pande1994interprocedural} (\S\ref{sec:tpl_data}) of personal information (PI).
%
As {\oursystem} uses function call graphs (FCG) to better trace the usage of target variables, we propose new methods (\S\ref{sec:tpl_data}) to optimize TPLs' FCG construction progress by investigating comprehensive entry points set for {\soot}.
%
Excepting PI name matching with predefined data types, we also construct a mapping knowledge set that builds connections with PI name and Android APIs to improve the variable locating precision.
% 



% \noindent\textbf{Identification of host apps' PI interaction with TPLs.}
%
% \cite{wei2018amandroid}


\end{comment}



\begin{comment}

\noindent\textbf{TPL usage identification in host apps.}
%
Taint analysis is widely used to identify data leakage in software with predefined sources and sinks.
%
However, it is still a challenge to locate the destination of those data leakages while it is necessary to locate them to further identify the correctness of host apps' usage of TPLs. 
%
{\oursystem} first builds a knowledge set to match {\tpl} related invocations in binary code.% (\kaifa{revise it}).
%
Combining the data flow of personal information and {\tpl}s, {\oursystem} determines the destination of PI data (\S\ref{sec:host_app_data})

%
% \xiancm{I am dying if I just read more lines..... I do not know what are you doing...... many things are totally incorrect}
% \xiancm{The figure cannot show any useful information and ugly }
% % 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{figures/tpl_enumeration_in_host_app_pp_new.png}
%     \caption{TPL usage in privacy policy of \textit{jp.ne.ibis.ibis-paintx.app}}
%     \label{fig:pp_tpl_list}
% \end{figure} 你见过婊子吗


\noindent\textbf{TPL related statements extraction in host apps' privacy policies.}
%
\revise{Existing data-related statements extraction methods~\cite{ppcheck, andow2019policylint} are generally constructed on named entity recognition techniques that require a large amount of labeled corpus for model training.
%
Besides, existing methods are usually based on predefined sharing and collecting verbs to locate those data-related sentences. \xiancm{you just say the existing method, where is the challenges of your work}
%
Although those methods achieves desirable performance for analyzing apps' data collection statements in privacy policy, those methods may omit information related to {\tpl}s because host apps may provide {\tpl}s' information in form of table or enumeration.} \xiancm{this is limitation of existing work is not your work's challenges. logic chaos}
%(as is illustrated in 
% Fig.~\ref{fig:pp_table} and 
% Fig.~\ref{fig:pp_tpl_list} separately).  
%
Besides extending the existing sharing and collection words list to locate data usage-related statements in the privacy policy, {\oursystem} also designs \revise{heuristic patterns}\xiancm{when anytime you use heuristic you need to explain the heuristic patterns first} to precisely extract {\tpl} related statements for further flow-to-policy analysis.
\xiancm{I still cannot see any challenges here}



\end{comment}
% write a paragraph to summarize the performance of our tool

\vspace{0.5em}
Overall, our contributions are summarized as follows:


\begin{itemize}[leftmargin=*]


\item We propose a novel system named {\oursystem} to analyze the compliance of Android TPLs. 
%
{\oursystem} uses static analysis to identify TPL's user data access behavior and host apps' data interaction with TPLs, and uses  NLP techniques to analyze TPLs' and host apps' privacy policies.
% TPLs' personal information accessing both individually and inside host apps, and applies NLP techniques to analyze TPLs' and host apps' privacy policies.
%
Combining the results of bytecode analysis and privacy policy analysis, {\oursystem} determines whether TPLs and usage of TPLs in host apps comply with regulation. \xiancm{what do your mean the TPLs and usage of TPLs in host apps, what's kinds of the differences}
\xiancm{how do we just analysis the TPLs' behaviors and pp, we can get to know whether a TPL comply with regulations or not, if here we miss some descriptions? I do not know? here we want to do is that the conflicts between the TPLs' behaviors and pp, or TPL's behaviors conflcit with laws, hard to clear my mind from the description. I suggest clear the mind and give the detailed description about what kinds of the issues we really want to handle. }
% requirements or not.



\item To evaluate the performance of {\oursystem} and facilitate further research in this area, we construct a privacy dataset that includes 187 TPLs and their privacy policies, and 642 host apps and their privacy policies.
\xiancm{why the dataset is inconsistent with tht of abs, 458 tpls with the 642 apps, and 178 TPLs with the 256 apps}
% 
Our dataset contains TPL's privacy policies with related data access behavior.
%
Our dataset includes host app's privacy policies that contains labels related to host app's interaction with TPLs.
% TPL's privacy policies in our data set contain labeled corpus related to TPLs' data accessing behavior and the host app's privacy policies are labeled with used TPLs and data interaction with TPLs.
%
Our dataset will be released after this paper get published.

% \vspace{1em}

\item {\oursystem} discovers over 23\% (107 out of 458) of TPLs miss providing privacy policies, 37\% (24 out of 65) of TPL's privacy policies conceal data usage.\xiancm{hard to understand, where is the 187 TPLs, why suddenly the number changes to 65, that is really too dangerous. these data cannot match}
%
{\oursystem} discovers over 65\% (168 out of 256) of host apps violate the regulation requirements for disclosing data interactions with TPLs. \xiancm{there are many dataset, make people confused}





\end{itemize}









\begin{comment}
%
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.






This is introduction
\subsection{Our target}


\begin{itemize}
    \item We have to identify whether the action of {\tpl} is consistent with {\tpl}'s privacy policy.
     
    \item We need to detect all data usage (at least sensitive data usage) in APP. And specify which groups are used by app and which groups are used by {\tpl}.
    
    \item
\end{itemize}


Tool name: {\oursystem} Android Third party libraries misuse and Privacy policy conflict checker.

\subsection{Challenges}

\textbf{1. {\tpl} information extraction}: Information about the usage of {\tpl}, the data related to {\tpl} are usually formatted as a table or organized as form of explanations (for example, facebook: data1, data2 \kaifa{put a case study in Appendix}).
%
% We apply \texttt{Tablemaster} to extract information from tables and \kaifa{a new NLP technique} to merge information in form of explanations.
\kaifa{not suitable. I analyze 3502 privacy policy. Only 471/3502 privacy policy contains html tag \textit{table}. I manually checked 200/471. Only 6/200 contains table are related to data usage that cannot be analyzed by the method in PolicyLint.}

PolicyLint~\cite{andow2019policylint} deals with the table data by merging the formatted lists into sentences.
%
This preprocessing method fails when only noun phrase on the table because the method in PolicyLint directly merges the items together without considering the characteristics of table, i.e., the data in each item shares same attributes. \kaifa{give an example in appendix}
%


\textbf{2. Data analysis in third party libraries. }
As third party libraries may not have a \textit{main} function, it is difficult to analyze the data collection and sharing actions by {\tpl} by static analysis.
%
For dynamic analysis,  we must find the apk that uses the {\tpl} and leverage the data usage of {\tpl}. 
%
However, it's not easy to accurately find an apk that use target {\tpl} nor identify the data usage by the apk is responsible by the host apk or the {\tpl}. 
%
Besides, the {\tpl} hosted apk may not use all data or functions of target {\tpl}.
%
That makes the usage of dynamic analysis for {\tpl} data usage into a chicken-and-egg situation.
%
Thus, to extract data usage of {\tpl}, we build a tool based on soot to conduct static analysis.
%
\kaifa{details, how to design such a tool}


\textbf{3. Consistency analysis} We focus on two aspect of consistency analysis: a) whether the app's privacy policy covers all {\tpl} usage. 
%
To relax condition, the app's privacy policy should contain all {\tpl}s that collect or share data.
%
b) If the app's privacy policy covers the {\tpl} usage, does the data usage in privacy policy consistent with the {\tpl}'s real data usage.

\end{comment}
